Trade When Opportunity Comes: Price Movement Forecasting via Locality-Aware Attention and Iterative Refinement Labeling

Price movement forecasting, aimed at predicting financial asset trends based on current market information, has achieved promising advancements through machine learning (ML) methods. Most existing ML methods, however, struggle with the extremely low signal-to-noise ratio and stochastic nature of financial data, often mistaking noises for real trading signals without careful selection of potentially profitable samples. To address this issue, we propose LARA, a novel price movement forecasting framework with two main components: Locality-Aware Attention (LA-Attention) and Iterative Refinement Labeling (RA-Labeling). (1) LA-Attention, enhanced by metric learning techniques, automatically extracts the potentially profitable samples through masked attention scheme and task-specific distance metrics. (2) RA-Labeling further iteratively refines the noisy labels of potentially profitable samples, and combines the learned predictors robust to the unseen and noisy samples. In a set of experiments on three real-world financial markets: stocks, cryptocurrencies, and ETFs, LARA significantly outperforms several machine learning based methods on the Qlib quantitative investment platform. Extensive ablation studies confirm LARA's superior ability in capturing more reliable trading opportunities.

==> Case_study.tex <==
\section{Case study: Locality-Aware Attention}
\label{sec:case_study}
We propose the Locality-Aware Attention algorithm. First, it \textcolor{red}{audits} financial datasets into the subset\textcolor{red}{ of interest} according to a attention module; second, it retests them by building more precise classifiers over them. \textcolor{red}{This has the advantage of} dividing the space of financial datasets into a distinct region in which similar samples will fall. So, a natural problem arises here: how does this algorithm work?

We generate a small case to study the above essential question shown in Figure \ref{fig_case}. Even though the optimal linear classifier (omitting the bias term for  convenience) is determined\footnote{This conclusion is intuitive, and the rigorous mathematical proof can refer to \cite{bishop2006pattern}}, $y = x$ , to classify $\mathcal{N}\left( \left(-2,2\right), 4I_2 \right)$ and $\mathcal{N}\left( \left(2,-2\right), 4I_2 \right)$, the actual classifier built over the whole set will deviate from the optimal owing to the insufficient samples and noise, especially in the region where positive and negative samples coincide. Then intuitively, searching for the blue and red regions with less noise and then building classifiers over them will give out a more robust decision boundary around the optimal one. Moreover in testing phase, the samples we attend to in blue and red will be more robust to the deviation of the decision boundary, which falls in green.
Hence, the Locality-Aware Attention algorithm including \textcolor{red}{auditioning and retesting} is more robust to the deviation of the learned decision boundary and deserves further study.

% We generate a small case to study the above essential question. As shown in Figure \ref{fig_case}, we draw random 200 positive training samples using the first Gaussian distribution $\mathcal{N}\left( \left(0,4\right), 4I_2 \right)$ and 200 negative training samples using the second one $\mathcal{N}\left( \left(4,0\right), 4I_2 \right)$. And the above two Gaussian distributions are independent of each other. The same process and configurations are used to generate the testing data. In order to illustrate the motivation briefly, we use the linear classifier as the retest learner in this section, whose bias term is fixed as 2 and origin is point $\left(2, 2\right)$, to discriminate the positive and negative samples. The form is formulated as $y = w \cdot x + 2$, and the dimension of $w$ and $x$ in this example is only one. 

\begin{figure}[htbp]
	\centering
	\includegraphics[width=.28\textwidth]{pics/case-study.pdf}
	\caption{The case-study example for illustrating how Locality-Aware Attention works. Respectively sample 200 data points from $\mathcal{N}\left( \left(-2,2\right), 4I_2 \right)$ and $\mathcal{N}\left( \left(2,-2\right), 4I_2 \right)$ as positive and negative training samples. Testing samples are sampled from the same distributions. The blue region (up left) stands for the super-positive area with less noise. The same for the super-negative area in the red region (low right). For a linear classifier $y = w \cdot x$, the red dotted line represents the optimal solution and other solutions will deviate from the optimal (mainly located in green) due to the insufficient samples and noise.}
	\label{fig_case}
\end{figure}

% TODO 描述数据生成过程
% \subsection{Case 1: eager learners only}
% % We assume the similar samples have the similar label distribution, and then the similar labels. And the principle behind the nearest neighbor methods is to find a predefined number of training samples closest to the query testing sample in some distance metric, and predict the label according to them. It agrees with our assumptions. We use the two most commonly used nearest-neighbor techniques: k-neighbors classification and r-radius classifications. And in validation datasets, we select the two main parameters: 
% % k-nearest neighbors of each query point and fixed radius r of each training point.
% In the first case, as we know, for two independent Gaussian distributions, the decision plane is the vertical line connecting their midpoint \footnote{This conclusion is intuitive, and the rigorous mathematical proof can refer to \cite{bishop2006pattern}}. In the training phase, the optimal linear classifier, whose bias term is fixed 2, is $y = x + 2$. However, this optimal linear classifier is determined, when we know the distribution of the positive and negative generators. In practice, we can only get some data points induced from these distribution generators. In most actual cases, the training positive samples and training negative samples are not even. Thus the linear classifier, whose origin is point $\left(2, 2\right)$, will deviate the optimal line $y = x + 2$ and fall in the purple region. We can get intuition from Figure \ref{fig_case}, this trained classifier is not robust, and may produce errors when predicting on testing datasets, especially in the region where positive and negative samples coincide. It agrees with our assumptions that eager learner only in this simple example is not robust and the performance will degrade on testing datasets.

% \subsection{Case 2: Semi-lazy framework}
% As for eager learners, we use the gradient boosting decision trees for case studies, since the traditional time-series analysis models and machine learning models have been reported to be less effective than GBM.

% As we know, for two independent Gaussian distributions, the decision plane is the vertical line connecting their midpoint \footnote{This conclusion is intuitive, and the rigorous mathematical proof can refer to \cite{bishop2006pattern}}. In the training phase, the optimal linear classifier is $y = x + 2$, whose bias term is fixed 2. However, this optimal linear classifier is determined, when we know the distribution of the positive and negative generators. In practice, we can only get some data points sampled from these distribution generators. In most scenarios, the training positive and negative samples are not even. Thus the linear classifier will deviate the optimal line $y = x + 2$ and fall in the purple region. We can get intuition from Figure \ref{fig_case}, this trained classifier is not robust, and may produce errors when predicting on testing datasets, especially in the region where positive and negative samples coincide. And in the testing phase, we first use clustering methods to audition the positive and negative points, and we can roughly get super-positive points in the blue sector and super-negative points in the red sector. Second, we use the linear classifier, to make predictions on these samples of interest. Although the trained classifier may fall in the purple region, the samples of interest are robust to this deviation. 



\begin{figure*}[htp]
    \centering
    \includegraphics[width=18cm]{pics/framework.pdf}
    \caption{The architecture of our proposed LARA framework. (a) The input of the model. (b) The metric learning module. (c) The localization module with Locality-Aware Attention. (d) The Adaptive Refined Labeling module.}
    \label{fig:framework}
\end{figure*}

\textbf{Summary.} These cases show that the standard learner is distant from optimal or even satisfactory with noisy training datasets. Our proposed \textcolor{blue}{two-stage audition-retest label attention method} is more powerful to select samples \textcolor{blue}{of interest.}
% compared with the standard learning (e.g. classification) approaches 
It is more suitable for actual fast-changing financial datasets consisting of \textcolor{blue}{many uncertain data points}, where positive and negative samples coincide just like in Figure \ref{fig_case}. \textcolor{red}{It can pay attention to the samples of interest to boost the prediction in the test phase.}

==> Experiment_temp.tex <==
\section{Experiments}
Our proposed framework are qualified for real-world applications. We evaluate our framework on the Chinese ETF high-frequency datasets. All implementation codes can be found in the Github repo\footnote{We will release out Github repo address in the camera-ready version paper due to anonymity considerations.}. And demonstrative backtesting results are available at this https URL\footnote{……}. As such, in the following section, we conduct experiments with the aim to answer the three following research questions:
\begin{itemize}
    \item \textbf{RQ1:} Does the proposed three key elements(semi-lazy; bi-level labeling and metric learning) of SABA really work? Does the subset with selection using our methods can promote the performance of predictors?
    \item \textbf{RQ2:} What is the efficiency compared to the state-of-the-art traditional time-series analysis and machine learning methods?
    \item \textbf{RQ3:} Is the hyper-parameter sensitive? And is the computational complexity high?
\end{itemize}


\subsection{Dataset description}
% TODO: One statistic form is missing.
% TODO: list some used factors.
We conduct our experiments over the Chinese exchange traded fund (ETF) high-frequency financial datasets as depicted in Tabel \ref{table_datasets}, which are collected from HuaTai cloud service\footnote{}. The time span of the dataset is from Jan. 1, 2020 to Jul. 6 2020. The magnitude of datasets in this time range is sufficient for high-frequency trading, which cover several important economics events, including 2020 financial market crash and COVID-19, and representative to evaluate the performance in diverse market status. The granularity of datasets in our experiments is tick-level(3-second), which is a measure of the minimum upward or downward movement in the price of a security. And it belongs to the high-frequency  fast-changing market environment. We back-test our algorithms over a seven-month trading period and there are 110446 trading instances in all. Each record contains last price, amount, volume, IOPV and five-level price-volume data, which are basic elements of ETF datasets. The features in our experiment are composed of two parts. The first one is technical factors and limit order book factors, such as Moving average convergence divergence (MACD)[] and buy/sell pressure indicators. And the second one is ETF factors, such as the weighted return ratio among some ETF.

\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}

\begin{table}
    \caption{Details of the datasets.}
    \centering
    \begin{tabular}{|l|l|}
        \hline
        \makecell[c]{\textbf{Property}} & \makecell[c]{\textbf{Value}} \\  \hline
        Time spans & 2020-01-01 -- 2020-07-06 \\ \hline
        Datasets(ETF) &  \tabincell{c}{159915.SZ; 512480.SH; \\  512880.SH; 515050.SH} \\  \hline
        Time granularity & \makecell[c]{3 seconds} \\ \hline
        \#Instances & \makecell[c]{110446} \\ \hline
        \#Features & \makecell[c]{40} \\ \hline
    \end{tabular}
    \label{table_datasets}
\end{table}


\subsection{Performance matrices}
\label{eva}
    \textit{Precision:} While standard classification problem care more about the prediction accuracy on the entire datasets. While in the financial environment, we care more about positive prediction samples, because these samples can lead us to construct the trading signals. Unlike the experiment setting in [], they retrieved approximately 1$\%$ of the samples, these experimental setting cannot transform the actual trading behavior, because they utilize the future datasets. We adjust the threshold of probability of the training sets, and use it to back-test on the testing sets. And this method is comparable with the traditional machine learning pipeline and can be used in practice.
	In this paper, we use the following traditional financial metrics to evaluate the performance of our proposed algorithm, which can be classified into three main categories: \textit{Profitability}, \textit{Risk} and \textit{Performance Ratios}. 
	\begin{itemize}
	\item \textit{Profitability} --- \textbf{Annual return}, AR Annual return is the basic and direct index to evaluate the performance of the corresponding strategy. It is the geometric average of returns scaling $l$ trading days to one year. We can assume that there are about 250 market trading days in a year.
	\begin{equation}
	AR = (1 + return) ^{\frac{250}{l}} - 1 \label{eq_1}
	\end{equation}

	\item \textit{Profitability} --- \textbf{Winning percentage}, WP is the percentage of profitable trades. It is desirable to have as high winning percentages as possible. It is defined as follows:
	\begin{equation}
	WP = \frac{\text{the number of winning trades}}{\text{the number of total trades}} \label{eq_5}
	\end{equation}

	\item \textit{Risk} --- \textbf{Annual volatility}, AV Annual volatility is the variation in its return over a period of time. To present the volatility in annualized terms, we simply need to multiply our daily standard deviation by the square root of 250.
	\begin{equation}
	AV = \sqrt{250} \cdot \sqrt{\frac{1}{l}\sum_{i=1}^{l}(x_i - \overline{x})^2} \label{eq_2}
	\end{equation}
	where $\overline{x}$ is the mean average, that is, $\overline{x} = \frac{1}{l}\sum_{i=1}^{l} x_i$

	\item \textit{Risk} --- \textbf{Max drawdown}, MD Max drawdown is the maximum observed loss from a peak to a bottom of your invested assets. Max drawdown is an important indicator of downside risk over a specified time period. It is calculated by the following formula:
	\begin{equation}
	MD = max_{\substack{t \in (0,l) \\ \tau \in (0,t)}} |x_t - x_{\tau}| \label{eq_3}
	\end{equation}

	\item \textit{Performance Ratios} --- \textbf{Sharp ratio}, SR Sharp ratio is used to help investors to understand the return of an investment compared to its risk. The ratio is the average return earned in excess of the risk-free rate per unit of volatility or total risk. The formula for sharp ratio is: 
	\begin{equation}
	SR = \frac{R - R_f}{\sigma} \label{eq_4}
	\end{equation}
	where $R$ denotes the return of the investment portfolio, $R_f$ denotes the risk-free benchmark rate, and the denominator $\sigma$ denotes the standard deviation of the investment portfolio's excess return.

	\item \textit{Performance Ratios} --- \textbf{Profit factor}, PF Profit factor is the ratio of the average mean of winnings to the average mean of losses for the entire trading period. It measures the money-making ability for each of winnings in excess of that for each of the losses.
	\begin{equation}
	PF = \frac{\mathbb{E} [\text{return of winnings}]}{\mathbb{E} [\text{return of losses}]} \label{eq_6}
	\end{equation}

	\end{itemize}

\subsection{Model implementation}
In our experiments, we follow the standard machine learning pipeline, viz. Jan. 1, 2020 to Apr. 17, 2020 for training, Apr. 20, 2020 to May. 29, 2020 for validation, May. 30, 2020 to July 6, 2020 for testing. And the Conditional Label Estimation we use the KNN/RNN method (detailed in Appendix). The metric learning method we use is Sparse High-Dimensional Metric Learning (SDML), which is an efficient sparse metric learning in high-dimensional space via double regularization. And the ensemble methods of bi-level labeling we use are 'vote', 'last' and 'and', which described in section \ref{sec-bi-level}. In order to fair comparison, the hyper-parameters in metric learning, conditional label estimation and bi-level labeling we use are the default recommended ones.

And we compare with the following methods in our experiments: it can divided into two main classes:
\begin{itemize}
    \item time-series analysis methods
        \item
    \item traditional machine learning methods
        \item
    
\end{itemize}

\subsection{Ablation experimental results}
We conduct an ablation experiment for three proposed methods, 

And the ratio of the switch strategy in bi-level labeling 

\begin{table*}[htp]
    \centering
    \begin{tabular}{c|ccc|ccccc}
    \toprule
        Fund & Semi-Lazy & Metric & Labeling & Precision(\%) & Transactions & Profit-Loss Ratio & Max Drawdown & One-trade Return  \\
    \midrule
        \multirow{8}*{512880} 
         & - & - & - & 53.20  $\pm$ 0.23  & 15760.8  $\pm$ 161.1  & 1.115  $\pm$ 0.015  & -0.0077  $\pm$ 0.0009  & 8.04E-05 $\pm$ 1.05E-06 \\ 
         & RNN & - & - & 56.01  $\pm$ 0.15  & 6076.4  $\pm$ 70.9  & 1.242  $\pm$ 0.024  & -0.0042  $\pm$ 0.0008  & 1.37E-04 $\pm$ 3.66E-06 \\ 
         & - & TRUE & - & 57.83  $\pm$ 0.17  & 16850.8  $\pm$ 71.2  & 1.029  $\pm$ 0.022  & -0.0190  $\pm$ 0.0031  & 7.87E-05 $\pm$ 2.98E-06 \\ 
         & RNN & TRUE & - & 75.05  $\pm$ 1.62  & 484.8  $\pm$ 99.6  & 1.288  $\pm$ 0.173  & -0.0029  $\pm$ 0.0008  & 6.95E-04 $\pm$ 5.08E-05 \\ 
         & - & - & TRUE & 54.92  $\pm$ 0.14  & 13256.4  $\pm$ 41.7  & 1.138  $\pm$ 0.014  & -0.0063  $\pm$ 0.0010  & 9.27E-05 $\pm$ 1.86E-06 \\ 
         & RNN & - & TRUE & 58.37  $\pm$ 0.34  & 4737.6  $\pm$ 56.9  & 1.211  $\pm$ 0.010  & -0.0027  $\pm$ 0.0007  & 1.41E-04 $\pm$ 4.10E-06 \\ 
         & - & TRUE & TRUE & 59.77  $\pm$ 0.14  & 14204.4  $\pm$ 141.0  & 1.081  $\pm$ 0.021  & -0.0108  $\pm$ 0.0017  & 9.02E-05 $\pm$ 1.76E-06 \\ 
         & RNN & TRUE & TRUE & 80.40  $\pm$ 2.02  & 245.8  $\pm$ 56.3  & 1.279  $\pm$ 0.215  & -0.0022  $\pm$ 0.0010  & 8.42E-04 $\pm$ 4.04E-05 \\ 
    \midrule
        \multirow{8}*{512480} 
         & - & - & - & 49.73  $\pm$ 0.30  & 9856.0  $\pm$ 26.4  & 1.185  $\pm$ 0.005  & -0.0046  $\pm$ 0.0000  & 1.55E-04 $\pm$ 4.87E-06 \\ 
         & RNN & - & - & 60.58  $\pm$ 1.17  & 2821.0  $\pm$ 105.3  & 1.595  $\pm$ 0.033  & -0.0030  $\pm$ 0.0003  & 3.47E-04 $\pm$ 4.42E-06 \\ 
         & - & TRUE & - & 58.65  $\pm$ 0.32  & 8442.6  $\pm$ 29.6  & 1.085  $\pm$ 0.004  & -0.0074  $\pm$ 0.0006  & 1.68E-04 $\pm$ 1.85E-06 \\ 
         & RNN & TRUE & - & 84.39  $\pm$ 0.96  & 616.6  $\pm$ 32.1  & 1.886  $\pm$ 0.101  & -0.0032  $\pm$ 0.0003  & 6.70E-04 $\pm$ 2.50E-05 \\ 
         & - & - & TRUE & 64.99  $\pm$ 0.31  & 7424.4  $\pm$ 59.4  & 1.255  $\pm$ 0.011  & -0.0045  $\pm$ 0.0008  & 1.92E-04 $\pm$ 1.93E-06 \\ 
         & RNN & - & TRUE & 52.58  $\pm$ 0.84  & 1461.0  $\pm$ 51.5  & 1.826  $\pm$ 0.021  & -0.0027  $\pm$ 0.0008  & 4.74E-04 $\pm$ 4.16E-06 \\ 
         & - & TRUE & TRUE & 62.11  $\pm$ 0.18  & 6625.0  $\pm$ 23.1  & 1.151  $\pm$ 0.012  & -0.0051  $\pm$ 0.0009  & 2.01E-04 $\pm$ 2.26E-06 \\ 
         & RNN & TRUE & TRUE & 88.70  $\pm$ 1.49  & 299.6  $\pm$ 22.1  & 2.017  $\pm$ 0.228  & -0.0024  $\pm$ 0.0007  & 8.47E-04 $\pm$ 2.36E-05 \\ 
    \midrule
        \multirow{8}*{515050} 
         & - & - & - & 25.21  $\pm$ 0.25  & 15860.2  $\pm$ 313.1  & 1.011  $\pm$ 0.010  & -0.0052  $\pm$ 0.0002  & 9.36E-05 $\pm$ 1.63E-06 \\ 
         & KNN & - & - & 26.87  $\pm$ 0.24  & 7617.2  $\pm$ 172.6  & 1.126  $\pm$ 0.010  & -0.0043  $\pm$ 0.0006  & 1.93E-04 $\pm$ 5.59E-06 \\ 
         & - & TRUE & - & 35.20  $\pm$ 0.28  & 10666.8  $\pm$ 218.1  & 1.008  $\pm$ 0.008  & -0.0059  $\pm$ 0.0006  & 1.41E-04 $\pm$ 3.08E-06 \\ 
         & KNN & TRUE & - & 56.76  $\pm$ 1.07  & 820.4  $\pm$ 59.7  & 1.379  $\pm$ 0.074  & -0.0027  $\pm$ 0.0002  & 6.33E-04 $\pm$ 1.35E-04 \\ 
         & - & - & TRUE & 26.46  $\pm$ 0.23  & 13020.4  $\pm$ 470.8  & 1.041  $\pm$ 0.006  & -0.0044  $\pm$ 0.0000  & 1.17E-04 $\pm$ 1.84E-06 \\ 
         & KNN & - & TRUE & 27.65  $\pm$ 0.43  & 4828.4  $\pm$ 84.7  & 1.184  $\pm$ 0.017  & -0.0037  $\pm$ 0.0002  & 2.65E-04 $\pm$ 4.42E-06 \\ 
         & - & TRUE & TRUE & 37.96  $\pm$ 0.31  & 8378.4  $\pm$ 149.0  & 1.023  $\pm$ 0.006  & -0.0056  $\pm$ 0.0011  & 1.73E-04 $\pm$ 2.76E-06 \\ 
         & KNN & TRUE & TRUE & 63.59  $\pm$ 3.62  & 282.8  $\pm$ 15.4  & 1.655  $\pm$ 0.120  & -0.0014  $\pm$ 0.0003  & 9.08E-04 $\pm$ 6.63E-05 \\ 
    \midrule
        \multirow{8}*{159915} 
         & - & - & - & 19.84  $\pm$ 0.06  & 13846.8  $\pm$ 218.6  & 1.013  $\pm$ 0.006  & -0.0042  $\pm$ 0.0004  & 8.23E-05 $\pm$ 1.88E-06 \\ 
         & KNN & - & - & 23.92  $\pm$ 0.47  & 7072.4  $\pm$ 212.1  & 1.140  $\pm$ 0.017  & -0.0027  $\pm$ 0.0001  & 1.44E-04 $\pm$ 8.97E-06 \\ 
         & - & TRUE & - & 28.94  $\pm$ 0.26  & 7214.2  $\pm$ 141.3  & 1.065  $\pm$ 0.014  & -0.0054  $\pm$ 0.0009  & 1.37E-04 $\pm$ 1.07E-06 \\ 
         & KNN & TRUE & - & 44.93  $\pm$ 2.66  & 806.8  $\pm$ 233.9  & 1.483  $\pm$ 0.212  & -0.0018  $\pm$ 0.0011  & 4.35E-04 $\pm$ 3.11E-05 \\ 
         & - & - & TRUE & 21.32  $\pm$ 0.10  & 11189.0  $\pm$ 161.3  & 1.060  $\pm$ 0.004  & -0.0041  $\pm$ 0.0002  & 1.04E-04 $\pm$ 1.73E-06 \\ 
         & KNN & - & TRUE & 26.63  $\pm$ 0.11  & 4548.8  $\pm$ 114.8  & 1.235  $\pm$ 0.015  & -0.0022  $\pm$ 0.0004  & 1.94E-04 $\pm$ 5.90E-06 \\ 
         & - & TRUE & TRUE & 31.48  $\pm$ 0.35  & 5479.0  $\pm$ 128.6  & 1.127  $\pm$ 0.016  & -0.0033  $\pm$ 0.0016  & 1.70E-04 $\pm$ 1.01E-06 \\ 
         & KNN & TRUE & TRUE & 51.56  $\pm$ 3.41  & 324.0  $\pm$ 147.6  & 1.675  $\pm$ 0.075  & -0.0013  $\pm$ 0.0008  & 6.25E-04 $\pm$ 4.08E-05 \\ 
    \bottomrule
    \end{tabular}
    \caption{Ablation experiments with 4 ETFs. Long position in lastprice.}
    \label{tab:ablation-long-position-lastprice}
\end{table*}

\begin{table*}[htp]
    \centering
    \begin{tabular}{c|ccc|ccccc}
    \toprule
        Fund & Semi-Lazy & Metric & Labeling & Precision(\%) & Transactions & Profit-Loss Ratio & Max Drawdown & One-trade Return  \\
    \midrule
        \multirow{8}*{512880} 
         & - & - & - & 51.72  $\pm$ 0.25  & 16458.2  $\pm$ 181.6  & 0.992  $\pm$ 0.014  & -0.0225  $\pm$ 0.0017  & 7.55E-05 $\pm$ 2.86E-06 \\ 
         & RNN & - & - & 57.18  $\pm$ 0.18  & 7333.2  $\pm$ 104.7  & 1.113  $\pm$ 0.038  & -0.0077  $\pm$ 0.0017  & 1.50E-04 $\pm$ 1.35E-06 \\ 
         & - & TRUE & - & 53.75  $\pm$ 0.56  & 17754.0  $\pm$ 339.3  & 0.942  $\pm$ 0.013  & -0.0863  $\pm$ 0.0016  & 4.67E-05 $\pm$ 4.87E-05 \\ 
         & RNN & TRUE & - & 71.26  $\pm$ 2.04  & 588.8  $\pm$ 93.9  & 1.097  $\pm$ 0.104  & -0.0049  $\pm$ 0.0108  & 5.88E-04 $\pm$ 1.29E-06 \\ 
         & - & - & TRUE & 53.60  $\pm$ 0.22  & 13537.4  $\pm$ 114.4  & 1.024  $\pm$ 0.012  & -0.0125  $\pm$ 0.0000  & 9.16E-05 $\pm$ 4.50E-06 \\ 
         & RNN & - & TRUE & 58.85  $\pm$ 0.28  & 5529.2  $\pm$ 20.3  & 1.120  $\pm$ 0.036  & -0.0054  $\pm$ 0.0011  & 1.64E-04 $\pm$ 2.56E-06 \\ 
         & - & TRUE & TRUE & 57.87  $\pm$ 0.30  & 13735.2  $\pm$ 224.2  & 0.980  $\pm$ 0.019  & -0.0331  $\pm$ 0.0041  & 7.39E-05 $\pm$ 6.24E-05 \\ 
         & RNN & TRUE & TRUE & 78.37  $\pm$ 3.46  & 297.2  $\pm$ 72.3  & 1.100  $\pm$ 0.253  & -0.0045  $\pm$ 0.0034  & 7.24E-04 $\pm$ 2.89E-06 \\ 
    \midrule
        \multirow{8}*{512480} 
         & - & - & - & 42.95  $\pm$ 0.13  & 10934.8  $\pm$ 125.6  & 1.161  $\pm$ 0.006  & -0.0041  $\pm$ 0.0005  & 1.19E-04 $\pm$ 5.25E-06 \\ 
         & KNN & - & - & 53.59  $\pm$ 0.61  & 4049.2  $\pm$ 152.9  & 1.432  $\pm$ 0.031  & -0.0032  $\pm$ 0.0004  & 2.33E-04 $\pm$ 1.51E-06 \\ 
         & - & TRUE & - & 52.48  $\pm$ 0.10  & 7940.2  $\pm$ 82.6  & 1.121  $\pm$ 0.008  & -0.0059  $\pm$ 0.0000  & 1.45E-04 $\pm$ 1.75E-05 \\ 
         & KNN & TRUE & - & 77.17  $\pm$ 2.03  & 967.8  $\pm$ 49.5  & 1.621  $\pm$ 0.067  & -0.0028  $\pm$ 0.0007  & 4.02E-04 $\pm$ 2.02E-06 \\ 
         & - & - & TRUE & 45.83  $\pm$ 0.27  & 8702.2  $\pm$ 47.4  & 1.219  $\pm$ 0.009  & -0.0035  $\pm$ 0.0001  & 1.43E-04 $\pm$ 2.52E-06 \\ 
         & KNN & - & TRUE & 58.11  $\pm$ 0.46  & 2625.8  $\pm$ 39.0  & 1.583  $\pm$ 0.014  & -0.0023  $\pm$ 0.0003  & 2.92E-04 $\pm$ 1.69E-06 \\ 
         & - & TRUE & TRUE & 55.81  $\pm$ 0.19  & 6246.8  $\pm$ 41.0  & 1.188  $\pm$ 0.007  & -0.0046  $\pm$ 0.0007  & 1.74E-04 $\pm$ 9.31E-06 \\ 
         & KNN & TRUE & TRUE & 85.03  $\pm$ 0.91  & 548.0  $\pm$ 16.2  & 2.018  $\pm$ 0.148  & -0.0016  $\pm$ 0.0009  & 5.32E-04 $\pm$ 2.32E-06 \\ 
    \midrule
        \multirow{8}*{515050} 
         & - & - & - & 27.71  $\pm$ 0.16  & 11412.2  $\pm$ 109.4  & 1.047  $\pm$ 0.007  & -0.0053  $\pm$ 0.0006  & 1.31E-04 $\pm$ 6.29E-06 \\ 
         & KNN & - & - & 36.72  $\pm$ 0.60  & 4294.2  $\pm$ 163.3  & 1.189  $\pm$ 0.006  & -0.0035  $\pm$ 0.0004  & 2.65E-04 $\pm$ 1.61E-06 \\ 
         & - & TRUE & - & 33.92  $\pm$ 0.42  & 8703.6  $\pm$ 185.4  & 1.039  $\pm$ 0.005  & -0.0082  $\pm$ 0.0002  & 1.59E-04 $\pm$ 2.67E-05 \\ 
         & KNN & TRUE & - & 65.21  $\pm$ 2.30  & 566.0  $\pm$ 59.5  & 1.347  $\pm$ 0.090  & -0.0027  $\pm$ 0.0010  & 5.92E-04 $\pm$ 2.69E-06 \\ 
         & - & - & TRUE & 29.78  $\pm$ 0.27  & 9183.0  $\pm$ 198.3  & 1.078  $\pm$ 0.005  & -0.0037  $\pm$ 0.0005  & 1.62E-04 $\pm$ 5.13E-06 \\ 
         & KNN & - & TRUE & 40.40  $\pm$ 0.60  & 2756.2  $\pm$ 70.3  & 1.311  $\pm$ 0.009  & -0.0030  $\pm$ 0.0003  & 3.46E-04 $\pm$ 3.41E-06 \\ 
         & - & TRUE & TRUE & 36.95  $\pm$ 0.40  & 6935.8  $\pm$ 118.9  & 1.058  $\pm$ 0.008  & -0.0073  $\pm$ 0.0008  & 1.89E-04 $\pm$ 1.60E-05 \\ 
         & KNN & TRUE & TRUE & 72.85  $\pm$ 1.82  & 262.4 $\pm$ 28.1  & 1.504  $\pm$ 0.220  & -0.0021  $\pm$ 0.0011  & 7.49E-04 $\pm$ 1.61E-06 \\ 
    \midrule
        \multirow{8}*{159915} 
         & - & - & - & 18.27  $\pm$ 0.12  & 14516.0  $\pm$ 151.8  & 1.028  $\pm$ 0.005  & -0.0055  $\pm$ 0.0003  & 6.63E-05 $\pm$ 6.15E-06 \\ 
         & KNN & - & - & 23.69  $\pm$ 0.33  & 6823.2  $\pm$ 287.8  & 1.176  $\pm$ 0.016  & -0.0042  $\pm$ 0.0005  & 1.30E-04 $\pm$ 1.63E-07 \\ 
         & - & TRUE & - & 30.78  $\pm$ 0.55  & 5941.2  $\pm$ 166.8  & 1.101  $\pm$ 0.009  & -0.0054  $\pm$ 0.0005  & 1.32E-04 $\pm$ 7.31E-05 \\ 
         & KNN & TRUE & - & 53.64  $\pm$ 3.37  & 385.8  $\pm$ 132.7  & 1.847  $\pm$ 0.274  & -0.0014  $\pm$ 0.0009  & 5.41E-04 $\pm$ 3.12E-06 \\ 
         & - & - & TRUE & 20.13  $\pm$ 0.15  & 11259.0  $\pm$ 94.4  & 1.067  $\pm$ 0.004  & -0.0039  $\pm$ 0.0004  & 8.71E-05 $\pm$ 2.43E-06 \\ 
         & KNN & - & TRUE & 26.85  $\pm$ 0.18  & 4130.6  $\pm$ 52.1  & 1.295  $\pm$ 0.008  & -0.0033  $\pm$ 0.0002  & 1.84E-04 $\pm$ 1.04E-06 \\ 
         & - & TRUE & TRUE & 34.76  $\pm$ 0.90  & 4233.8  $\pm$ 250.6  & 1.164  $\pm$ 0.005  & -0.0035  $\pm$ 0.0002  & 1.71E-04 $\pm$ 7.13E-05 \\ 
         & KNN & TRUE & TRUE & 65.02  $\pm$ 3.52  & 110.2  $\pm$ 35.4  & 2.080  $\pm$ 0.071  & -0.0010  $\pm$ 0.0002  & 7.88E-04 $\pm$ 9.45E-06 \\ 
    \bottomrule
    \end{tabular}
    \caption{Ablation experiments with 4 ETFs. Short position in lastprice.}
    \label{tab:ablation-short-position-lastprice}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{c|cc|ccccc}
    \toprule
        Fund & Metric & Semi-Lazy & Precision(\%) & Transactions & Profit-Loss Ratio & Max Drawdown & One-trade Return  \\
    \midrule
        512880 & - & - & 73.28  $\pm$ 0.52  & 1000 $\pm$ 0 & NAN  & -0.0006  $\pm$ 0.0013  & 1.01E-03 $\pm$ 2.20E-05 \\ 
        512880 & TRUE & RNN & 68.66  $\pm$ 0.79  & 1000 $\pm$ 0 & 1.426  $\pm$ 0.068  & -0.0119  $\pm$ 0.0040  & 1.21E-03 $\pm$ 5.90E-05 \\
    \midrule
        512480 & - & - & 69.30  $\pm$ 0.41  & 1000 $\pm$ 0 & 3.218  $\pm$ 0.421  & -0.0043  $\pm$ 0.0014  & 2.08E-03 $\pm$ 4.43E-05 \\ 
        512480 & TRUE & RNN & 80.06  $\pm$ 0.62  & 1000 $\pm$ 0 & 3.644  $\pm$ 0.507  & -0.0078  $\pm$ 0.0014  & 2.36E-03 $\pm$ 5.82E-05 \\ 
    \midrule
        515050 & - & - & 33.04  $\pm$ 0.94  & 1000 $\pm$ 0 & 1.338  $\pm$ 0.102  & -0.0043  $\pm$ 0.0012  & 1.07E-03 $\pm$ 1.82E-05 \\ 
        515050 & TRUE & kNN & 55.36  $\pm$ 1.16  & 1000 $\pm$ 0 & 1.870  $\pm$ 0.085  & -0.0076  $\pm$ 0.0014  & 1.50E-03 $\pm$ 3.01E-05 \\ 
    \midrule
        159915 & - & - & 37.14 $\pm$ 0.45  & 1000 $\pm$ 0 & 2.232  $\pm$ 0.225  & -0.0034  $\pm$ 0.0009  & 1.09E-03 $\pm$ 1.92E-05 \\ 
        159915 & TRUE & KNN & 43.56  $\pm$ 1.17  & 1000 $\pm$ 0 & 2.253  $\pm$ 0.196  & -0.0054  $\pm$ 0.0011  & 1.15E-03 $\pm$ 2.98E-05 \\ 
    \bottomrule
    \end{tabular}
    \caption{Ablation experiments with 4 ETFs. Long position in lastprice condition on maximum 1000 trades.}
    \label{tab:ablation-long-position-lastprice-1000}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{c|cc|ccccc}
    \toprule
        Fund & Metric & Semi-Lazy & Precision(\%) & Transactions & Profit-Loss Ratio & Max Drawdown & One-trade Return  \\
    \midrule
        159915 & - & - & 35.36 $\pm$ 1.40  & 1000 $\pm$ 0 & 2.142  $\pm$ 0.186  & -0.0035  $\pm$ 0.0017  & 1.06E-03 $\pm$ 1.32E-05 \\ 
        159915 & TRUE & KNN & 44.66 $\pm$ 0.78  & 1000 $\pm$ 0 & 1.984  $\pm$ 0.128  & -0.0091  $\pm$ 0.0011  & 1.18E-03 $\pm$ 4.45E-05 \\ 
    \midrule
        512480 & - & - & 70.66 $\pm$ 1.59  & 1000 $\pm$ 0 & 3.298  $\pm$ 0.171  & -0.0038  $\pm$ 0.0008  & 2.01E-03 $\pm$ 3.60E-05 \\ 
        512480 & TRUE & KNN & 76.66 $\pm$ 1.66  & 1000 $\pm$ 0 & 2.779  $\pm$ 0.405  & -0.0102  $\pm$ 0.0031  & 2.21E-03 $\pm$ 8.40E-06 \\ 
    \midrule
        512880 & - & - & 68.52 $\pm$ 0.42  & 1000 $\pm$ 0 & 1.253  $\pm$ 0.251  & -0.0027  $\pm$ 0.0006  & 1.08E-03 $\pm$ 2.54E-05 \\ 
        512880 & TRUE & RNN & 67.2 $\pm$ 1.92  & 1000 $\pm$ 0 & 1.111  $\pm$ 0.061  & -0.0144  $\pm$ 0.0031  & 1.17E-03 $\pm$ 3.18E-05 \\ 
    \midrule
        515050 & - & - & 49.38 $\pm$ 1.14  & 1000 $\pm$ 0 & 1.711  $\pm$ 0.115  & -0.0029  $\pm$ 0.0014  & 1.44E-03 $\pm$ 2.16E-05 \\ 
        515050 & TRUE & KNN & 58.1 $\pm$ 1.15  & 1000 $\pm$ 0 & 1.833  $\pm$ 0.079  & -0.0108  $\pm$ 0.0021  & 1.64E-03 $\pm$ 2.74E-05 \\ 
    \bottomrule
    \end{tabular}
    \caption{Ablation experiments with 4 ETFs. Short position in lastprice condition on maximum 1000 trades.}
    \label{tab:ablation-short-position-lastprice-1000}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{c|cc|ccccc}
    \toprule
        \multirow{2}*{Fund} & \multicolumn{2}{c|}{Semi-Lazy} & \multirow{2}*{Precision(\%)}  & \multirow{2}*{Transactions} & \multirow{2}*{Profit-Loss Ratio} & \multirow{2}*{Max Drawdown} & \multirow{2}*{One-trade Return}  \\
        & Train & Test & & & & &  \\
    \midrule
        \multirow{4}*{512880}
         & train:no & test:no & 53.20  $\pm$ 0.23  & 15760.8  $\pm$ 161.1  & 1.115  $\pm$ 0.015  & -0.0077  $\pm$ 0.0010  & 8.04E-05 $\pm$ 1.86E-06 \\ 
         & train:no & test:yes & 59.22  $\pm$ 1.72  & 1419.0  $\pm$ 272.4  & 1.233  $\pm$ 0.048  & -0.0034  $\pm$ 0.0005  & 4.77E-04 $\pm$ 6.32E-05 \\ 
         & train:yes & test:no & 56.16  $\pm$ 3.17  & 6008.6  $\pm$ 351.7  & 1.163  $\pm$ 0.065  & -0.0293  $\pm$ 0.0135  & 1.86E-04 $\pm$ 1.06E-05 \\ 
         & train:yes & test:yes & 74.95  $\pm$ 2.40  & 467.2  $\pm$ 106.9  & 1.303  $\pm$ 0.163  & -0.0037  $\pm$ 0.0027  & 7.28E-04 $\pm$ 8.01E-05 \\ 
    \midrule
        \multirow{4}*{512480}
         & train:no & test:no & 49.73  $\pm$ 0.30  & 9856.0  $\pm$ 26.4  & 1.185  $\pm$ 0.005  & -0.0046  $\pm$ 0.0002  & 1.55E-04 $\pm$ 1.73E-06 \\ 
         & train:no & test:yes & 52.17  $\pm$ 0.47  & 8237.8  $\pm$ 158.7  & 1.197  $\pm$ 0.008  & -0.0048  $\pm$ 0.0002  & 1.70E-04 $\pm$ 5.10E-06 \\ 
         & train:yes & test:no & 33.19  $\pm$ 11.70  & 3282.4  $\pm$ 1208.6  & 1.326  $\pm$ 0.087  & -0.0167  $\pm$ 0.0048  & 8.79E-05 $\pm$ 8.62E-05 \\ 
         & train:yes & test:yes & 83.79  $\pm$ 1.42  & 634.2  $\pm$ 52.6  & 1.908  $\pm$ 0.060  & -0.0035  $\pm$ 0.0000  & 6.50E-04 $\pm$ 3.81E-05 \\ 
    \midrule
        \multirow{4}*{159915}
         & train:no & test:no & 19.84  $\pm$ 0.06  & 13846.8  $\pm$ 218.6  & 1.013  $\pm$ 0.006  & -0.0042  $\pm$ 0.0000  & 8.23E-05 $\pm$ 1.84E-06 \\ 
         & train:no & test:yes & 24.22  $\pm$ 0.30  & 5289.6  $\pm$ 149.2  & 1.123  $\pm$ 0.011  & -0.0039  $\pm$ 0.0004  & 1.45E-04 $\pm$ 5.51E-06 \\ 
         & train:yes & test:no & 40.86  $\pm$ 5.96  & 1495.0  $\pm$ 719.8  & 1.344  $\pm$ 0.211  & -0.0039  $\pm$ 0.0029  & 3.36E-04 $\pm$ 1.04E-04 \\ 
         & train:yes & test:yes & 48.45  $\pm$ 4.54  & 745.4  $\pm$ 252.5  & 1.501  $\pm$ 0.178  & -0.0019  $\pm$ 0.0005  & 4.52E-04 $\pm$ 7.51E-05 \\ 
    \midrule
        \multirow{4}*{515050}
         & train:no & test:no & 25.21  $\pm$ 0.25  & 15860.2  $\pm$ 313.1  & 1.011  $\pm$ 0.010  & -0.0052  $\pm$ 0.0008  & 9.36E-05 $\pm$ 1.93E-06 \\ 
         & train:no & test:yes & 33.48  $\pm$ 1.45  & 6003.6  $\pm$ 1028.3  & 1.079  $\pm$ 0.047  & -0.0043  $\pm$ 0.0006  & 2.06E-04 $\pm$ 3.63E-05 \\ 
         & train:yes & test:no & 50.14  $\pm$ 1.95  & 1251.4  $\pm$ 206.2  & 1.362  $\pm$ 0.062  & -0.0030  $\pm$ 0.0009  & 5.62E-04 $\pm$ 2.73E-05 \\ 
         & train:yes & test:yes & 56.06  $\pm$ 1.02  & 817.2  $\pm$ 78.4  & 1.374  $\pm$ 0.037  & -0.0026  $\pm$ 0.0006  & 6.42E-04 $\pm$ 1.11E-05 \\ 
    \bottomrule
    \end{tabular}
    \caption{Subset settings. Long position with lastprice.}
    \label{tab:subset-setting-long}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{c|cc|ccccc}
    \toprule
        \multirow{2}*{Fund} & \multicolumn{2}{c|}{Semi-Lazy} & \multirow{2}*{Precision(\%)}  & \multirow{2}*{Transactions} & \multirow{2}*{Profit-Loss Ratio} & \multirow{2}*{Max Drawdown} & \multirow{2}*{One-trade Return}  \\
        & Train & Test & & & & &  \\
    \midrule
        \multirow{4}*{159915}
         & train:no & test:no & 37.14  $\pm$ 0.45  & 1000 $\pm$ 0 & 2.232  $\pm$ 0.225  & -0.0034  $\pm$ 0.0009  & 1.09E-03 $\pm$ 1.92E-05 \\ 
         & train:no & test:yes & 36.92  $\pm$ 1.11  & 1000 $\pm$ 0 & 2.141  $\pm$ 0.085  & -0.0044  $\pm$ 0.0016  & 1.08E-03 $\pm$ 1.90E-05 \\ 
         & train:yes & test:no & 42.88  $\pm$ 3.62  & 1000 $\pm$ 0 & 1.994  $\pm$ 0.307  & -0.0130  $\pm$ 0.0098  & 1.17E-03 $\pm$ 1.06E-04 \\ 
         & train:yes & test:yes & 44.02  $\pm$ 1.60  & 1000 $\pm$ 0 & 2.339  $\pm$ 0.160  & -0.0039  $\pm$ 0.0006  & 1.20E-03 $\pm$ 1.96E-05 \\ 
    \midrule
        \multirow{4}*{512480}
        & train:no & test:no & 69.30  $\pm$ 0.41  & 1000 $\pm$ 0 & 3.218  $\pm$ 0.421  & -0.0043  $\pm$ 0.0014  & 2.08E-03 $\pm$ 4.43E-05 \\ 
         & train:no & test:yes & 70.08  $\pm$ 0.79  & 1000 $\pm$ 0 & 3.088  $\pm$ 0.227  & -0.0049  $\pm$ 0.0002  & 2.11E-03 $\pm$ 5.32E-05 \\ 
         & train:yes & test:no & 38.28  $\pm$ 14.82  & 1000 $\pm$ 0 & 1.813  $\pm$ 0.324  & -0.0573  $\pm$ 0.0543  & 9.11E-04 $\pm$ 6.56E-04 \\ 
         & train:yes & test:yes & 80.50  $\pm$ 0.96  & 1000 $\pm$ 0 & 3.476  $\pm$ 0.318  & -0.0087  $\pm$ 0.0038  & 2.36E-03 $\pm$ 3.48E-05 \\ 
    \midrule
        \multirow{4}*{512880}
         & train:no & test:no & 73.28  $\pm$ 0.52  & 1000 $\pm$ 0 & NAN  & -0.0006  $\pm$ 0.0013  & 1.01E-03 $\pm$ 2.20E-05 \\ 
         & train:no & test:yes & 62.06  $\pm$ 3.16  & 1000 $\pm$ 0 & 1.454  $\pm$ 0.107  & -0.0058  $\pm$ 0.0018  & 1.18E-03 $\pm$ 5.47E-05 \\ 
         & train:yes & test:no & 63.96  $\pm$ 4.84  & 1000 $\pm$ 0 & 0.922  $\pm$ 0.124  & -0.0541  $\pm$ 0.0558  & 1.14E-03 $\pm$ 1.34E-04 \\ 
         & train:yes & test:yes & 68.66  $\pm$ 1.46  & 1000 $\pm$ 0 & 1.437  $\pm$ 0.080  & -0.0101  $\pm$ 0.0047  & 1.20E-03 $\pm$ 4.10E-05 \\ 
    \midrule
        \multirow{4}*{515050}
         & train:no & test:no & 33.04  $\pm$ 0.94  & 1000 $\pm$ 0 & 1.338  $\pm$ 0.102  & -0.0043  $\pm$ 0.0012  & 1.07E-03 $\pm$ 1.82E-05 \\ 
         & train:no & test:yes & 38.40  $\pm$ 0.80  & 1000 $\pm$ 0 & 1.318  $\pm$ 0.044  & -0.0064  $\pm$ 0.0017  & 1.16E-03 $\pm$ 3.40E-05 \\ 
         & train:yes & test:no & 51.56  $\pm$ 0.88  & 1000 $\pm$ 0 & 1.865  $\pm$ 0.061  & -0.0071  $\pm$ 0.0007  & 1.46E-03 $\pm$ 4.00E-05 \\ 
         & train:yes & test:yes & 54.56  $\pm$ 0.90  & 1000 $\pm$ 0 & 1.853  $\pm$ 0.126  & -0.0080  $\pm$ 0.0003  & 1.49E-03 $\pm$ 3.45E-05 \\ 
    \bottomrule
    \end{tabular}
    \caption{Subset settings. Long position with lastprice condition on maximum 1000 trades.}
    \label{tab:subset-setting-long-1000}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{c|cc|ccccc}
    \toprule
        \multirow{2}*{Fund} & \multicolumn{2}{c|}{Semi-Lazy} & \multirow{2}*{Precision(\%)}  & \multirow{2}*{Transactions} & \multirow{2}*{Profit-Loss Ratio} & \multirow{2}*{Max Drawdown} & \multirow{2}*{One-trade Return}  \\
        & Train & Test & & & & &  \\
    \midrule
        \multirow{4}*{159915}
         & train:no & test:no & 18.27  $\pm$ 0.12  & 14516.0  $\pm$ 151.8  & 1.028  $\pm$ 0.005  & -0.0055  $\pm$ 0.0005  & 6.63E-05 $\pm$ 1.63E-07 \\ 
         & train:no & test:yes & 26.19  $\pm$ 0.17  & 4740.8  $\pm$ 107.0  & 1.165  $\pm$ 0.010  & -0.0032  $\pm$ 0.0002  & 1.41E-04 $\pm$ 2.12E-06 \\ 
         & train:yes & test:no & 43.65  $\pm$ 8.04  & 668.4  $\pm$ 239.6  & 1.637  $\pm$ 0.243  & -0.0028  $\pm$ 0.0008  & 4.16E-04 $\pm$ 8.44E-05 \\ 
         & train:yes & test:yes & 52.18  $\pm$ 5.89  & 387.8  $\pm$ 109.0  & 1.883  $\pm$ 0.169  & -0.0013  $\pm$ 0.0006  & 5.19E-04 $\pm$ 5.47E-05 \\ 
    \midrule
        \multirow{4}*{512480}
        & train:no & test:no & 42.93  $\pm$ 0.13  & 10934.8  $\pm$ 125.6  & 1.161  $\pm$ 0.006  & -0.0041  $\pm$ 0.0004  & 1.19E-04 $\pm$ 1.51E-06 \\ 
         & train:no & test:yes & 44.57  $\pm$ 0.27  & 8773.8  $\pm$ 101.8  & 1.157  $\pm$ 0.007  & -0.0044  $\pm$ 0.0003  & 1.34E-04 $\pm$ 1.63E-06 \\ 
         & train:yes & test:no & 29.18  $\pm$ 11.41  & 4600.0  $\pm$ 1374.3  & 1.224  $\pm$ 0.018  & -0.0674  $\pm$ 0.0354  & 1.47E-05 $\pm$ 3.42E-05 \\ 
         & train:yes & test:yes & 77.77  $\pm$ 2.23  & 962.2  $\pm$ 77.1  & 1.692  $\pm$ 0.073  & -0.0026  $\pm$ 0.0003  & 4.10E-04 $\pm$ 9.49E-06 \\ 
    \midrule
        \multirow{4}*{512880}
         & train:no & test:no & 51.72  $\pm$ 0.25  & 16458.2  $\pm$ 181.6  & 0.992  $\pm$ 0.014  & -0.0225  $\pm$ 0.0017  & 7.55E-05 $\pm$ 1.35E-06 \\ 
         & train:no & test:yes & 62.80  $\pm$ 0.44  & 1361.2  $\pm$ 314.5  & 1.150  $\pm$ 0.058  & -0.0069  $\pm$ 0.0017  & 4.91E-04 $\pm$ 7.07E-05 \\ 
         & train:yes & test:no & 54.86  $\pm$ 4.84  & 6394.8  $\pm$ 1533.6  & 1.073  $\pm$ 0.045  & -0.0529  $\pm$ 0.0110  & 1.26E-04 $\pm$ 4.02E-05 \\ 
         & train:yes & test:yes & 72.01  $\pm$ 3.13  & 570.0  $\pm$ 94.0  & 1.102  $\pm$ 0.106  & -0.0059  $\pm$ 0.0029  & 5.92E-04 $\pm$ 3.32E-05 \\ 
    \midrule
        \multirow{4}*{515050}
         & train:no & test:no & 27.71  $\pm$ 0.16  & 11412.2  $\pm$ 109.4  & 1.047  $\pm$ 0.007  & -0.0053  $\pm$ 0.0004  & 1.31E-04 $\pm$ 1.61E-06 \\ 
         & train:no & test:yes & 34.93  $\pm$ 1.64  & 5371.0  $\pm$ 544.6  & 1.074  $\pm$ 0.023  & -0.0037  $\pm$ 0.0003  & 1.87E-04 $\pm$ 1.63E-05 \\ 
         & train:yes & test:no & 58.54  $\pm$ 2.26  & 757.2  $\pm$ 88.3  & 1.313  $\pm$ 0.063  & -0.0050  $\pm$ 0.0036  & 5.42E-04 $\pm$ 4.38E-05 \\ 
         & train:yes & test:yes & 64.07  $\pm$ 1.19  & 560.6  $\pm$ 56.1  & 1.329  $\pm$ 0.061  & -0.0026  $\pm$ 0.0000  & 6.05E-04 $\pm$ 2.44E-05 \\ 
    \bottomrule
    \end{tabular}
    \caption{Subset settings. Short position with lastprice}
    \label{tab:subset-setting-short}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{c|cc|ccccc}
    \toprule
        \multirow{2}*{Fund} & \multicolumn{2}{c|}{Semi-Lazy} & \multirow{2}*{Precision(\%)}  & \multirow{2}*{Transactions} & \multirow{2}*{Profit-Loss Ratio} & \multirow{2}*{Max Drawdown} & \multirow{2}*{One-trade Return}  \\
        & Train & Test & & & & &  \\
    \midrule
        \multirow{4}*{159915}
         & train:no & test:no & 35.36  $\pm$ 1.40  & 1000 $\pm$ 0 & 2.142  $\pm$ 0.186  & -0.0035  $\pm$ 0.0017  & 1.06E-03 $\pm$ 1.32E-05 \\ 
         & train:no & test:yes & 35.32  $\pm$ 0.79  & 1000 $\pm$ 0 & 1.677  $\pm$ 0.121  & -0.0058  $\pm$ 0.0011  & 1.03E-03 $\pm$ 2.42E-05 \\ 
         & train:yes & test:no & 40.86  $\pm$ 4.42  & 1000 $\pm$ 0 & 1.831  $\pm$ 0.201  & -0.0159  $\pm$ 0.0046  & 1.05E-03 $\pm$ 1.41E-04 \\ 
         & train:yes & test:yes & 44.96  $\pm$ 2.98  & 1000 $\pm$ 0 & 1.950  $\pm$ 0.139  & -0.0105  $\pm$ 0.0030  & 1.19E-03 $\pm$ 5.44E-05 \\ 
    \midrule
        \multirow{4}*{512480}
        & train:no & test:no & 71.02  $\pm$ 1.37  & 1000 $\pm$ 0 & 3.298  $\pm$ 0.171  & -0.0038  $\pm$ 0.0008  & 2.01E-03 $\pm$ 3.60E-05 \\ 
         & train:no & test:yes & 70.70  $\pm$ 1.34  & 1000 $\pm$ 0 & 3.266  $\pm$ 0.252  & -0.0038  $\pm$ 0.0015  & 2.01E-03 $\pm$ 5.52E-05 \\ 
         & train:yes & test:no & 39.64  $\pm$ 13.35  & 1000 $\pm$ 0 & 1.467  $\pm$ 0.102  & -0.0874  $\pm$ 0.0386  & 7.61E-04 $\pm$ 4.61E-04 \\ 
         & train:yes & test:yes & 77.26  $\pm$ 1.87  & 1000 $\pm$ 0 & 3.007  $\pm$ 0.535  & -0.0089  $\pm$ 0.0036  & 2.20E-03 $\pm$ 3.05E-05 \\ 
    \midrule
        \multirow{4}*{512880}
         & train:no & test:no & 68.52  $\pm$ 0.42  & 1000 $\pm$ 0 & 1.253  $\pm$ 0.251  & -0.0027  $\pm$ 0.0006  & 1.08E-03 $\pm$ 2.54E-05 \\ 
         & train:no & test:yes & 65.44  $\pm$ 2.37  & 1000 $\pm$ 0 & 1.206  $\pm$ 0.118  & -0.0098  $\pm$ 0.0057  & 1.21E-03 $\pm$ 5.53E-05 \\ 
         & train:yes & test:no & 52.72  $\pm$ 13.22  & 1000 $\pm$ 0 & 0.731  $\pm$ 0.124  & -0.3294  $\pm$ 0.3036  & 8.13E-04 $\pm$ 4.33E-04 \\ 
         & train:yes & test:yes & 67.92  $\pm$ 1.39  & 1000 $\pm$ 0 & 1.065  $\pm$ 0.109  & -0.0144  $\pm$ 0.0023  & 1.16E-03 $\pm$ 5.17E-05 \\ 
    \midrule
        \multirow{4}*{515050}
         & train:no & test:no & 49.38  $\pm$ 1.14  & 1000 $\pm$ 0 & 1.711  $\pm$ 0.115  & -0.0029  $\pm$ 0.0014  & 1.44E-03 $\pm$ 2.16E-05 \\ 
         & train:no & test:yes & 51.32  $\pm$ 0.66  & 1000 $\pm$ 0 & 1.706  $\pm$ 0.224  & -0.0044  $\pm$ 0.0026  & 1.50E-03 $\pm$ 4.51E-05 \\ 
         & train:yes & test:no & 55.10  $\pm$ 2.66  & 1000 $\pm$ 0 & 1.515  $\pm$ 0.232  & -0.0291  $\pm$ 0.0327  & 1.50E-03 $\pm$ 7.74E-05 \\ 
         & train:yes & test:yes & 58.02  $\pm$ 2.07  & 1000 $\pm$ 0 & 1.886  $\pm$ 0.153  & -0.0110  $\pm$ 0.0053  & 1.66E-03 $\pm$ 3.03E-05 \\ 
    \bottomrule
    \end{tabular}
    \caption{Subset settings. Short position with lastprice condition on maximum 1000 trades.}
    \label{tab:subset-setting-short-1000}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{l|l|cc|cc|cc|cc|cc}
    \toprule
        etf & method & Precision(\%) &  & Trans &  & PLR &  & MDD &  & OTR &  \\    
    \midrule
        159915.SZ & ols & 26.22  & 0.06  & 7544.8  & 27.9  & 1.132  & 0.001  & -0.0037  & 0.0002  & 1.46E-04 & 3.10E-07 \\ 
        159915.SZ & gls & 26.22  & 0.06  & 7544.8  & 27.9  & 1.132  & 0.001  & -0.0037  & 0.0002  & 1.46E-04 & 3.10E-07 \\ 
        159915.SZ & glsar & 26.21  & 0.06  & 7544.8  & 28.0  & 1.132  & 0.001  & -0.0037  & 0.0002  & 1.46E-04 & 3.20E-07 \\ 
        159915.SZ & autoreg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E3 & 0.00E3 \\ 
        159915.SZ & arima & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E4 & 0.00E4 \\ 
        159915.SZ & expsmooth & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E5 & 0.00E5 \\ 
        159915.SZ & ets & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E6 & 0.00E6 \\ 
        159915.SZ & linearreg & 26.22  & 0.06  & 7544.8  & 27.9  & 1.132  & 0.001  & -0.0037  & 0.0002  & 1.46E-04 & 3.10E-07 \\ 
        159915.SZ & ridge & 23.86  & 0.02  & 6338.6  & 24.1  & 1.105  & 0.001  & -0.0044  & 0.0000  & 1.38E-04 & 2.66E-07 \\ 
        159915.SZ & lasso & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E9 & 0.00E9 \\ 
        159915.SZ & elasticnet & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E10 & 0.00E10 \\ 
        159915.SZ & lassolars & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E11 & 0.00E11 \\ 
        159915.SZ & bayesianridge & 26.23  & 0.05  & 7547.0  & 24.0  & 1.133  & 0.002  & -0.0038  & 0.0000  & 1.46E-04 & 4.54E-07 \\ 
        159915.SZ & PassiveAggressiveReg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E13 & 0.00E13 \\ 
        159915.SZ & sgdreg & 10.10  & 0.18  & 42550.6  & 1507.8  & 0.944  & 0.006  & -0.0207  & 0.0019  & 6.66E-06 & 5.75E-07 \\ 
        159915.SZ & svr & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E15 & 0.00E15 \\ 
        159915.SZ & mlpreg & 7.55  & 2.08  & 18606.8  & 27532.8  & 1.039  & 0.085  & -0.0230  & 0.0219  & 2.40E-05 & 4.93E-05 \\ 
        159915.SZ & knnreg & 11.53  & 0.04  & 22364.8  & 58.3  & 0.927  & 0.001  & -0.0126  & 0.0006  & 2.42E-05 & 1.95E-07 \\ 
        159915.SZ & adareg & 26.28  & 3.59  & 2260.4  & 893.0  & 1.292  & 0.122  & -0.0056  & 0.0009  & 2.23E-04 & 5.43E-05 \\ 
        159915.SZ & gbreg & 21.15  & 0.55  & 12726.8  & 868.1  & 0.994  & 0.009  & -0.0043  & 0.0001  & 8.76E-05 & 6.53E-06 \\ 
        159915.SZ & baggingreg & 15.33  & 0.12  & 21726.6  & 372.8  & 0.951  & 0.004  & -0.0076  & 0.0011  & 4.05E-05 & 8.98E-07 \\ 
        159915.SZ & extratreereg & 9.89  & 0.15  & 43801.2  & 555.9  & 0.948  & 0.005  & -0.0222  & 0.0010  & 5.51E-06 & 3.27E-07 \\ 
    \midrule
        512480.SH & ols & 46.76  & 0.04  & 15422.4  & 14.5  & 1.021  & 0.001  & -0.0051  & 0.0000  & 9.69E-05 & 1.36E-07 \\ 
        512480.SH & gls & 46.76  & 0.04  & 15422.4  & 14.5  & 1.021  & 0.001  & -0.0051  & 0.0000  & 9.69E-05 & 1.36E-07 \\ 
        512480.SH & glsar & 46.76  & 0.04  & 15422.4  & 14.8  & 1.021  & 0.001  & -0.0051  & 0.0000  & 9.69E-05 & 1.38E-07 \\ 
        512480.SH & autoreg & 0.00  & 0.00  & 0.4  & 0.9  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E26 & 0.00E26 \\ 
        512480.SH & arima & 0.00  & 0.00  & 1.0  & 0.0  &  &  & 0.0000  & 0.0000  & 5.39E-04 & 0.00E27 \\ 
        512480.SH & expsmooth & 3.29  & 7.36  & 16971.4  & 37949.2  & 0.201  & 0.450  & -0.0112  & 0.0251  & 4.90E-07 & 1.10E-06 \\ 
        512480.SH & ets & 3.29  & 7.36  & 16971.4  & 37949.2  & 0.201  & 0.450  & -0.0112  & 0.0251  & 4.90E-07 & 1.10E-06 \\ 
        512480.SH & linearreg & 46.76  & 0.04  & 15422.4  & 14.5  & 1.021  & 0.001  & -0.0051  & 0.0000  & 9.69E-05 & 1.36E-07 \\ 
        512480.SH & ridge & 41.59  & 0.01  & 17724.6  & 8.2  & 1.013  & 0.000  & -0.0065  & 0.0000  & 7.66E-05 & 1.37E-07 \\ 
        512480.SH & lasso & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E32 & 0.00E32 \\ 
        512480.SH & elasticnet & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E33 & 0.00E33 \\ 
        512480.SH & lassolars & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E34 & 0.00E34 \\ 
        512480.SH & bayesianridge & 46.75  & 0.03  & 15427.2  & 10.5  & 1.021  & 0.000  & -0.0051  & 0.0000  & 9.68E-05 & 8.85E-08 \\ 
        512480.SH & PassiveAggressiveReg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E36 & 0.00E36 \\ 
        512480.SH & sgdreg & 24.88  & 0.11  & 42839.0  & 201.1  & 0.951  & 0.004  & -0.0349  & 0.0012  & 9.30E-06 & 4.14E-07 \\ 
        512480.SH & svr & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E38 & 0.00E38 \\ 
        512480.SH & mlpreg & 34.48  & 18.55  & 31566.6  & 28382.0  & 1.107  & 0.245  & -0.0237  & 0.0231  & 1.41E-04 & 2.52E-04 \\ 
        512480.SH & knnreg & 29.77  & 0.07  & 25684.2  & 53.6  & 0.949  & 0.002  & -0.0154  & 0.0007  & 3.25E-05 & 2.80E-07 \\ 
        512480.SH & adareg & 33.28  & 1.50  & 10456.4  & 4150.0  & 1.240  & 0.094  & -0.0091  & 0.0014  & 8.72E-05 & 2.16E-05 \\ 
        512480.SH & gbreg & 43.46  & 0.28  & 18192.4  & 146.3  & 1.001  & 0.007  & -0.0113  & 0.0000  & 8.00E-05 & 1.08E-06 \\ 
        512480.SH & baggingreg & 35.94  & 0.19  & 23447.6  & 201.0  & 0.973  & 0.011  & -0.0124  & 0.0012  & 5.20E-05 & 1.08E-06 \\ 
        512480.SH & extratreereg & 24.43  & 0.03  & 43054.0  & 238.7  & 0.954  & 0.003  & -0.0377  & 0.0014  & 8.09E-06 & 2.77E-07 \\ 
    \bottomrule
    \end{tabular}
    \caption{Baselines. Long position with lastprice.}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{l|l|cc|cc|cc|cc|cc}
    \toprule
        etf & method & Precision(\%) &  & Trans &  & PLR &  & MDD &  & OTR &  \\ 
    \midrule
        512880.SH & ols & 55.07  & 0.05  & 12583.4  & 26.2  & 0.916  & 0.001  & -0.0226  & 0.0000  & 1.34E-04 & 2.89E-07 \\ 
        512880.SH & gls & 55.07  & 0.05  & 12583.4  & 26.2  & 0.916  & 0.001  & -0.0226  & 0.0000  & 1.34E-04 & 2.89E-07 \\ 
        512880.SH & glsar & 55.08  & 0.05  & 12581.8  & 26.2  & 0.916  & 0.001  & -0.0226  & 0.0000  & 1.34E-04 & 2.83E-07 \\ 
        512880.SH & autoreg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E49 & 0.00E49 \\ 
        512880.SH & arima & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E50 & 0.00E50 \\ 
        512880.SH & expsmooth & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E51 & 0.00E51 \\ 
        512880.SH & ets & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E52 & 0.00E52 \\ 
        512880.SH & linearreg & 55.07  & 0.05  & 12583.4  & 26.2  & 0.916  & 0.001  & -0.0226  & 0.0000  & 1.34E-04 & 2.89E-07 \\ 
        512880.SH & ridge & 55.88  & 0.07  & 5641.0  & 26.7  & 0.987  & 0.001  & -0.0210  & 0.0000  & 2.51E-04 & 8.70E-07 \\ 
        512880.SH & lasso & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E55 & 0.00E55 \\ 
        512880.SH & elasticnet & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E56 & 0.00E56 \\ 
        512880.SH & lassolars & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E57 & 0.00E57 \\ 
        512880.SH & bayesianridge & 55.10  & 0.06  & 12569.8  & 22.4  & 0.917  & 0.001  & -0.0226  & 0.0000  & 1.35E-04 & 2.42E-07 \\ 
        512880.SH & PassiveAggressiveReg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E59 & 0.00E59 \\ 
        512880.SH & sgdreg & 35.62  & 0.15  & 45195.8  & 160.4  & 0.987  & 0.003  & -0.0435  & 0.0004  & 8.66E-06 & 1.92E-07 \\ 
        512880.SH & svr & 24.46  & 0.00  & 90317.0  & 0.0  & 1.002  & 0.000  & -0.0437  & 0.0000  & 3.70E-06 & 4.74E-22 \\ 
        512880.SH & mlpreg & 26.75  & 1.87  & 50997.2  & 27141.8  & 1.013  & 0.034  & -0.0435  & 0.0007  & 1.04E-05 & 6.23E-06 \\ 
        512880.SH & knnreg & 31.23  & 0.03  & 16253.2  & 68.9  & 0.932  & 0.001  & -0.0381  & 0.0010  & 3.80E-05 & 4.14E-07 \\ 
        512880.SH & adareg & 44.32  & 3.06  & 9540.8  & 3332.9  & 0.872  & 0.023  & -0.0226  & 0.0043  & 1.17E-04 & 3.42E-05 \\ 
        512880.SH & gbreg & 51.83  & 0.30  & 12790.4  & 38.3  & 0.942  & 0.009  & -0.0164  & 0.0016  & 1.17E-04 & 1.69E-06 \\ 
        512880.SH & baggingreg & 45.10  & 0.29  & 21666.2  & 350.2  & 0.944  & 0.004  & -0.0415  & 0.0022  & 5.17E-05 & 7.41E-07 \\ 
        512880.SH & extratreereg & 35.48  & 0.19  & 45046.4  & 194.8  & 0.986  & 0.007  & -0.0428  & 0.0007  & 8.77E-06 & 2.78E-07 \\ 
    \midrule
        515050.SH & ols & 26.83  & 0.02  & 17709.8  & 24.0  & 0.966  & 0.001  & -0.0074  & 0.0000  & 8.14E-05 & 2.27E-07 \\ 
        515050.SH & gls & 26.83  & 0.02  & 17709.8  & 24.0  & 0.966  & 0.001  & -0.0074  & 0.0000  & 8.14E-05 & 2.27E-07 \\ 
        515050.SH & glsar & 26.83  & 0.03  & 17709.0  & 24.0  & 0.966  & 0.001  & -0.0074  & 0.0000  & 8.14E-05 & 2.29E-07 \\ 
        515050.SH & autoreg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E72 & 0.00E72 \\ 
        515050.SH & arima & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E73 & 0.00E73 \\ 
        515050.SH & expsmooth & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E74 & 0.00E74 \\ 
        515050.SH & ets & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E75 & 0.00E75 \\ 
        515050.SH & linearreg & 26.83  & 0.02  & 17709.8  & 24.0  & 0.966  & 0.001  & -0.0074  & 0.0000  & 8.14E-05 & 2.27E-07 \\ 
        515050.SH & ridge & 23.72  & 0.01  & 16725.0  & 22.0  & 0.988  & 0.000  & -0.0093  & 0.0000  & 7.32E-05 & 1.83E-07 \\ 
        515050.SH & lasso & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E78 & 0.00E78 \\ 
        515050.SH & elasticnet & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E79 & 0.00E79 \\ 
        515050.SH & lassolars & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E80 & 0.00E80 \\ 
        515050.SH & bayesianridge & 26.86  & 0.02  & 17685.6  & 24.9  & 0.966  & 0.001  & -0.0074  & 0.0000  & 8.16E-05 & 1.68E-07 \\ 
        515050.SH & PassiveAggressiveReg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E82 & 0.00E82 \\ 
        515050.SH & sgdreg & 13.94  & 0.08  & 50003.0  & 381.8  & 0.975  & 0.001  & -0.0425  & 0.0029  & 5.36E-06 & 2.21E-07 \\ 
        515050.SH & svr & 9.51  & 0.00  & 92417.0  & 0.0  & 1.001  & 0.000  & -0.0550  & 0.0000  & 1.94E-06 & 0.00E84 \\ 
        515050.SH & mlpreg & 16.01  & 4.13  & 23367.4  & 23633.4  & 1.029  & 0.061  & -0.0206  & 0.0112  & 7.48E-05 & 9.33E-05 \\ 
        515050.SH & knnreg & 14.60  & 0.02  & 33695.8  & 36.9  & 0.969  & 0.000  & -0.0208  & 0.0014  & 1.78E-05 & 1.02E-07 \\ 
        515050.SH & adareg & 26.38  & 6.40  & 12238.8  & 8152.6  & 1.023  & 0.044  & -0.0079  & 0.0019  & 1.24E-04 & 8.51E-05 \\ 
        515050.SH & gbreg & 23.00  & 0.09  & 24235.6  & 117.0  & 0.971  & 0.002  & -0.0077  & 0.0004  & 5.09E-05 & 4.17E-07 \\ 
        515050.SH & baggingreg & 18.54  & 0.11  & 32801.2  & 404.2  & 0.961  & 0.002  & -0.0143  & 0.0007  & 2.45E-05 & 6.37E-07 \\ 
        515050.SH & extratreereg & 13.95  & 0.10  & 48740.2  & 232.0  & 0.977  & 0.004  & -0.0475  & 0.0050  & 5.36E-06 & 1.82E-07 \\ 
    \bottomrule
    \end{tabular}
    \caption{Baselines. Long position with lastprice.}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{l|l|cc|cc|cc|cc|cc}
    \toprule
        etf & method & Precision(\%) &  & Trans &  & PLR &  & MDD &  & OTR &  \\ 
    \midrule
        159915.SZ & ols & 24.24  & 0.02  & 9000.6  & 13.7  & 1.094  & 0.000  & -0.0041  & 0.0001  & 1.11E-04 & 3.00E-07 \\ 
        159915.SZ & gls & 24.24  & 0.02  & 9000.6  & 13.7  & 1.094  & 0.000  & -0.0041  & 0.0001  & 1.11E-04 & 3.00E-07 \\ 
        159915.SZ & glsar & 24.24  & 0.02  & 8999.0  & 14.2  & 1.093  & 0.000  & -0.0041  & 0.0001  & 1.11E-04 & 3.14E-07 \\ 
        159915.SZ & autoreg & 0.00  & 0.00  & 3.0  & 0.0  & 3.000  & 0.000  & -0.0005  & 0.0000  & 8.20E-04 & 0.00E3 \\ 
        159915.SZ & arima & 0.00  & 0.00  & 3.0  & 0.0  & 3.000  & 0.000  & -0.0005  & 0.0000  & 8.20E-04 & 0.00E4 \\ 
        159915.SZ & expsmooth & 5.89  & 0.00  & 87521.0  & 0.0  & 1.007  & 0.000  & -0.1645  & 0.0000  & -1.82E-06 & 0.00E5 \\ 
        159915.SZ & ets & 5.89  & 0.00  & 87521.0  & 0.0  & 1.007  & 0.000  & -0.1645  & 0.0000  & -1.82E-06 & 0.00E6 \\ 
        159915.SZ & linearreg & 24.24  & 0.02  & 9000.6  & 13.7  & 1.094  & 0.000  & -0.0041  & 0.0001  & 1.11E-04 & 3.00E-07 \\ 
        159915.SZ & ridge & 23.40  & 0.04  & 8025.0  & 15.0  & 1.086  & 0.001  & -0.0048  & 0.0000  & 1.04E-04 & 1.84E-07 \\ 
        159915.SZ & lasso & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E9 & 0.00E9 \\ 
        159915.SZ & elasticnet & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E10 & 0.00E10 \\ 
        159915.SZ & lassolars & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E11 & 0.00E11 \\ 
        159915.SZ & bayesianridge & 24.23  & 0.02  & 9004.0  & 12.6  & 1.094  & 0.001  & -0.0041  & 0.0001  & 1.11E-04 & 1.27E-07 \\ 
        159915.SZ & PassiveAggressiveReg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E13 & 0.00E13 \\ 
        159915.SZ & sgdreg & 9.04  & 0.21  & 44970.4  & 1507.8  & 0.950  & 0.004  & -0.0912  & 0.0133  & -1.39E-06 & 2.12E-07 \\ 
        159915.SZ & svr & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E15 & 0.00E15 \\ 
        159915.SZ & mlpreg & 7.62  & 2.43  & 54183.8  & 38045.8  & 1.025  & 0.077  & -0.1040  & 0.0817  & 1.14E-05 & 2.34E-05 \\ 
        159915.SZ & knnreg & 11.32  & 0.01  & 19765.8  & 28.0  & 0.943  & 0.001  & -0.0204  & 0.0003  & 1.68E-05 & 2.20E-07 \\ 
        159915.SZ & adareg & 44.09  & 26.11  & 85.0  & 131.2  & 2.828  & 0.833  & -0.0006  & 0.0004  & 7.89E-04 & 2.86E-04 \\ 
        159915.SZ & gbreg & 18.97  & 0.22  & 15020.0  & 438.9  & 1.001  & 0.002  & -0.0053  & 0.0002  & 6.06E-05 & 2.06E-06 \\ 
        159915.SZ & baggingreg & 13.92  & 0.13  & 23344.2  & 488.4  & 0.955  & 0.002  & -0.0094  & 0.0005  & 2.69E-05 & 1.14E-06 \\ 
        159915.SZ & extratreereg & 9.01  & 0.10  & 43719.8  & 555.9  & 0.953  & 0.001  & -0.1052  & 0.0067  & -2.03E-06 & 2.07E-07 \\ 
    \midrule
        512480.SH & ols & 36.43  & 0.02  & 14862.8  & 24.4  & 1.102  & 0.001  & -0.0335  & 0.0000  & 8.54E-05 & 1.45E-07 \\ 
        512480.SH & gls & 36.43  & 0.02  & 14862.8  & 24.4  & 1.102  & 0.001  & -0.0335  & 0.0000  & 8.54E-05 & 1.45E-07 \\ 
        512480.SH & glsar & 36.43  & 0.02  & 14862.4  & 24.1  & 1.102  & 0.001  & -0.0335  & 0.0000  & 8.54E-05 & 1.43E-07 \\ 
        512480.SH & autoreg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E26 & 0.00E26 \\ 
        512480.SH & arima & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E27 & 0.00E27 \\ 
        512480.SH & expsmooth & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E28 & 0.00E28 \\ 
        512480.SH & ets & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E29 & 0.00E29 \\ 
        512480.SH & linearreg & 36.43  & 0.02  & 14862.8  & 24.4  & 1.102  & 0.001  & -0.0335  & 0.0000  & 8.54E-05 & 1.45E-07 \\ 
        512480.SH & ridge & 34.33  & 0.02  & 16258.6  & 31.2  & 1.055  & 0.001  & -0.0208  & 0.0002  & 7.28E-05 & 1.26E-07 \\ 
        512480.SH & lasso & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E32 & 0.00E32 \\ 
        512480.SH & elasticnet & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E33 & 0.00E33 \\ 
        512480.SH & lassolars & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E34 & 0.00E34 \\ 
        512480.SH & bayesianridge & 36.45  & 0.03  & 14862.0  & 28.2  & 1.102  & 0.002  & -0.0334  & 0.0002  & 8.54E-05 & 2.07E-07 \\ 
        512480.SH & PassiveAggressiveReg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E36 & 0.00E36 \\ 
        512480.SH & sgdreg & 21.82  & 0.05  & 42018.0  & 201.1  & 0.907  & 0.005  & -0.0892  & 0.0046  & -2.62E-07 & 1.75E-07 \\ 
        512480.SH & svr & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E38 & 0.00E38 \\ 
        512480.SH & mlpreg & 22.67  & 5.13  & 32326.4  & 32131.2  & 1.158  & 0.320  & -0.0595  & 0.0823  & 7.34E-05 & 1.11E-04 \\ 
        512480.SH & knnreg & 25.75  & 0.05  & 24292.0  & 50.1  & 0.906  & 0.002  & -0.0289  & 0.0007  & 2.40E-05 & 2.25E-07 \\ 
        512480.SH & adareg & 63.36  & 10.57  & 1794.2  & 1318.4  & 1.444  & 0.252  & -0.0041  & 0.0009  & 3.54E-04 & 1.53E-04 \\ 
        512480.SH & gbreg & 37.76  & 0.16  & 15859.8  & 101.5  & 1.022  & 0.005  & -0.0130  & 0.0010  & 7.93E-05 & 9.46E-07 \\ 
        512480.SH & baggingreg & 31.99  & 0.17  & 20288.2  & 111.6  & 0.970  & 0.008  & -0.0249  & 0.0024  & 5.31E-05 & 6.74E-07 \\ 
        512480.SH & extratreereg & 21.58  & 0.15  & 41803.0  & 238.7  & 0.914  & 0.003  & -0.1018  & 0.0179  & -1.21E-06 & 3.30E-07 \\ 
    \bottomrule
    \end{tabular}
    \caption{Baselines. Short position with lastprice.}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{l|l|cc|cc|cc|cc|cc}
    \toprule
        etf & method & Precision(\%) &  & Trans &  & PLR &  & MDD &  & OTR &  \\ 
    \midrule
        512880.SH & ols & 48.93  & 0.03  & 13371.8  & 13.9  & 0.953  & 0.002  & -0.0732  & 0.0007  & 9.37E-05 & 1.51E-07 \\ 
        512880.SH & gls & 48.93  & 0.03  & 13371.8  & 13.9  & 0.953  & 0.002  & -0.0732  & 0.0007  & 9.37E-05 & 1.51E-07 \\ 
        512880.SH & glsar & 48.92  & 0.03  & 13373.4  & 14.2  & 0.953  & 0.002  & -0.0732  & 0.0007  & 9.37E-05 & 1.83E-07 \\ 
        512880.SH & autoreg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E49 & 0.00E49 \\ 
        512880.SH & arima & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E50 & 0.00E50 \\ 
        512880.SH & expsmooth & 4.54  & 10.15  & 3612.6  & 8078.0  & 0.197  & 0.441  & -0.0668  & 0.1493  & -3.64E-06 & 8.13E-06 \\ 
        512880.SH & ets & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E52 & 0.00E52 \\ 
        512880.SH & linearreg & 48.93  & 0.03  & 13371.8  & 13.9  & 0.953  & 0.002  & -0.0732  & 0.0007  & 9.37E-05 & 1.51E-07 \\ 
        512880.SH & ridge & 48.30  & 0.06  & 5384.6  & 19.7  & 0.962  & 0.002  & -0.0382  & 0.0000  & 1.96E-04 & 4.43E-07 \\ 
        512880.SH & lasso & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E55 & 0.00E55 \\ 
        512880.SH & elasticnet & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E56 & 0.00E56 \\ 
        512880.SH & lassolars & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E57 & 0.00E57 \\ 
        512880.SH & bayesianridge & 48.95  & 0.04  & 13369.2  & 13.3  & 0.955  & 0.002  & -0.0728  & 0.0007  & 9.40E-05 & 1.85E-07 \\ 
        512880.SH & PassiveAggressiveReg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E59 & 0.00E59 \\ 
        512880.SH & sgdreg & 33.49  & 0.22  & 45121.2  & 160.4  & 0.964  & 0.003  & -0.2946  & 0.0045  & -5.78E-06 & 2.07E-07 \\ 
        512880.SH & svr & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E61 & 0.00E61 \\ 
        512880.SH & mlpreg & 27.03  & 3.77  & 21329.2  & 24622.4  & 0.977  & 0.043  & -0.1939  & 0.0886  & -5.60E-06 & 2.75E-05 \\ 
        512880.SH & knnreg & 27.98  & 0.06  & 14348.4  & 66.6  & 0.904  & 0.002  & -0.1289  & 0.0048  & 3.09E-06 & 4.94E-07 \\ 
        512880.SH & adareg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E64 & 0.00E64 \\ 
        512880.SH & gbreg & 45.82  & 0.39  & 15410.0  & 236.6  & 0.958  & 0.004  & -0.1283  & 0.0020  & 7.18E-05 & 1.10E-06 \\ 
        512880.SH & baggingreg & 43.12  & 0.42  & 19097.4  & 203.2  & 0.910  & 0.005  & -0.0927  & 0.0122  & 3.73E-05 & 2.14E-06 \\ 
        512880.SH & extratreereg & 33.22  & 0.17  & 45270.6  & 194.8  & 0.965  & 0.007  & -0.3008  & 0.0046  & -6.04E-06 & 1.50E-07 \\ 
    \midrule
        515050.SH & ols & 25.21  & 0.01  & 15068.2  & 2.2  & 0.986  & 0.000  & -0.0088  & 0.0000  & 9.28E-05 & 1.44E-07 \\ 
        515050.SH & gls & 25.21  & 0.01  & 15068.2  & 2.2  & 0.986  & 0.000  & -0.0088  & 0.0000  & 9.28E-05 & 1.44E-07 \\ 
        515050.SH & glsar & 25.21  & 0.00  & 15068.6  & 2.5  & 0.986  & 0.000  & -0.0088  & 0.0000  & 9.28E-05 & 1.41E-07 \\ 
        515050.SH & autoreg & 0.00  & 0.00  & 9.0  & 0.0  & 0.999  & 0.000  & -0.0009  & 0.0000  & 1.02E-04 & 0.00E72 \\ 
        515050.SH & arima & 0.00  & 0.00  & 5.0  & 0.0  & 1.499  & 0.000  & -0.0009  & 0.0000  & 1.84E-04 & 0.00E73 \\ 
        515050.SH & expsmooth & 7.88  & 0.00  & 92417.0  & 0.0  & 0.999  & 0.000  & -0.1887  & 0.0000  & -1.94E-06 & 0.00E74 \\ 
        515050.SH & ets & 7.88  & 0.00  & 92417.0  & 0.0  & 0.999  & 0.000  & -0.1887  & 0.0000  & -1.94E-06 & 0.00E75 \\ 
        515050.SH & linearreg & 25.21  & 0.01  & 15068.2  & 2.2  & 0.986  & 0.000  & -0.0088  & 0.0000  & 9.28E-05 & 1.44E-07 \\ 
        515050.SH & ridge & 22.04  & 0.01  & 14555.2  & 11.0  & 0.985  & 0.000  & -0.0096  & 0.0000  & 7.52E-05 & 1.23E-07 \\ 
        515050.SH & lasso & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E78 & 0.00E78 \\ 
        515050.SH & elasticnet & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E79 & 0.00E79 \\ 
        515050.SH & lassolars & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E80 & 0.00E80 \\ 
        515050.SH & bayesianridge & 25.22  & 0.02  & 15071.8  & 6.9  & 0.987  & 0.001  & -0.0088  & 0.0000  & 9.28E-05 & 9.12E-08 \\ 
        515050.SH & PassiveAggressiveReg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E82 & 0.00E82 \\ 
        515050.SH & sgdreg & 13.12  & 0.08  & 42414.0  & 381.8  & 0.963  & 0.002  & -0.0963  & 0.0056  & -1.28E-06 & 2.19E-07 \\ 
        515050.SH & svr & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E84 & 0.00E84 \\ 
        515050.SH & mlpreg & 11.98  & 4.56  & 47846.8  & 32086.8  & 0.993  & 0.010  & -0.1122  & 0.0800  & 1.87E-05 & 3.32E-05 \\ 
        515050.SH & knnreg & 13.60  & 0.02  & 27247.2  & 29.4  & 0.954  & 0.001  & -0.0240  & 0.0000  & 1.49E-05 & 2.08E-07 \\ 
        515050.SH & adareg & 42.21  & 5.05  & 922.4  & 345.8  & 1.161  & 0.029  & -0.0039  & 0.0010  & 3.40E-04 & 4.14E-05 \\ 
        515050.SH & gbreg & 21.94  & 0.14  & 19902.2  & 158.1  & 0.977  & 0.001  & -0.0085  & 0.0005  & 6.03E-05 & 8.53E-07 \\ 
        515050.SH & baggingreg & 18.98  & 0.09  & 24368.4  & 218.1  & 0.964  & 0.003  & -0.0159  & 0.0023  & 3.59E-05 & 1.38E-06 \\ 
        515050.SH & extratreereg & 12.64  & 0.10  & 43676.8  & 232.0  & 0.967  & 0.003  & -0.1099  & 0.0040  & -1.83E-06 & 1.27E-07 \\ 
    \bottomrule
    \end{tabular}
    \caption{Baselines. Short position with lastprice.}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{l|l|cc|cc|cc|cc|cc}
    \toprule
        etf & method & Precision(\%) &  & Trans &  & PLR &  & MDD &  & OTR &  \\ 
    \midrule
        159915.SZ & ols & 43.12  & 0.04  & 1000 & 0 & 2.1372  & 0.0057  & -0.0082  & 0.0000  & 1.17E-03 & 1.87E-06 \\ 
        159915.SZ & gls & 43.12  & 0.04  & 1000 & 0 & 2.1372  & 0.0057  & -0.0082  & 0.0000  & 1.17E-03 & 1.87E-06 \\ 
        159915.SZ & glsar & 43.12  & 0.04  & 1000 & 0 & 2.1364  & 0.0062  & -0.0082  & 0.0000  & 1.17E-03 & 1.52E-06 \\ 
        159915.SZ & autoreg & 4.56  & 0.05  & 1000 & 0 & 2.1809  & 0.0502  & -0.0426  & 0.0000  & 1.03E-03 & 5.72E-05 \\ 
        159915.SZ & arima & 5.60  & 0.00  & 1000 & 0 & 4.2400  & 0.0000  & -0.0426  & 0.0000  & 1.81E-03 & 2.42E-19 \\ 
        159915.SZ & expsmooth & 5.08  & 0.41  & 1000 & 0 & 0.7414  & 0.1822  & -0.6880  & 0.3254  & -8.45E-04 & 7.59E-04 \\ 
        159915.SZ & ets & 5.60  & 0.00  & 1000 & 0 & 4.1275  & 0.0000  & -0.0426  & 0.0000  & 1.81E-03 & 2.42E-19 \\ 
        159915.SZ & linearreg & 43.12  & 0.04  & 1000 & 0 & 2.1372  & 0.0057  & -0.0082  & 0.0000  & 1.17E-03 & 1.87E-06 \\ 
        159915.SZ & ridge & 43.12  & 0.15  & 1000 & 0 & 2.0517  & 0.0144  & -0.0058  & 0.0000  & 1.01E-03 & 1.99E-06 \\ 
        159915.SZ & lasso & 5.60  & 0.00  & 1000 & 0 & 4.1275  & 0.0000  & -0.0426  & 0.0000  & 1.81E-03 & 2.42E-19 \\ 
        159915.SZ & elasticnet & 5.60  & 0.00  & 1000 & 0 & 4.1275  & 0.0000  & -0.0426  & 0.0000  & 1.81E-03 & 2.42E-19 \\ 
        159915.SZ & lassolars & 5.60  & 0.00  & 1000 & 0 & 4.1275  & 0.0000  & -0.0426  & 0.0000  & 1.81E-03 & 2.42E-19 \\ 
        159915.SZ & bayesianridge & 43.12  & 0.15  & 1000 & 0 & 2.1256  & 0.0084  & -0.0082  & 0.0000  & 1.17E-03 & 2.96E-06 \\ 
        159915.SZ & PassiveAggressiveReg & 5.60  & 0.00  & 1000 & 0 & 4.1275  & 0.0000  & -0.0426  & 0.0000  & 1.81E-03 & 2.42E-19 \\ 
        159915.SZ & sgdreg & 16.66  & 2.13  & 1000 & 0 & 1.2974  & 0.0643  & -0.0134  & 0.0062  & 4.45E-04 & 4.23E-05 \\ 
        159915.SZ & svr & 5.60  & 0.00  & 1000 & 0 & 4.1275  & 0.0000  & -0.0426  & 0.0000  & 1.81E-03 & 2.42E-19 \\ 
        159915.SZ & mlpreg & 10.76  & 6.64  & 1000 & 0 & 1.1547  & 0.3050  & -0.0769  & 0.0643  & 2.80E-04 & 2.58E-04 \\ 
        159915.SZ & knnreg & 15.46  & 0.65  & 1000 & 0 & 1.3749  & 0.0204  & -0.0111  & 0.0020  & 4.57E-04 & 8.90E-06 \\ 
        159915.SZ & adareg & 29.16  & 2.94  & 1000 & 0 & 1.6978  & 0.1872  & -0.0303  & 0.0110  & 8.30E-04 & 1.20E-04 \\ 
        159915.SZ & gbreg & 43.86  & 0.47  & 1000 & 0 & 2.4976  & 0.1110  & -0.0029  & 0.0006  & 1.21E-03 & 2.40E-05 \\ 
        159915.SZ & baggingreg & 30.88  & 0.68  & 1000 & 0 & 1.9799  & 0.1016  & -0.0046  & 0.0008  & 9.03E-04 & 2.88E-05 \\ 
        159915.SZ & extratreereg & 14.20  & 1.12  & 1000 & 0 & 1.3437  & 0.1231  & -0.0113  & 0.0056  & 3.69E-04 & 6.61E-05 \\ 
    \midrule
        512480.SH & ols & 81.66  & 0.09  & 1000 & 0 & 2.7672  & 0.0023  & -0.0127  & 0.0000  & 2.44E-03 & 2.07E-06 \\ 
        512480.SH & gls & 81.66  & 0.09  & 1000 & 0 & 2.7672  & 0.0023  & -0.0127  & 0.0000  & 2.44E-03 & 2.07E-06 \\ 
        512480.SH & glsar & 81.66  & 0.09  & 1000 & 0 & 2.7672  & 0.0023  & -0.0127  & 0.0000  & 2.44E-03 & 2.07E-06 \\ 
        512480.SH & autoreg & 12.18  & 0.18  & 1000 & 0 & 1.0136  & 0.0109  & -1.0000  & 0.0000  & -1.31E-03 & 3.70E-05 \\ 
        512480.SH & arima & 23.52  & 1.03  & 1000 & 0 & 3.3989  & 0.3367  & -0.5926  & 0.1409  & 3.32E-03 & 4.84E-04 \\ 
        512480.SH & expsmooth & 18.28  & 1.39  & 1000 & 0 & 2.6570  & 1.8237  & -0.5443  & 0.0774  & 3.35E-03 & 1.14E-03 \\ 
        512480.SH & ets & 5.20  & 0.00  & 1000 & 0 & 0.2635  & 0.0000  & -1.0000  & 0.0000  & -1.75E-03 & 2.42E-19 \\ 
        512480.SH & linearreg & 81.66  & 0.09  & 1000 & 0 & 2.7672  & 0.0023  & -0.0127  & 0.0000  & 2.44E-03 & 2.07E-06 \\ 
        512480.SH & ridge & 81.64  & 0.15  & 1000 & 0 & 3.9930  & 0.0136  & -0.0031  & 0.0000  & 2.15E-03 & 2.75E-06 \\ 
        512480.SH & lasso & 5.20  & 0.00  & 1000 & 0 & 0.2635  & 0.0000  & -1.0000  & 0.0000  & -1.75E-03 & 2.42E-19 \\ 
        512480.SH & elasticnet & 5.20  & 0.00  & 1000 & 0 & 0.2635  & 0.0000  & -1.0000  & 0.0000  & -1.75E-03 & 2.42E-19 \\ 
        512480.SH & lassolars & 5.20  & 0.00  & 1000 & 0 & 0.2635  & 0.0000  & -1.0000  & 0.0000  & -1.75E-03 & 2.42E-19 \\ 
        512480.SH & bayesianridge & 81.64  & 0.15  & 1000 & 0 & 2.6740  & 0.2132  & -0.0127  & 0.0000  & 2.44E-03 & 7.26E-06 \\ 
        512480.SH & PassiveAggressiveReg & 5.20  & 0.00  & 1000 & 0 & 0.2635  & 0.0000  & -1.0000  & 0.0000  & -1.75E-03 & 2.42E-19 \\ 
        512480.SH & sgdreg & 35.60  & 1.43  & 1000 & 0 & 1.7419  & 0.0873  & -0.0190  & 0.0031  & 9.09E-04 & 5.66E-05 \\ 
        512480.SH & svr & 5.20  & 0.00  & 1000 & 0 & 0.2635  & 0.0000  & -1.0000  & 0.0000  & -1.75E-03 & 2.42E-19 \\ 
        512480.SH & mlpreg & 50.62  & 15.99  & 1000 & 0 & 2.0782  & 0.5923  & -0.0374  & 0.0255  & 1.34E-03 & 5.30E-04 \\ 
        512480.SH & knnreg & 42.28  & 0.31  & 1000 & 0 & 2.2000  & 0.0374  & -0.0129  & 0.0002  & 1.11E-03 & 1.39E-05 \\ 
        512480.SH & adareg & 36.22  & 4.55  & 1000 & 0 & 2.1746  & 0.2690  & -0.0192  & 0.0062  & 1.02E-03 & 1.53E-04 \\ 
        512480.SH & gbreg & 79.62  & 0.36  & 1000 & 0 & 2.9550  & 0.0574  & -0.0176  & 0.0003  & 2.43E-03 & 2.11E-05 \\ 
        512480.SH & baggingreg & 66.28  & 1.54  & 1000 & 0 & 2.7310  & 0.2925  & -0.0120  & 0.0028  & 2.05E-03 & 7.20E-05 \\ 
        512480.SH & extratreereg & 35.88  & 2.27  & 1000 & 0 & 1.8200  & 0.0979  & -0.0202  & 0.0068  & 9.16E-04 & 1.09E-04 \\ 
    \bottomrule
    \end{tabular}
    \caption{Baselines. Long position with lastprice condition on 1000 trades.}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{l|l|cc|cc|cc|cc|cc}
    \toprule
        etf & method & Precision(\%) &  & Trans &  & PLR &  & MDD &  & OTR &  \\ 
    \midrule
        512880.SH & ols & 64.44  & 0.11  & 1000 & 0 & 0.9941  & 0.0142  & -0.2227  & 0.0000  & 1.77E-03 & 1.12E-05 \\ 
        512880.SH & gls & 64.44  & 0.11  & 1000 & 0 & 0.9941  & 0.0142  & -0.2227  & 0.0000  & 1.77E-03 & 1.12E-05 \\ 
        512880.SH & glsar & 64.48  & 0.13  & 1000 & 0 & 0.9956  & 0.0150  & -0.2227  & 0.0000  & 1.77E-03 & 1.10E-05 \\ 
        512880.SH & autoreg & 14.22  & 6.36  & 1000 & 0 & 1.1171  & 0.2154  & -0.3160  & 0.1341  & -3.63E-05 & 1.66E-04 \\ 
        512880.SH & arima & 8.88  & 0.18  & 1000 & 0 & 1.6555  & 0.1214  & -0.1844  & 0.0619  & 8.40E-04 & 1.33E-04 \\ 
        512880.SH & expsmooth & 22.86  & 3.68  & 1000 & 0 & 1.8316  & 1.7105  & -0.5141  & 0.3316  & 6.51E-04 & 1.73E-03 \\ 
        512880.SH & ets & 8.70  & 0.00  & 1000 & 0 & 1.6028  & 0.0000  & -0.2121  & 0.0000  & 7.77E-04 & 0.00E52 \\ 
        512880.SH & linearreg & 64.44  & 0.11  & 1000 & 0 & 0.9941  & 0.0142  & -0.2227  & 0.0000  & 1.77E-03 & 1.12E-05 \\ 
        512880.SH & ridge & 64.58  & 0.13  & 1000 & 0 & 1.3660  & 0.0050  & -0.0796  & 0.0000  & 1.87E-03 & 8.92E-06 \\ 
        512880.SH & lasso & 8.70  & 0.00  & 1000 & 0 & 1.6028  & 0.0000  & -0.2121  & 0.0000  & 7.77E-04 & 0.00E55 \\ 
        512880.SH & elasticnet & 8.70  & 0.00  & 1000 & 0 & 1.6028  & 0.0000  & -0.2121  & 0.0000  & 7.77E-04 & 0.00E56 \\ 
        512880.SH & lassolars & 8.70  & 0.00  & 1000 & 0 & 1.6028  & 0.0000  & -0.2121  & 0.0000  & 7.77E-04 & 0.00E57 \\ 
        512880.SH & bayesianridge & 64.58  & 0.13  & 1000 & 0 & 0.9545  & 0.0025  & -0.2320  & 0.0000  & 1.81E-03 & 4.90E-06 \\ 
        512880.SH & PassiveAggressiveReg & 8.70  & 0.00  & 1000 & 0 & 1.6028  & 0.0000  & -0.2121  & 0.0000  & 7.77E-04 & 0.00E59 \\ 
        512880.SH & sgdreg & 38.84  & 2.72  & 1000 & 0 & 1.1832  & 0.2335  & -0.1201  & 0.0752  & 1.01E-03 & 2.34E-04 \\ 
        512880.SH & svr & 8.70  & 0.00  & 1000 & 0 & 1.6028  & 0.0000  & -0.2121  & 0.0000  & 7.77E-04 & 0.00E61 \\ 
        512880.SH & mlpreg & 37.24  & 6.25  & 1000 & 0 & 0.9113  & 0.5415  & -0.8354  & 0.2327  & 4.14E-04 & 1.35E-03 \\ 
        512880.SH & knnreg & 40.20  & 0.49  & 1000 & 0 & 1.3210  & 0.0653  & -0.0625  & 0.0058  & 9.42E-04 & 5.76E-05 \\ 
        512880.SH & adareg & 46.36  & 6.06  & 1000 & 0 & 1.2094  & 0.2200  & -0.1725  & 0.0299  & 1.42E-03 & 4.98E-04 \\ 
        512880.SH & gbreg & 47.62  & 1.02  & 1000 & 0 & 1.3313  & 0.1198  & -0.0826  & 0.0188  & 1.48E-03 & 7.78E-05 \\ 
        512880.SH & baggingreg & 47.54  & 1.30  & 1000 & 0 & 1.3653  & 0.1042  & -0.0793  & 0.0217  & 1.55E-03 & 1.74E-04 \\ 
        512880.SH & extratreereg & 39.00  & 3.07  & 1000 & 0 & 1.3188  & 0.1772  & -0.1472  & 0.0730  & 1.03E-03 & 3.14E-04 \\ 
    \midrule
        515050.SH & ols & 55.22  & 0.08  & 1000 & 0 & 1.6669  & 0.0042  & -0.0081  & 0.0000  & 1.47E-03 & 4.01E-06 \\ 
        515050.SH & gls & 55.22  & 0.08  & 1000 & 0 & 1.6669  & 0.0042  & -0.0081  & 0.0000  & 1.47E-03 & 4.01E-06 \\ 
        515050.SH & glsar & 55.24  & 0.05  & 1000 & 0 & 1.6709  & 0.0053  & -0.0081  & 0.0000  & 1.47E-03 & 9.99E-07 \\ 
        515050.SH & autoreg & 11.16  & 0.35  & 1000 & 0 & 3.2722  & 0.1903  & -0.0184  & 0.0146  & 2.75E-03 & 2.55E-04 \\ 
        515050.SH & arima & 11.50  & 0.00  & 1000 & 0 & 2.9546  & 0.0000  & -0.0324  & 0.0000  & 2.49E-03 & 0.00E73 \\ 
        515050.SH & expsmooth & 8.08  & 1.29  & 1000 & 0 & 1.4976  & 0.6174  & -0.6688  & 0.3679  & 8.82E-04 & 1.13E-03 \\ 
        515050.SH & ets & 11.40  & 0.00  & 1000 & 0 & 2.8859  & 0.0000  & -0.0324  & 0.0000  & 2.48E-03 & 0.00E75 \\ 
        515050.SH & linearreg & 55.22  & 0.08  & 1000 & 0 & 1.6669  & 0.0042  & -0.0081  & 0.0000  & 1.47E-03 & 4.01E-06 \\ 
        515050.SH & ridge & 55.52  & 0.13  & 1000 & 0 & 1.4807  & 0.0035  & -0.0080  & 0.0000  & 1.21E-03 & 1.77E-06 \\ 
        515050.SH & lasso & 11.40  & 0.00  & 1000 & 0 & 2.8859  & 0.0000  & -0.0324  & 0.0000  & 2.48E-03 & 0.00E78 \\ 
        515050.SH & elasticnet & 11.40  & 0.00  & 1000 & 0 & 2.8859  & 0.0000  & -0.0324  & 0.0000  & 2.48E-03 & 0.00E79 \\ 
        515050.SH & lassolars & 11.40  & 0.00  & 1000 & 0 & 2.8859  & 0.0000  & -0.0324  & 0.0000  & 2.48E-03 & 0.00E80 \\ 
        515050.SH & bayesianridge & 55.52  & 0.13  & 1000 & 0 & 1.6720  & 0.0047  & -0.0081  & 0.0000  & 1.48E-03 & 2.30E-06 \\ 
        515050.SH & PassiveAggressiveReg & 11.40  & 0.00  & 1000 & 0 & 2.8859  & 0.0000  & -0.0324  & 0.0000  & 2.48E-03 & 0.00E82 \\ 
        515050.SH & sgdreg & 20.52  & 1.13  & 1000 & 0 & 1.2582  & 0.0769  & -0.0200  & 0.0084  & 4.78E-04 & 4.31E-05 \\ 
        515050.SH & svr & 11.40  & 0.00  & 1000 & 0 & 2.8859  & 0.0000  & -0.0324  & 0.0000  & 2.48E-03 & 0.00E84 \\ 
        515050.SH & mlpreg & 16.82  & 3.81  & 1000 & 0 & 1.1545  & 0.0852  & -0.0555  & 0.0396  & 3.49E-04 & 1.92E-04 \\ 
        515050.SH & knnreg & 20.64  & 0.22  & 1000 & 0 & 1.2380  & 0.0345  & -0.0285  & 0.0062  & 4.85E-04 & 2.49E-05 \\ 
        515050.SH & adareg & 35.54  & 3.23  & 1000 & 0 & 1.4282  & 0.1420  & -0.0248  & 0.0046  & 1.01E-03 & 1.12E-04 \\ 
        515050.SH & gbreg & 51.78  & 0.29  & 1000 & 0 & 1.8225  & 0.0257  & -0.0057  & 0.0007  & 1.41E-03 & 8.59E-06 \\ 
        515050.SH & baggingreg & 41.68  & 1.20  & 1000 & 0 & 1.6431  & 0.1014  & -0.0181  & 0.0062  & 1.19E-03 & 4.84E-05 \\ 
        515050.SH & extratreereg & 19.22  & 0.99  & 1000 & 0 & 1.3188  & 0.0369  & -0.0209  & 0.0090  & 4.45E-04 & 4.32E-05 \\ 
    \bottomrule
    \end{tabular}
    \caption{Baselines. Long position with lastprice condition on 1000 trades.}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{l|l|cc|cc|cc|cc|cc}
    \toprule
        etf & method & Precision(\%) &  & Trans &  & PLR &  & MDD &  & OTR &  \\ 
    \midrule
        159915.SZ & ols & 46.22  & 0.13  & 1000 & 0 & 2.648  & 0.064  & -0.0019  & 0.0000  & 1.19E-03 & 3.75E-06 \\ 
        159915.SZ & gls & 46.22  & 0.13  & 1000 & 0 & 2.648  & 0.064  & -0.0019  & 0.0000  & 1.19E-03 & 3.75E-06 \\ 
        159915.SZ & glsar & 46.22  & 0.13  & 1000 & 0 & 2.647  & 0.064  & -0.0019  & 0.0000  & 1.19E-03 & 3.97E-06 \\ 
        159915.SZ & autoreg & 2.26  & 0.09  & 1000 & 0 & 0.389  & 0.005  & -0.9937  & 0.0138  & -1.01E-03 & 5.27E-05 \\ 
        159915.SZ & arima & 2.90  & 0.00  & 1000 & 0 & 0.233  & 0.014  & -1.0000  & 0.0000  & -1.69E-03 & 1.28E-04 \\ 
        159915.SZ & expsmooth & 5.50  & 0.83  & 1000 & 0 & 1.324  & 0.908  & -0.3456  & 0.2016  & 5.01E-04 & 1.05E-03 \\ 
        159915.SZ & ets & 3.10  & 0.00  & 1000 & 0 & 0.314  & 0.000  & -1.0000  & 0.0000  & -1.33E-03 & 0.00E6 \\ 
        159915.SZ & linearreg & 46.22  & 0.13  & 1000 & 0 & 2.648  & 0.064  & -0.0019  & 0.0000  & 1.19E-03 & 3.75E-06 \\ 
        159915.SZ & ridge & 46.38  & 0.16  & 1000 & 0 & 2.437  & 0.030  & -0.0022  & 0.0000  & 1.10E-03 & 2.66E-06 \\ 
        159915.SZ & lasso & 3.10  & 0.00  & 1000 & 0 & 0.314  & 0.000  & -1.0000  & 0.0000  & -1.33E-03 & 0.00E9 \\ 
        159915.SZ & elasticnet & 3.10  & 0.00  & 1000 & 0 & 0.314  & 0.000  & -1.0000  & 0.0000  & -1.33E-03 & 0.00E10 \\ 
        159915.SZ & lassolars & 3.10  & 0.00  & 1000 & 0 & 0.314  & 0.000  & -1.0000  & 0.0000  & -1.33E-03 & 0.00E11 \\ 
        159915.SZ & bayesianridge & 46.38  & 0.16  & 1000 & 0 & 2.688  & 0.010  & -0.0019  & 0.0000  & 1.19E-03 & 4.32E-06 \\ 
        159915.SZ & PassiveAggressiveReg & 3.10  & 0.00  & 1000 & 0 & 0.314  & 0.000  & -1.0000  & 0.0000  & -1.33E-03 & 0.00E13 \\ 
        159915.SZ & sgdreg & 16.26  & 3.34  & 1000 & 0 & 1.462  & 0.162  & -0.0122  & 0.0032  & 4.33E-04 & 9.50E-05 \\ 
        159915.SZ & svr & 3.10  & 0.00  & 1000 & 0 & 0.314  & 0.000  & -1.0000  & 0.0000  & -1.33E-03 & 0.00E15 \\ 
        159915.SZ & mlpreg & 8.00  & 5.02  & 1000 & 0 & 1.033  & 0.275  & -0.2322  & 0.1458  & -6.80E-05 & 3.04E-04 \\ 
        159915.SZ & knnreg & 16.36  & 0.28  & 1000 & 0 & 1.449  & 0.011  & -0.0126  & 0.0022  & 4.50E-04 & 6.70E-06 \\ 
        159915.SZ & adareg & 35.16  & 1.36  & 1000 & 0 & 2.016  & 0.233  & -0.0055  & 0.0015  & 1.00E-03 & 2.69E-05 \\ 
        159915.SZ & gbreg & 45.36  & 0.41  & 1000 & 0 & 2.067  & 0.073  & -0.0047  & 0.0008  & 1.19E-03 & 2.13E-05 \\ 
        159915.SZ & baggingreg & 31.12  & 3.77  & 1000 & 0 & 1.869  & 0.105  & -0.0084  & 0.0021  & 8.71E-04 & 5.16E-05 \\ 
        159915.SZ & extratreereg & 15.98  & 1.27  & 1000 & 0 & 1.326  & 0.086  & -0.0161  & 0.0067  & 3.55E-04 & 4.67E-05 \\ 
    \midrule
        512480.SH & ols & 22.78  & 0.33  & 1000 & 0 & 2.548  & 0.022  & -0.1612  & 0.0019  & 2.65E-03 & 7.68E-06 \\ 
        512480.SH & gls & 22.78  & 0.33  & 1000 & 0 & 2.548  & 0.022  & -0.1612  & 0.0019  & 2.65E-03 & 7.68E-06 \\ 
        512480.SH & glsar & 22.78  & 0.33  & 1000 & 0 & 2.548  & 0.022  & -0.1612  & 0.0019  & 2.65E-03 & 7.68E-06 \\ 
        512480.SH & autoreg & 13.00  & 0.45  & 1000 & 0 & 1.462  & 0.365  & -0.5337  & 0.1927  & 1.72E-03 & 2.19E-04 \\ 
        512480.SH & arima & 7.70  & 0.00  & 1000 & 0 & 3.808  & 0.000  & -0.0155  & 0.0000  & 1.75E-03 & 0.00E27 \\ 
        512480.SH & expsmooth & 17.58  & 1.52  & 1000 & 0 & 1.503  & 1.488  & -0.6809  & 0.1788  & 6.98E-04 & 2.22E-03 \\ 
        512480.SH & ets & 7.70  & 0.00  & 1000 & 0 & 3.809  & 0.000  & -0.0155  & 0.0000  & 1.75E-03 & 0.00E29 \\ 
        512480.SH & linearreg & 22.78  & 0.33  & 1000 & 0 & 2.548  & 0.022  & -0.1612  & 0.0019  & 2.65E-03 & 7.68E-06 \\ 
        512480.SH & ridge & 22.82  & 0.35  & 1000 & 0 & 3.630  & 0.037  & -0.0884  & 0.0017  & 3.56E-03 & 5.22E-06 \\ 
        512480.SH & lasso & 7.70  & 0.00  & 1000 & 0 & 3.809  & 0.000  & -0.0155  & 0.0000  & 1.75E-03 & 0.00E32 \\ 
        512480.SH & elasticnet & 7.70  & 0.00  & 1000 & 0 & 3.809  & 0.000  & -0.0155  & 0.0000  & 1.75E-03 & 0.00E33 \\ 
        512480.SH & lassolars & 7.70  & 0.00  & 1000 & 0 & 3.809  & 0.000  & -0.0155  & 0.0000  & 1.75E-03 & 0.00E34 \\ 
        512480.SH & bayesianridge & 22.82  & 0.35  & 1000 & 0 & 2.571  & 0.010  & -0.1604  & 0.0000  & 2.65E-03 & 9.25E-06 \\ 
        512480.SH & PassiveAggressiveReg & 7.70  & 0.00  & 1000 & 0 & 3.809  & 0.000  & -0.0155  & 0.0000  & 1.75E-03 & 0.00E36 \\ 
        512480.SH & sgdreg & 33.32  & 1.47  & 1000 & 0 & 1.527  & 0.252  & -0.0436  & 0.0267  & 7.66E-04 & 9.61E-05 \\ 
        512480.SH & svr & 7.70  & 0.00  & 1000 & 0 & 3.809  & 0.000  & -0.0155  & 0.0000  & 1.75E-03 & 0.00E38 \\ 
        512480.SH & mlpreg & 36.44  & 19.79  & 1000 & 0 & 2.284  & 0.414  & -0.0841  & 0.0910  & 1.70E-03 & 6.73E-04 \\ 
        512480.SH & knnreg & 34.50  & 0.66  & 1000 & 0 & 2.401  & 0.152  & -0.0146  & 0.0017  & 1.09E-03 & 2.76E-05 \\ 
        512480.SH & adareg & 66.48  & 1.82  & 1000 & 0 & 2.230  & 0.258  & -0.0188  & 0.0024  & 1.79E-03 & 8.20E-05 \\ 
        512480.SH & gbreg & 69.78  & 1.42  & 1000 & 0 & 2.612  & 0.227  & -0.0207  & 0.0076  & 2.20E-03 & 8.76E-05 \\ 
        512480.SH & baggingreg & 57.98  & 1.54  & 1000 & 0 & 2.463  & 0.144  & -0.0168  & 0.0061  & 1.88E-03 & 4.91E-05 \\ 
        512480.SH & extratreereg & 32.66  & 2.94  & 1000 & 0 & 1.546  & 0.240  & -0.0307  & 0.0118  & 7.91E-04 & 1.67E-04 \\ 
    \bottomrule
    \end{tabular}
    \caption{Baselines. Short position with lastprice condition on 1000 trades.}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{l|l|cc|cc|cc|cc|cc}
    \toprule
        etf & method & Precision(\%) &  & Trans &  & PLR &  & MDD &  & OTR &  \\ 
    \midrule
        512880.SH & ols & 39.46  & 0.18  & 1000 & 0 & 0.495  & 0.002  & -1.0000  & 0.0000  & -1.52E-03 & 2.41E-05 \\ 
        512880.SH & gls & 39.46  & 0.18  & 1000 & 0 & 0.495  & 0.002  & -1.0000  & 0.0000  & -1.52E-03 & 2.41E-05 \\ 
        512880.SH & glsar & 39.48  & 0.16  & 1000 & 0 & 0.495  & 0.002  & -1.0000  & 0.0000  & -1.52E-03 & 2.27E-05 \\ 
        512880.SH & autoreg & 12.94  & 7.25  & 1000 & 0 & 0.679  & 0.111  & -0.5631  & 0.2445  & -5.78E-04 & 1.11E-03 \\ 
        512880.SH & arima & 11.20  & 0.12  & 1000 & 0 & 0.676  & 0.035  & -0.6101  & 0.0000  & 1.27E-04 & 2.74E-05 \\ 
        512880.SH & expsmooth & 18.68  & 2.89  & 1000 & 0 & 1.516  & 0.628  & -0.5620  & 0.4012  & 5.80E-04 & 1.00E-03 \\ 
        512880.SH & ets & 7.90  & 0.00  & 1000 & 0 & 0.623  & 0.000  & -1.0000  & 0.0000  & -7.83E-04 & 0.00E52 \\ 
        512880.SH & linearreg & 39.46  & 0.18  & 1000 & 0 & 0.495  & 0.002  & -1.0000  & 0.0000  & -1.52E-03 & 2.41E-05 \\ 
        512880.SH & ridge & 39.34  & 0.09  & 1000 & 0 & 0.983  & 0.005  & -0.3403  & 0.0068  & 1.03E-03 & 3.82E-06 \\ 
        512880.SH & lasso & 7.90  & 0.00  & 1000 & 0 & 0.623  & 0.000  & -1.0000  & 0.0000  & -7.83E-04 & 0.00E55 \\ 
        512880.SH & elasticnet & 7.90  & 0.00  & 1000 & 0 & 0.623  & 0.000  & -1.0000  & 0.0000  & -7.83E-04 & 0.00E56 \\ 
        512880.SH & lassolars & 7.90  & 0.00  & 1000 & 0 & 0.623  & 0.000  & -1.0000  & 0.0000  & -7.83E-04 & 0.00E57 \\ 
        512880.SH & bayesianridge & 39.34  & 0.09  & 1000 & 0 & 0.498  & 0.001  & -1.0000  & 0.0000  & -1.49E-03 & 1.87E-05 \\ 
        512880.SH & PassiveAggressiveReg & 7.90  & 0.00  & 1000 & 0 & 0.623  & 0.000  & -1.0000  & 0.0000  & -7.83E-04 & 0.00E59 \\ 
        512880.SH & sgdreg & 30.10  & 4.04  & 1000 & 0 & 0.855  & 0.116  & -0.4168  & 0.2311  & 1.23E-04 & 1.05E-04 \\ 
        512880.SH & svr & 7.90  & 0.00  & 1000 & 0 & 0.623  & 0.000  & -1.0000  & 0.0000  & -7.83E-04 & 0.00E61 \\ 
        512880.SH & mlpreg & 27.24  & 5.16  & 1000 & 0 & 1.111  & 0.394  & -0.4970  & 0.3361  & -1.50E-04 & 1.65E-03 \\ 
        512880.SH & knnreg & 32.50  & 0.47  & 1000 & 0 & 1.541  & 0.042  & -0.1514  & 0.0199  & 8.08E-04 & 6.18E-05 \\ 
        512880.SH & adareg & 54.16  & 2.45  & 1000 & 0 & 1.537  & 0.276  & -0.0279  & 0.0152  & 1.44E-03 & 2.77E-04 \\ 
        512880.SH & gbreg & 42.74  & 1.57  & 1000 & 0 & 1.442  & 0.202  & -0.1586  & 0.0209  & 1.31E-03 & 3.19E-04 \\ 
        512880.SH & baggingreg & 38.84  & 1.99  & 1000 & 0 & 1.038  & 0.218  & -0.2062  & 0.1462  & 9.16E-04 & 2.47E-04 \\ 
        512880.SH & extratreereg & 29.40  & 0.94  & 1000 & 0 & 1.044  & 0.171  & -0.2730  & 0.1354  & 2.55E-04 & 2.29E-04 \\ 
    \midrule
        515050.SH & ols & 55.24  & 0.11  & 1000 & 0 & 1.403  & 0.016  & -0.0212  & 0.0000  & 1.41E-03 & 3.12E-06 \\ 
        515050.SH & gls & 55.24  & 0.11  & 1000 & 0 & 1.403  & 0.016  & -0.0212  & 0.0000  & 1.41E-03 & 3.12E-06 \\ 
        515050.SH & glsar & 55.24  & 0.11  & 1000 & 0 & 1.403  & 0.016  & -0.0212  & 0.0000  & 1.41E-03 & 3.12E-06 \\ 
        515050.SH & autoreg & 7.76  & 0.09  & 1000 & 0 & 0.684  & 0.058  & -1.0000  & 0.0000  & -2.53E-03 & 2.73E-04 \\ 
        515050.SH & arima & 8.50  & 0.00  & 1000 & 0 & 0.137  & 0.000  & -1.0000  & 0.0000  & -3.92E-03 & 0.00E73 \\ 
        515050.SH & expsmooth & 7.12  & 0.50  & 1000 & 0 & 0.739  & 0.246  & -0.9306  & 0.0950  & -7.13E-04 & 6.59E-04 \\ 
        515050.SH & ets & 9.30  & 0.00  & 1000 & 0 & 0.279  & 0.000  & -1.0000  & 0.0000  & -2.92E-03 & 0.00E75 \\ 
        515050.SH & linearreg & 55.24  & 0.11  & 1000 & 0 & 1.403  & 0.016  & -0.0212  & 0.0000  & 1.41E-03 & 3.12E-06 \\ 
        515050.SH & ridge & 55.50  & 0.10  & 1000 & 0 & 1.670  & 0.001  & -0.0073  & 0.0000  & 1.26E-03 & 4.63E-07 \\ 
        515050.SH & lasso & 9.30  & 0.00  & 1000 & 0 & 0.279  & 0.000  & -1.0000  & 0.0000  & -2.92E-03 & 0.00E78 \\ 
        515050.SH & elasticnet & 9.30  & 0.00  & 1000 & 0 & 0.279  & 0.000  & -1.0000  & 0.0000  & -2.92E-03 & 0.00E79 \\ 
        515050.SH & lassolars & 9.30  & 0.00  & 1000 & 0 & 0.279  & 0.000  & -1.0000  & 0.0000  & -2.92E-03 & 0.00E80 \\ 
        515050.SH & bayesianridge & 55.50  & 0.10  & 1000 & 0 & 1.392  & 0.002  & -0.0212  & 0.0000  & 1.41E-03 & 1.50E-06 \\ 
        515050.SH & PassiveAggressiveReg & 9.30  & 0.00  & 1000 & 0 & 0.279  & 0.000  & -1.0000  & 0.0000  & -2.92E-03 & 0.00E82 \\ 
        515050.SH & sgdreg & 20.68  & 3.21  & 1000 & 0 & 1.187  & 0.102  & -0.0320  & 0.0121  & 4.48E-04 & 9.94E-05 \\ 
        515050.SH & svr & 9.30  & 0.00  & 1000 & 0 & 0.279  & 0.000  & -1.0000  & 0.0000  & -2.92E-03 & 0.00E84 \\ 
        515050.SH & mlpreg & 12.42  & 4.92  & 1000 & 0 & 1.106  & 0.115  & -0.0801  & 0.0432  & 2.33E-04 & 2.06E-04 \\ 
        515050.SH & knnreg & 23.94  & 0.38  & 1000 & 0 & 1.348  & 0.023  & -0.0300  & 0.0011  & 6.65E-04 & 1.61E-05 \\ 
        515050.SH & adareg & 40.76  & 1.07  & 1000 & 0 & 1.622  & 0.080  & -0.0186  & 0.0049  & 1.29E-03 & 6.19E-05 \\ 
        515050.SH & gbreg & 55.18  & 0.51  & 1000 & 0 & 1.840  & 0.160  & -0.0046  & 0.0008  & 1.52E-03 & 1.84E-05 \\ 
        515050.SH & baggingreg & 40.22  & 1.18  & 1000 & 0 & 1.455  & 0.113  & -0.0136  & 0.0075  & 1.10E-03 & 4.02E-05 \\ 
        515050.SH & extratreereg & 18.82  & 0.73  & 1000 & 0 & 1.197  & 0.132  & -0.0269  & 0.0160  & 4.27E-04 & 5.90E-05 \\ 
    \bottomrule
    \end{tabular}
    \caption{Baselines. Short position with lastprice condition on 1000 trades.}
\end{table*}

\subsection{Comparison experimental results}
\subsection{Parameter study}
\subsection{Discussion of Computational complexity}


==> Table.tex <==
\begin{table*}[htp]
    \centering
    \begin{tabular}{c|ccc|ccccc}
    \toprule
        Fund & Semi-Lazy & Metric & Labeling & Precision(\%) & Transactions & Profit-Loss Ratio & Max Drawdown & One-trade Return  \\
    \midrule
        \multirow{8}*{512880} 
         & - & - & - & 53.20  $\pm$ 0.23  & 15760.8  $\pm$ 161.1  & 1.115  $\pm$ 0.015  & -0.0077  $\pm$ 0.0009  & 8.04E-05 $\pm$ 1.05E-06 \\ 
         & RNN & - & - & 56.01  $\pm$ 0.15  & 6076.4  $\pm$ 70.9  & 1.242  $\pm$ 0.024  & -0.0042  $\pm$ 0.0008  & 1.37E-04 $\pm$ 3.66E-06 \\ 
         & - & TRUE & - & 57.83  $\pm$ 0.17  & 16850.8  $\pm$ 71.2  & 1.029  $\pm$ 0.022  & -0.0190  $\pm$ 0.0031  & 7.87E-05 $\pm$ 2.98E-06 \\ 
         & RNN & TRUE & - & 75.05  $\pm$ 1.62  & 484.8  $\pm$ 99.6  & 1.288  $\pm$ 0.173  & -0.0029  $\pm$ 0.0008  & 6.95E-04 $\pm$ 5.08E-05 \\ 
         & - & - & TRUE & 54.92  $\pm$ 0.14  & 13256.4  $\pm$ 41.7  & 1.138  $\pm$ 0.014  & -0.0063  $\pm$ 0.0010  & 9.27E-05 $\pm$ 1.86E-06 \\ 
         & RNN & - & TRUE & 58.37  $\pm$ 0.34  & 4737.6  $\pm$ 56.9  & 1.211  $\pm$ 0.010  & -0.0027  $\pm$ 0.0007  & 1.41E-04 $\pm$ 4.10E-06 \\ 
         & - & TRUE & TRUE & 59.77  $\pm$ 0.14  & 14204.4  $\pm$ 141.0  & 1.081  $\pm$ 0.021  & -0.0108  $\pm$ 0.0017  & 9.02E-05 $\pm$ 1.76E-06 \\ 
         & RNN & TRUE & TRUE & 80.40  $\pm$ 2.02  & 245.8  $\pm$ 56.3  & 1.279  $\pm$ 0.215  & -0.0022  $\pm$ 0.0010  & 8.42E-04 $\pm$ 4.04E-05 \\ 
    \midrule
        \multirow{8}*{512480} 
         & - & - & - & 49.73  $\pm$ 0.30  & 9856.0  $\pm$ 26.4  & 1.185  $\pm$ 0.005  & -0.0046  $\pm$ 0.0000  & 1.55E-04 $\pm$ 4.87E-06 \\ 
         & RNN & - & - & 60.58  $\pm$ 1.17  & 2821.0  $\pm$ 105.3  & 1.595  $\pm$ 0.033  & -0.0030  $\pm$ 0.0003  & 3.47E-04 $\pm$ 4.42E-06 \\ 
         & - & TRUE & - & 58.65  $\pm$ 0.32  & 8442.6  $\pm$ 29.6  & 1.085  $\pm$ 0.004  & -0.0074  $\pm$ 0.0006  & 1.68E-04 $\pm$ 1.85E-06 \\ 
         & RNN & TRUE & - & 84.39  $\pm$ 0.96  & 616.6  $\pm$ 32.1  & 1.886  $\pm$ 0.101  & -0.0032  $\pm$ 0.0003  & 6.70E-04 $\pm$ 2.50E-05 \\ 
         & - & - & TRUE & 64.99  $\pm$ 0.31  & 7424.4  $\pm$ 59.4  & 1.255  $\pm$ 0.011  & -0.0045  $\pm$ 0.0008  & 1.92E-04 $\pm$ 1.93E-06 \\ 
         & RNN & - & TRUE & 52.58  $\pm$ 0.84  & 1461.0  $\pm$ 51.5  & 1.826  $\pm$ 0.021  & -0.0027  $\pm$ 0.0008  & 4.74E-04 $\pm$ 4.16E-06 \\ 
         & - & TRUE & TRUE & 62.11  $\pm$ 0.18  & 6625.0  $\pm$ 23.1  & 1.151  $\pm$ 0.012  & -0.0051  $\pm$ 0.0009  & 2.01E-04 $\pm$ 2.26E-06 \\ 
         & RNN & TRUE & TRUE & 88.70  $\pm$ 1.49  & 299.6  $\pm$ 22.1  & 2.017  $\pm$ 0.228  & -0.0024  $\pm$ 0.0007  & 8.47E-04 $\pm$ 2.36E-05 \\ 
    \midrule
        \multirow{8}*{515050} 
         & - & - & - & 25.21  $\pm$ 0.25  & 15860.2  $\pm$ 313.1  & 1.011  $\pm$ 0.010  & -0.0052  $\pm$ 0.0002  & 9.36E-05 $\pm$ 1.63E-06 \\ 
         & KNN & - & - & 26.87  $\pm$ 0.24  & 7617.2  $\pm$ 172.6  & 1.126  $\pm$ 0.010  & -0.0043  $\pm$ 0.0006  & 1.93E-04 $\pm$ 5.59E-06 \\ 
         & - & TRUE & - & 35.20  $\pm$ 0.28  & 10666.8  $\pm$ 218.1  & 1.008  $\pm$ 0.008  & -0.0059  $\pm$ 0.0006  & 1.41E-04 $\pm$ 3.08E-06 \\ 
         & KNN & TRUE & - & 56.76  $\pm$ 1.07  & 820.4  $\pm$ 59.7  & 1.379  $\pm$ 0.074  & -0.0027  $\pm$ 0.0002  & 6.33E-04 $\pm$ 1.35E-04 \\ 
         & - & - & TRUE & 26.46  $\pm$ 0.23  & 13020.4  $\pm$ 470.8  & 1.041  $\pm$ 0.006  & -0.0044  $\pm$ 0.0000  & 1.17E-04 $\pm$ 1.84E-06 \\ 
         & KNN & - & TRUE & 27.65  $\pm$ 0.43  & 4828.4  $\pm$ 84.7  & 1.184  $\pm$ 0.017  & -0.0037  $\pm$ 0.0002  & 2.65E-04 $\pm$ 4.42E-06 \\ 
         & - & TRUE & TRUE & 37.96  $\pm$ 0.31  & 8378.4  $\pm$ 149.0  & 1.023  $\pm$ 0.006  & -0.0056  $\pm$ 0.0011  & 1.73E-04 $\pm$ 2.76E-06 \\ 
         & KNN & TRUE & TRUE & 63.59  $\pm$ 3.62  & 282.8  $\pm$ 15.4  & 1.655  $\pm$ 0.120  & -0.0014  $\pm$ 0.0003  & 9.08E-04 $\pm$ 6.63E-05 \\ 
    \midrule
        \multirow{8}*{159915} 
         & - & - & - & 19.84  $\pm$ 0.06  & 13846.8  $\pm$ 218.6  & 1.013  $\pm$ 0.006  & -0.0042  $\pm$ 0.0004  & 8.23E-05 $\pm$ 1.88E-06 \\ 
         & KNN & - & - & 23.92  $\pm$ 0.47  & 7072.4  $\pm$ 212.1  & 1.140  $\pm$ 0.017  & -0.0027  $\pm$ 0.0001  & 1.44E-04 $\pm$ 8.97E-06 \\ 
         & - & TRUE & - & 28.94  $\pm$ 0.26  & 7214.2  $\pm$ 141.3  & 1.065  $\pm$ 0.014  & -0.0054  $\pm$ 0.0009  & 1.37E-04 $\pm$ 1.07E-06 \\ 
         & KNN & TRUE & - & 44.93  $\pm$ 2.66  & 806.8  $\pm$ 233.9  & 1.483  $\pm$ 0.212  & -0.0018  $\pm$ 0.0011  & 4.35E-04 $\pm$ 3.11E-05 \\ 
         & - & - & TRUE & 21.32  $\pm$ 0.10  & 11189.0  $\pm$ 161.3  & 1.060  $\pm$ 0.004  & -0.0041  $\pm$ 0.0002  & 1.04E-04 $\pm$ 1.73E-06 \\ 
         & KNN & - & TRUE & 26.63  $\pm$ 0.11  & 4548.8  $\pm$ 114.8  & 1.235  $\pm$ 0.015  & -0.0022  $\pm$ 0.0004  & 1.94E-04 $\pm$ 5.90E-06 \\ 
         & - & TRUE & TRUE & 31.48  $\pm$ 0.35  & 5479.0  $\pm$ 128.6  & 1.127  $\pm$ 0.016  & -0.0033  $\pm$ 0.0016  & 1.70E-04 $\pm$ 1.01E-06 \\ 
         & KNN & TRUE & TRUE & 51.56  $\pm$ 3.41  & 324.0  $\pm$ 147.6  & 1.675  $\pm$ 0.075  & -0.0013  $\pm$ 0.0008  & 6.25E-04 $\pm$ 4.08E-05 \\ 
    \bottomrule
    \end{tabular}
    \caption{Ablation experiments with 4 ETFs. Long position in lastprice.}
    \label{tab:ablation-long-position-lastprice}
\end{table*}

\begin{table*}[htp]
    \centering
    \begin{tabular}{c|ccc|ccccc}
    \toprule
        Fund & Semi-Lazy & Metric & Labeling & Precision(\%) & Transactions & Profit-Loss Ratio & Max Drawdown & One-trade Return  \\
    \midrule
        \multirow{8}*{512880} 
         & - & - & - & 51.72  $\pm$ 0.25  & 16458.2  $\pm$ 181.6  & 0.992  $\pm$ 0.014  & -0.0225  $\pm$ 0.0017  & 7.55E-05 $\pm$ 2.86E-06 \\ 
         & RNN & - & - & 57.18  $\pm$ 0.18  & 7333.2  $\pm$ 104.7  & 1.113  $\pm$ 0.038  & -0.0077  $\pm$ 0.0017  & 1.50E-04 $\pm$ 1.35E-06 \\ 
         & - & TRUE & - & 53.75  $\pm$ 0.56  & 17754.0  $\pm$ 339.3  & 0.942  $\pm$ 0.013  & -0.0863  $\pm$ 0.0016  & 4.67E-05 $\pm$ 4.87E-05 \\ 
         & RNN & TRUE & - & 71.26  $\pm$ 2.04  & 588.8  $\pm$ 93.9  & 1.097  $\pm$ 0.104  & -0.0049  $\pm$ 0.0108  & 5.88E-04 $\pm$ 1.29E-06 \\ 
         & - & - & TRUE & 53.60  $\pm$ 0.22  & 13537.4  $\pm$ 114.4  & 1.024  $\pm$ 0.012  & -0.0125  $\pm$ 0.0000  & 9.16E-05 $\pm$ 4.50E-06 \\ 
         & RNN & - & TRUE & 58.85  $\pm$ 0.28  & 5529.2  $\pm$ 20.3  & 1.120  $\pm$ 0.036  & -0.0054  $\pm$ 0.0011  & 1.64E-04 $\pm$ 2.56E-06 \\ 
         & - & TRUE & TRUE & 57.87  $\pm$ 0.30  & 13735.2  $\pm$ 224.2  & 0.980  $\pm$ 0.019  & -0.0331  $\pm$ 0.0041  & 7.39E-05 $\pm$ 6.24E-05 \\ 
         & RNN & TRUE & TRUE & 78.37  $\pm$ 3.46  & 297.2  $\pm$ 72.3  & 1.100  $\pm$ 0.253  & -0.0045  $\pm$ 0.0034  & 7.24E-04 $\pm$ 2.89E-06 \\ 
    \midrule
        \multirow{8}*{512480} 
         & - & - & - & 42.95  $\pm$ 0.13  & 10934.8  $\pm$ 125.6  & 1.161  $\pm$ 0.006  & -0.0041  $\pm$ 0.0005  & 1.19E-04 $\pm$ 5.25E-06 \\ 
         & KNN & - & - & 53.59  $\pm$ 0.61  & 4049.2  $\pm$ 152.9  & 1.432  $\pm$ 0.031  & -0.0032  $\pm$ 0.0004  & 2.33E-04 $\pm$ 1.51E-06 \\ 
         & - & TRUE & - & 52.48  $\pm$ 0.10  & 7940.2  $\pm$ 82.6  & 1.121  $\pm$ 0.008  & -0.0059  $\pm$ 0.0000  & 1.45E-04 $\pm$ 1.75E-05 \\ 
         & KNN & TRUE & - & 77.17  $\pm$ 2.03  & 967.8  $\pm$ 49.5  & 1.621  $\pm$ 0.067  & -0.0028  $\pm$ 0.0007  & 4.02E-04 $\pm$ 2.02E-06 \\ 
         & - & - & TRUE & 45.83  $\pm$ 0.27  & 8702.2  $\pm$ 47.4  & 1.219  $\pm$ 0.009  & -0.0035  $\pm$ 0.0001  & 1.43E-04 $\pm$ 2.52E-06 \\ 
         & KNN & - & TRUE & 58.11  $\pm$ 0.46  & 2625.8  $\pm$ 39.0  & 1.583  $\pm$ 0.014  & -0.0023  $\pm$ 0.0003  & 2.92E-04 $\pm$ 1.69E-06 \\ 
         & - & TRUE & TRUE & 55.81  $\pm$ 0.19  & 6246.8  $\pm$ 41.0  & 1.188  $\pm$ 0.007  & -0.0046  $\pm$ 0.0007  & 1.74E-04 $\pm$ 9.31E-06 \\ 
         & KNN & TRUE & TRUE & 85.03  $\pm$ 0.91  & 548.0  $\pm$ 16.2  & 2.018  $\pm$ 0.148  & -0.0016  $\pm$ 0.0009  & 5.32E-04 $\pm$ 2.32E-06 \\ 
    \midrule
        \multirow{8}*{515050} 
         & - & - & - & 27.71  $\pm$ 0.16  & 11412.2  $\pm$ 109.4  & 1.047  $\pm$ 0.007  & -0.0053  $\pm$ 0.0006  & 1.31E-04 $\pm$ 6.29E-06 \\ 
         & KNN & - & - & 36.72  $\pm$ 0.60  & 4294.2  $\pm$ 163.3  & 1.189  $\pm$ 0.006  & -0.0035  $\pm$ 0.0004  & 2.65E-04 $\pm$ 1.61E-06 \\ 
         & - & TRUE & - & 33.92  $\pm$ 0.42  & 8703.6  $\pm$ 185.4  & 1.039  $\pm$ 0.005  & -0.0082  $\pm$ 0.0002  & 1.59E-04 $\pm$ 2.67E-05 \\ 
         & KNN & TRUE & - & 65.21  $\pm$ 2.30  & 566.0  $\pm$ 59.5  & 1.347  $\pm$ 0.090  & -0.0027  $\pm$ 0.0010  & 5.92E-04 $\pm$ 2.69E-06 \\ 
         & - & - & TRUE & 29.78  $\pm$ 0.27  & 9183.0  $\pm$ 198.3  & 1.078  $\pm$ 0.005  & -0.0037  $\pm$ 0.0005  & 1.62E-04 $\pm$ 5.13E-06 \\ 
         & KNN & - & TRUE & 40.40  $\pm$ 0.60  & 2756.2  $\pm$ 70.3  & 1.311  $\pm$ 0.009  & -0.0030  $\pm$ 0.0003  & 3.46E-04 $\pm$ 3.41E-06 \\ 
         & - & TRUE & TRUE & 36.95  $\pm$ 0.40  & 6935.8  $\pm$ 118.9  & 1.058  $\pm$ 0.008  & -0.0073  $\pm$ 0.0008  & 1.89E-04 $\pm$ 1.60E-05 \\ 
         & KNN & TRUE & TRUE & 72.85  $\pm$ 1.82  & 262.4 $\pm$ 28.1  & 1.504  $\pm$ 0.220  & -0.0021  $\pm$ 0.0011  & 7.49E-04 $\pm$ 1.61E-06 \\ 
    \midrule
        \multirow{8}*{159915} 
         & - & - & - & 18.27  $\pm$ 0.12  & 14516.0  $\pm$ 151.8  & 1.028  $\pm$ 0.005  & -0.0055  $\pm$ 0.0003  & 6.63E-05 $\pm$ 6.15E-06 \\ 
         & KNN & - & - & 23.69  $\pm$ 0.33  & 6823.2  $\pm$ 287.8  & 1.176  $\pm$ 0.016  & -0.0042  $\pm$ 0.0005  & 1.30E-04 $\pm$ 1.63E-07 \\ 
         & - & TRUE & - & 30.78  $\pm$ 0.55  & 5941.2  $\pm$ 166.8  & 1.101  $\pm$ 0.009  & -0.0054  $\pm$ 0.0005  & 1.32E-04 $\pm$ 7.31E-05 \\ 
         & KNN & TRUE & - & 53.64  $\pm$ 3.37  & 385.8  $\pm$ 132.7  & 1.847  $\pm$ 0.274  & -0.0014  $\pm$ 0.0009  & 5.41E-04 $\pm$ 3.12E-06 \\ 
         & - & - & TRUE & 20.13  $\pm$ 0.15  & 11259.0  $\pm$ 94.4  & 1.067  $\pm$ 0.004  & -0.0039  $\pm$ 0.0004  & 8.71E-05 $\pm$ 2.43E-06 \\ 
         & KNN & - & TRUE & 26.85  $\pm$ 0.18  & 4130.6  $\pm$ 52.1  & 1.295  $\pm$ 0.008  & -0.0033  $\pm$ 0.0002  & 1.84E-04 $\pm$ 1.04E-06 \\ 
         & - & TRUE & TRUE & 34.76  $\pm$ 0.90  & 4233.8  $\pm$ 250.6  & 1.164  $\pm$ 0.005  & -0.0035  $\pm$ 0.0002  & 1.71E-04 $\pm$ 7.13E-05 \\ 
         & KNN & TRUE & TRUE & 65.02  $\pm$ 3.52  & 110.2  $\pm$ 35.4  & 2.080  $\pm$ 0.071  & -0.0010  $\pm$ 0.0002  & 7.88E-04 $\pm$ 9.45E-06 \\ 
    \bottomrule
    \end{tabular}
    \caption{Ablation experiments with 4 ETFs. Short position in lastprice.}
    \label{tab:ablation-short-position-lastprice}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{c|cc|ccccc}
    \toprule
        Fund & Metric & Semi-Lazy & Precision(\%) & Transactions & Profit-Loss Ratio & Max Drawdown & One-trade Return  \\
    \midrule
        512880 & - & - & 73.28  $\pm$ 0.52  & 1000 $\pm$ 0 & NAN  & -0.0006  $\pm$ 0.0013  & 1.01E-03 $\pm$ 2.20E-05 \\ 
        512880 & TRUE & RNN & 68.66  $\pm$ 0.79  & 1000 $\pm$ 0 & 1.426  $\pm$ 0.068  & -0.0119  $\pm$ 0.0040  & 1.21E-03 $\pm$ 5.90E-05 \\
    \midrule
        512480 & - & - & 69.30  $\pm$ 0.41  & 1000 $\pm$ 0 & 3.218  $\pm$ 0.421  & -0.0043  $\pm$ 0.0014  & 2.08E-03 $\pm$ 4.43E-05 \\ 
        512480 & TRUE & RNN & 80.06  $\pm$ 0.62  & 1000 $\pm$ 0 & 3.644  $\pm$ 0.507  & -0.0078  $\pm$ 0.0014  & 2.36E-03 $\pm$ 5.82E-05 \\ 
    \midrule
        515050 & - & - & 33.04  $\pm$ 0.94  & 1000 $\pm$ 0 & 1.338  $\pm$ 0.102  & -0.0043  $\pm$ 0.0012  & 1.07E-03 $\pm$ 1.82E-05 \\ 
        515050 & TRUE & kNN & 55.36  $\pm$ 1.16  & 1000 $\pm$ 0 & 1.870  $\pm$ 0.085  & -0.0076  $\pm$ 0.0014  & 1.50E-03 $\pm$ 3.01E-05 \\ 
    \midrule
        159915 & - & - & 37.14 $\pm$ 0.45  & 1000 $\pm$ 0 & 2.232  $\pm$ 0.225  & -0.0034  $\pm$ 0.0009  & 1.09E-03 $\pm$ 1.92E-05 \\ 
        159915 & TRUE & KNN & 43.56  $\pm$ 1.17  & 1000 $\pm$ 0 & 2.253  $\pm$ 0.196  & -0.0054  $\pm$ 0.0011  & 1.15E-03 $\pm$ 2.98E-05 \\ 
    \bottomrule
    \end{tabular}
    \caption{Ablation experiments with 4 ETFs. Long position in lastprice condition on maximum 1000 trades.}
    \label{tab:ablation-long-position-lastprice-1000}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{c|cc|ccccc}
    \toprule
        Fund & Metric & Semi-Lazy & Precision(\%) & Transactions & Profit-Loss Ratio & Max Drawdown & One-trade Return  \\
    \midrule
        159915 & - & - & 35.36 $\pm$ 1.40  & 1000 $\pm$ 0 & 2.142  $\pm$ 0.186  & -0.0035  $\pm$ 0.0017  & 1.06E-03 $\pm$ 1.32E-05 \\ 
        159915 & TRUE & KNN & 44.66 $\pm$ 0.78  & 1000 $\pm$ 0 & 1.984  $\pm$ 0.128  & -0.0091  $\pm$ 0.0011  & 1.18E-03 $\pm$ 4.45E-05 \\ 
    \midrule
        512480 & - & - & 70.66 $\pm$ 1.59  & 1000 $\pm$ 0 & 3.298  $\pm$ 0.171  & -0.0038  $\pm$ 0.0008  & 2.01E-03 $\pm$ 3.60E-05 \\ 
        512480 & TRUE & KNN & 76.66 $\pm$ 1.66  & 1000 $\pm$ 0 & 2.779  $\pm$ 0.405  & -0.0102  $\pm$ 0.0031  & 2.21E-03 $\pm$ 8.40E-06 \\ 
    \midrule
        512880 & - & - & 68.52 $\pm$ 0.42  & 1000 $\pm$ 0 & 1.253  $\pm$ 0.251  & -0.0027  $\pm$ 0.0006  & 1.08E-03 $\pm$ 2.54E-05 \\ 
        512880 & TRUE & RNN & 67.2 $\pm$ 1.92  & 1000 $\pm$ 0 & 1.111  $\pm$ 0.061  & -0.0144  $\pm$ 0.0031  & 1.17E-03 $\pm$ 3.18E-05 \\ 
    \midrule
        515050 & - & - & 49.38 $\pm$ 1.14  & 1000 $\pm$ 0 & 1.711  $\pm$ 0.115  & -0.0029  $\pm$ 0.0014  & 1.44E-03 $\pm$ 2.16E-05 \\ 
        515050 & TRUE & KNN & 58.1 $\pm$ 1.15  & 1000 $\pm$ 0 & 1.833  $\pm$ 0.079  & -0.0108  $\pm$ 0.0021  & 1.64E-03 $\pm$ 2.74E-05 \\ 
    \bottomrule
    \end{tabular}
    \caption{Ablation experiments with 4 ETFs. Short position in lastprice condition on maximum 1000 trades.}
    \label{tab:ablation-short-position-lastprice-1000}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{c|cc|ccccc}
    \toprule
        \multirow{2}*{Fund} & \multicolumn{2}{c|}{Semi-Lazy} & \multirow{2}*{Precision(\%)}  & \multirow{2}*{Transactions} & \multirow{2}*{Profit-Loss Ratio} & \multirow{2}*{Max Drawdown} & \multirow{2}*{One-trade Return}  \\
        & Train & Test & & & & &  \\
    \midrule
        \multirow{4}*{512880}
         & train:no & test:no & 53.20  $\pm$ 0.23  & 15760.8  $\pm$ 161.1  & 1.115  $\pm$ 0.015  & -0.0077  $\pm$ 0.0010  & 8.04E-05 $\pm$ 1.86E-06 \\ 
         & train:no & test:yes & 59.22  $\pm$ 1.72  & 1419.0  $\pm$ 272.4  & 1.233  $\pm$ 0.048  & -0.0034  $\pm$ 0.0005  & 4.77E-04 $\pm$ 6.32E-05 \\ 
         & train:yes & test:no & 56.16  $\pm$ 3.17  & 6008.6  $\pm$ 351.7  & 1.163  $\pm$ 0.065  & -0.0293  $\pm$ 0.0135  & 1.86E-04 $\pm$ 1.06E-05 \\ 
         & train:yes & test:yes & 74.95  $\pm$ 2.40  & 467.2  $\pm$ 106.9  & 1.303  $\pm$ 0.163  & -0.0037  $\pm$ 0.0027  & 7.28E-04 $\pm$ 8.01E-05 \\ 
    \midrule
        \multirow{4}*{512480}
         & train:no & test:no & 49.73  $\pm$ 0.30  & 9856.0  $\pm$ 26.4  & 1.185  $\pm$ 0.005  & -0.0046  $\pm$ 0.0002  & 1.55E-04 $\pm$ 1.73E-06 \\ 
         & train:no & test:yes & 52.17  $\pm$ 0.47  & 8237.8  $\pm$ 158.7  & 1.197  $\pm$ 0.008  & -0.0048  $\pm$ 0.0002  & 1.70E-04 $\pm$ 5.10E-06 \\ 
         & train:yes & test:no & 33.19  $\pm$ 11.70  & 3282.4  $\pm$ 1208.6  & 1.326  $\pm$ 0.087  & -0.0167  $\pm$ 0.0048  & 8.79E-05 $\pm$ 8.62E-05 \\ 
         & train:yes & test:yes & 83.79  $\pm$ 1.42  & 634.2  $\pm$ 52.6  & 1.908  $\pm$ 0.060  & -0.0035  $\pm$ 0.0000  & 6.50E-04 $\pm$ 3.81E-05 \\ 
    \midrule
        \multirow{4}*{159915}
         & train:no & test:no & 19.84  $\pm$ 0.06  & 13846.8  $\pm$ 218.6  & 1.013  $\pm$ 0.006  & -0.0042  $\pm$ 0.0000  & 8.23E-05 $\pm$ 1.84E-06 \\ 
         & train:no & test:yes & 24.22  $\pm$ 0.30  & 5289.6  $\pm$ 149.2  & 1.123  $\pm$ 0.011  & -0.0039  $\pm$ 0.0004  & 1.45E-04 $\pm$ 5.51E-06 \\ 
         & train:yes & test:no & 40.86  $\pm$ 5.96  & 1495.0  $\pm$ 719.8  & 1.344  $\pm$ 0.211  & -0.0039  $\pm$ 0.0029  & 3.36E-04 $\pm$ 1.04E-04 \\ 
         & train:yes & test:yes & 48.45  $\pm$ 4.54  & 745.4  $\pm$ 252.5  & 1.501  $\pm$ 0.178  & -0.0019  $\pm$ 0.0005  & 4.52E-04 $\pm$ 7.51E-05 \\ 
    \midrule
        \multirow{4}*{515050}
         & train:no & test:no & 25.21  $\pm$ 0.25  & 15860.2  $\pm$ 313.1  & 1.011  $\pm$ 0.010  & -0.0052  $\pm$ 0.0008  & 9.36E-05 $\pm$ 1.93E-06 \\ 
         & train:no & test:yes & 33.48  $\pm$ 1.45  & 6003.6  $\pm$ 1028.3  & 1.079  $\pm$ 0.047  & -0.0043  $\pm$ 0.0006  & 2.06E-04 $\pm$ 3.63E-05 \\ 
         & train:yes & test:no & 50.14  $\pm$ 1.95  & 1251.4  $\pm$ 206.2  & 1.362  $\pm$ 0.062  & -0.0030  $\pm$ 0.0009  & 5.62E-04 $\pm$ 2.73E-05 \\ 
         & train:yes & test:yes & 56.06  $\pm$ 1.02  & 817.2  $\pm$ 78.4  & 1.374  $\pm$ 0.037  & -0.0026  $\pm$ 0.0006  & 6.42E-04 $\pm$ 1.11E-05 \\ 
    \bottomrule
    \end{tabular}
    \caption{Subset settings. Long position with lastprice.}
    \label{tab:subset-setting-long}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{c|cc|ccccc}
    \toprule
        \multirow{2}*{Fund} & \multicolumn{2}{c|}{Semi-Lazy} & \multirow{2}*{Precision(\%)}  & \multirow{2}*{Transactions} & \multirow{2}*{Profit-Loss Ratio} & \multirow{2}*{Max Drawdown} & \multirow{2}*{One-trade Return}  \\
        & Train & Test & & & & &  \\
    \midrule
        \multirow{4}*{159915}
         & train:no & test:no & 37.14  $\pm$ 0.45  & 1000 $\pm$ 0 & 2.232  $\pm$ 0.225  & -0.0034  $\pm$ 0.0009  & 1.09E-03 $\pm$ 1.92E-05 \\ 
         & train:no & test:yes & 36.92  $\pm$ 1.11  & 1000 $\pm$ 0 & 2.141  $\pm$ 0.085  & -0.0044  $\pm$ 0.0016  & 1.08E-03 $\pm$ 1.90E-05 \\ 
         & train:yes & test:no & 42.88  $\pm$ 3.62  & 1000 $\pm$ 0 & 1.994  $\pm$ 0.307  & -0.0130  $\pm$ 0.0098  & 1.17E-03 $\pm$ 1.06E-04 \\ 
         & train:yes & test:yes & 44.02  $\pm$ 1.60  & 1000 $\pm$ 0 & 2.339  $\pm$ 0.160  & -0.0039  $\pm$ 0.0006  & 1.20E-03 $\pm$ 1.96E-05 \\ 
    \midrule
        \multirow{4}*{512480}
        & train:no & test:no & 69.30  $\pm$ 0.41  & 1000 $\pm$ 0 & 3.218  $\pm$ 0.421  & -0.0043  $\pm$ 0.0014  & 2.08E-03 $\pm$ 4.43E-05 \\ 
         & train:no & test:yes & 70.08  $\pm$ 0.79  & 1000 $\pm$ 0 & 3.088  $\pm$ 0.227  & -0.0049  $\pm$ 0.0002  & 2.11E-03 $\pm$ 5.32E-05 \\ 
         & train:yes & test:no & 38.28  $\pm$ 14.82  & 1000 $\pm$ 0 & 1.813  $\pm$ 0.324  & -0.0573  $\pm$ 0.0543  & 9.11E-04 $\pm$ 6.56E-04 \\ 
         & train:yes & test:yes & 80.50  $\pm$ 0.96  & 1000 $\pm$ 0 & 3.476  $\pm$ 0.318  & -0.0087  $\pm$ 0.0038  & 2.36E-03 $\pm$ 3.48E-05 \\ 
    \midrule
        \multirow{4}*{512880}
         & train:no & test:no & 73.28  $\pm$ 0.52  & 1000 $\pm$ 0 & NAN  & -0.0006  $\pm$ 0.0013  & 1.01E-03 $\pm$ 2.20E-05 \\ 
         & train:no & test:yes & 62.06  $\pm$ 3.16  & 1000 $\pm$ 0 & 1.454  $\pm$ 0.107  & -0.0058  $\pm$ 0.0018  & 1.18E-03 $\pm$ 5.47E-05 \\ 
         & train:yes & test:no & 63.96  $\pm$ 4.84  & 1000 $\pm$ 0 & 0.922  $\pm$ 0.124  & -0.0541  $\pm$ 0.0558  & 1.14E-03 $\pm$ 1.34E-04 \\ 
         & train:yes & test:yes & 68.66  $\pm$ 1.46  & 1000 $\pm$ 0 & 1.437  $\pm$ 0.080  & -0.0101  $\pm$ 0.0047  & 1.20E-03 $\pm$ 4.10E-05 \\ 
    \midrule
        \multirow{4}*{515050}
         & train:no & test:no & 33.04  $\pm$ 0.94  & 1000 $\pm$ 0 & 1.338  $\pm$ 0.102  & -0.0043  $\pm$ 0.0012  & 1.07E-03 $\pm$ 1.82E-05 \\ 
         & train:no & test:yes & 38.40  $\pm$ 0.80  & 1000 $\pm$ 0 & 1.318  $\pm$ 0.044  & -0.0064  $\pm$ 0.0017  & 1.16E-03 $\pm$ 3.40E-05 \\ 
         & train:yes & test:no & 51.56  $\pm$ 0.88  & 1000 $\pm$ 0 & 1.865  $\pm$ 0.061  & -0.0071  $\pm$ 0.0007  & 1.46E-03 $\pm$ 4.00E-05 \\ 
         & train:yes & test:yes & 54.56  $\pm$ 0.90  & 1000 $\pm$ 0 & 1.853  $\pm$ 0.126  & -0.0080  $\pm$ 0.0003  & 1.49E-03 $\pm$ 3.45E-05 \\ 
    \bottomrule
    \end{tabular}
    \caption{Subset settings. Long position with lastprice condition on maximum 1000 trades.}
    \label{tab:subset-setting-long-1000}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{c|cc|ccccc}
    \toprule
        \multirow{2}*{Fund} & \multicolumn{2}{c|}{Semi-Lazy} & \multirow{2}*{Precision(\%)}  & \multirow{2}*{Transactions} & \multirow{2}*{Profit-Loss Ratio} & \multirow{2}*{Max Drawdown} & \multirow{2}*{One-trade Return}  \\
        & Train & Test & & & & &  \\
    \midrule
        \multirow{4}*{159915}
         & train:no & test:no & 18.27  $\pm$ 0.12  & 14516.0  $\pm$ 151.8  & 1.028  $\pm$ 0.005  & -0.0055  $\pm$ 0.0005  & 6.63E-05 $\pm$ 1.63E-07 \\ 
         & train:no & test:yes & 26.19  $\pm$ 0.17  & 4740.8  $\pm$ 107.0  & 1.165  $\pm$ 0.010  & -0.0032  $\pm$ 0.0002  & 1.41E-04 $\pm$ 2.12E-06 \\ 
         & train:yes & test:no & 43.65  $\pm$ 8.04  & 668.4  $\pm$ 239.6  & 1.637  $\pm$ 0.243  & -0.0028  $\pm$ 0.0008  & 4.16E-04 $\pm$ 8.44E-05 \\ 
         & train:yes & test:yes & 52.18  $\pm$ 5.89  & 387.8  $\pm$ 109.0  & 1.883  $\pm$ 0.169  & -0.0013  $\pm$ 0.0006  & 5.19E-04 $\pm$ 5.47E-05 \\ 
    \midrule
        \multirow{4}*{512480}
        & train:no & test:no & 42.93  $\pm$ 0.13  & 10934.8  $\pm$ 125.6  & 1.161  $\pm$ 0.006  & -0.0041  $\pm$ 0.0004  & 1.19E-04 $\pm$ 1.51E-06 \\ 
         & train:no & test:yes & 44.57  $\pm$ 0.27  & 8773.8  $\pm$ 101.8  & 1.157  $\pm$ 0.007  & -0.0044  $\pm$ 0.0003  & 1.34E-04 $\pm$ 1.63E-06 \\ 
         & train:yes & test:no & 29.18  $\pm$ 11.41  & 4600.0  $\pm$ 1374.3  & 1.224  $\pm$ 0.018  & -0.0674  $\pm$ 0.0354  & 1.47E-05 $\pm$ 3.42E-05 \\ 
         & train:yes & test:yes & 77.77  $\pm$ 2.23  & 962.2  $\pm$ 77.1  & 1.692  $\pm$ 0.073  & -0.0026  $\pm$ 0.0003  & 4.10E-04 $\pm$ 9.49E-06 \\ 
    \midrule
        \multirow{4}*{512880}
         & train:no & test:no & 51.72  $\pm$ 0.25  & 16458.2  $\pm$ 181.6  & 0.992  $\pm$ 0.014  & -0.0225  $\pm$ 0.0017  & 7.55E-05 $\pm$ 1.35E-06 \\ 
         & train:no & test:yes & 62.80  $\pm$ 0.44  & 1361.2  $\pm$ 314.5  & 1.150  $\pm$ 0.058  & -0.0069  $\pm$ 0.0017  & 4.91E-04 $\pm$ 7.07E-05 \\ 
         & train:yes & test:no & 54.86  $\pm$ 4.84  & 6394.8  $\pm$ 1533.6  & 1.073  $\pm$ 0.045  & -0.0529  $\pm$ 0.0110  & 1.26E-04 $\pm$ 4.02E-05 \\ 
         & train:yes & test:yes & 72.01  $\pm$ 3.13  & 570.0  $\pm$ 94.0  & 1.102  $\pm$ 0.106  & -0.0059  $\pm$ 0.0029  & 5.92E-04 $\pm$ 3.32E-05 \\ 
    \midrule
        \multirow{4}*{515050}
         & train:no & test:no & 27.71  $\pm$ 0.16  & 11412.2  $\pm$ 109.4  & 1.047  $\pm$ 0.007  & -0.0053  $\pm$ 0.0004  & 1.31E-04 $\pm$ 1.61E-06 \\ 
         & train:no & test:yes & 34.93  $\pm$ 1.64  & 5371.0  $\pm$ 544.6  & 1.074  $\pm$ 0.023  & -0.0037  $\pm$ 0.0003  & 1.87E-04 $\pm$ 1.63E-05 \\ 
         & train:yes & test:no & 58.54  $\pm$ 2.26  & 757.2  $\pm$ 88.3  & 1.313  $\pm$ 0.063  & -0.0050  $\pm$ 0.0036  & 5.42E-04 $\pm$ 4.38E-05 \\ 
         & train:yes & test:yes & 64.07  $\pm$ 1.19  & 560.6  $\pm$ 56.1  & 1.329  $\pm$ 0.061  & -0.0026  $\pm$ 0.0000  & 6.05E-04 $\pm$ 2.44E-05 \\ 
    \bottomrule
    \end{tabular}
    \caption{Subset settings. Short position with lastprice}
    \label{tab:subset-setting-short}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{c|cc|ccccc}
    \toprule
        \multirow{2}*{Fund} & \multicolumn{2}{c|}{Semi-Lazy} & \multirow{2}*{Precision(\%)}  & \multirow{2}*{Transactions} & \multirow{2}*{Profit-Loss Ratio} & \multirow{2}*{Max Drawdown} & \multirow{2}*{One-trade Return}  \\
        & Train & Test & & & & &  \\
    \midrule
        \multirow{4}*{159915}
         & train:no & test:no & 35.36  $\pm$ 1.40  & 1000 $\pm$ 0 & 2.142  $\pm$ 0.186  & -0.0035  $\pm$ 0.0017  & 1.06E-03 $\pm$ 1.32E-05 \\ 
         & train:no & test:yes & 35.32  $\pm$ 0.79  & 1000 $\pm$ 0 & 1.677  $\pm$ 0.121  & -0.0058  $\pm$ 0.0011  & 1.03E-03 $\pm$ 2.42E-05 \\ 
         & train:yes & test:no & 40.86  $\pm$ 4.42  & 1000 $\pm$ 0 & 1.831  $\pm$ 0.201  & -0.0159  $\pm$ 0.0046  & 1.05E-03 $\pm$ 1.41E-04 \\ 
         & train:yes & test:yes & 44.96  $\pm$ 2.98  & 1000 $\pm$ 0 & 1.950  $\pm$ 0.139  & -0.0105  $\pm$ 0.0030  & 1.19E-03 $\pm$ 5.44E-05 \\ 
    \midrule
        \multirow{4}*{512480}
        & train:no & test:no & 71.02  $\pm$ 1.37  & 1000 $\pm$ 0 & 3.298  $\pm$ 0.171  & -0.0038  $\pm$ 0.0008  & 2.01E-03 $\pm$ 3.60E-05 \\ 
         & train:no & test:yes & 70.70  $\pm$ 1.34  & 1000 $\pm$ 0 & 3.266  $\pm$ 0.252  & -0.0038  $\pm$ 0.0015  & 2.01E-03 $\pm$ 5.52E-05 \\ 
         & train:yes & test:no & 39.64  $\pm$ 13.35  & 1000 $\pm$ 0 & 1.467  $\pm$ 0.102  & -0.0874  $\pm$ 0.0386  & 7.61E-04 $\pm$ 4.61E-04 \\ 
         & train:yes & test:yes & 77.26  $\pm$ 1.87  & 1000 $\pm$ 0 & 3.007  $\pm$ 0.535  & -0.0089  $\pm$ 0.0036  & 2.20E-03 $\pm$ 3.05E-05 \\ 
    \midrule
        \multirow{4}*{512880}
         & train:no & test:no & 68.52  $\pm$ 0.42  & 1000 $\pm$ 0 & 1.253  $\pm$ 0.251  & -0.0027  $\pm$ 0.0006  & 1.08E-03 $\pm$ 2.54E-05 \\ 
         & train:no & test:yes & 65.44  $\pm$ 2.37  & 1000 $\pm$ 0 & 1.206  $\pm$ 0.118  & -0.0098  $\pm$ 0.0057  & 1.21E-03 $\pm$ 5.53E-05 \\ 
         & train:yes & test:no & 52.72  $\pm$ 13.22  & 1000 $\pm$ 0 & 0.731  $\pm$ 0.124  & -0.3294  $\pm$ 0.3036  & 8.13E-04 $\pm$ 4.33E-04 \\ 
         & train:yes & test:yes & 67.92  $\pm$ 1.39  & 1000 $\pm$ 0 & 1.065  $\pm$ 0.109  & -0.0144  $\pm$ 0.0023  & 1.16E-03 $\pm$ 5.17E-05 \\ 
    \midrule
        \multirow{4}*{515050}
         & train:no & test:no & 49.38  $\pm$ 1.14  & 1000 $\pm$ 0 & 1.711  $\pm$ 0.115  & -0.0029  $\pm$ 0.0014  & 1.44E-03 $\pm$ 2.16E-05 \\ 
         & train:no & test:yes & 51.32  $\pm$ 0.66  & 1000 $\pm$ 0 & 1.706  $\pm$ 0.224  & -0.0044  $\pm$ 0.0026  & 1.50E-03 $\pm$ 4.51E-05 \\ 
         & train:yes & test:no & 55.10  $\pm$ 2.66  & 1000 $\pm$ 0 & 1.515  $\pm$ 0.232  & -0.0291  $\pm$ 0.0327  & 1.50E-03 $\pm$ 7.74E-05 \\ 
         & train:yes & test:yes & 58.02  $\pm$ 2.07  & 1000 $\pm$ 0 & 1.886  $\pm$ 0.153  & -0.0110  $\pm$ 0.0053  & 1.66E-03 $\pm$ 3.03E-05 \\ 
    \bottomrule
    \end{tabular}
    \caption{Subset settings. Short position with lastprice condition on maximum 1000 trades.}
    \label{tab:subset-setting-short-1000}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{l|l|cc|cc|cc|cc|cc}
    \toprule
        etf & method & Precision(\%) &  & Trans &  & PLR &  & MDD &  & OTR &  \\    
    \midrule
        159915.SZ & ols & 26.22  & 0.06  & 7544.8  & 27.9  & 1.132  & 0.001  & -0.0037  & 0.0002  & 1.46E-04 & 3.10E-07 \\ 
        159915.SZ & gls & 26.22  & 0.06  & 7544.8  & 27.9  & 1.132  & 0.001  & -0.0037  & 0.0002  & 1.46E-04 & 3.10E-07 \\ 
        159915.SZ & glsar & 26.21  & 0.06  & 7544.8  & 28.0  & 1.132  & 0.001  & -0.0037  & 0.0002  & 1.46E-04 & 3.20E-07 \\ 
        159915.SZ & autoreg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E3 & 0.00E3 \\ 
        159915.SZ & arima & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E4 & 0.00E4 \\ 
        159915.SZ & expsmooth & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E5 & 0.00E5 \\ 
        159915.SZ & ets & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E6 & 0.00E6 \\ 
        159915.SZ & linearreg & 26.22  & 0.06  & 7544.8  & 27.9  & 1.132  & 0.001  & -0.0037  & 0.0002  & 1.46E-04 & 3.10E-07 \\ 
        159915.SZ & ridge & 23.86  & 0.02  & 6338.6  & 24.1  & 1.105  & 0.001  & -0.0044  & 0.0000  & 1.38E-04 & 2.66E-07 \\ 
        159915.SZ & lasso & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E9 & 0.00E9 \\ 
        159915.SZ & elasticnet & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E10 & 0.00E10 \\ 
        159915.SZ & lassolars & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E11 & 0.00E11 \\ 
        159915.SZ & bayesianridge & 26.23  & 0.05  & 7547.0  & 24.0  & 1.133  & 0.002  & -0.0038  & 0.0000  & 1.46E-04 & 4.54E-07 \\ 
        159915.SZ & PassiveAggressiveReg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E13 & 0.00E13 \\ 
        159915.SZ & sgdreg & 10.10  & 0.18  & 42550.6  & 1507.8  & 0.944  & 0.006  & -0.0207  & 0.0019  & 6.66E-06 & 5.75E-07 \\ 
        159915.SZ & svr & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E15 & 0.00E15 \\ 
        159915.SZ & mlpreg & 7.55  & 2.08  & 18606.8  & 27532.8  & 1.039  & 0.085  & -0.0230  & 0.0219  & 2.40E-05 & 4.93E-05 \\ 
        159915.SZ & knnreg & 11.53  & 0.04  & 22364.8  & 58.3  & 0.927  & 0.001  & -0.0126  & 0.0006  & 2.42E-05 & 1.95E-07 \\ 
        159915.SZ & adareg & 26.28  & 3.59  & 2260.4  & 893.0  & 1.292  & 0.122  & -0.0056  & 0.0009  & 2.23E-04 & 5.43E-05 \\ 
        159915.SZ & gbreg & 21.15  & 0.55  & 12726.8  & 868.1  & 0.994  & 0.009  & -0.0043  & 0.0001  & 8.76E-05 & 6.53E-06 \\ 
        159915.SZ & baggingreg & 15.33  & 0.12  & 21726.6  & 372.8  & 0.951  & 0.004  & -0.0076  & 0.0011  & 4.05E-05 & 8.98E-07 \\ 
        159915.SZ & extratreereg & 9.89  & 0.15  & 43801.2  & 555.9  & 0.948  & 0.005  & -0.0222  & 0.0010  & 5.51E-06 & 3.27E-07 \\ 
    \midrule
        512480.SH & ols & 46.76  & 0.04  & 15422.4  & 14.5  & 1.021  & 0.001  & -0.0051  & 0.0000  & 9.69E-05 & 1.36E-07 \\ 
        512480.SH & gls & 46.76  & 0.04  & 15422.4  & 14.5  & 1.021  & 0.001  & -0.0051  & 0.0000  & 9.69E-05 & 1.36E-07 \\ 
        512480.SH & glsar & 46.76  & 0.04  & 15422.4  & 14.8  & 1.021  & 0.001  & -0.0051  & 0.0000  & 9.69E-05 & 1.38E-07 \\ 
        512480.SH & autoreg & 0.00  & 0.00  & 0.4  & 0.9  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E26 & 0.00E26 \\ 
        512480.SH & arima & 0.00  & 0.00  & 1.0  & 0.0  &  &  & 0.0000  & 0.0000  & 5.39E-04 & 0.00E27 \\ 
        512480.SH & expsmooth & 3.29  & 7.36  & 16971.4  & 37949.2  & 0.201  & 0.450  & -0.0112  & 0.0251  & 4.90E-07 & 1.10E-06 \\ 
        512480.SH & ets & 3.29  & 7.36  & 16971.4  & 37949.2  & 0.201  & 0.450  & -0.0112  & 0.0251  & 4.90E-07 & 1.10E-06 \\ 
        512480.SH & linearreg & 46.76  & 0.04  & 15422.4  & 14.5  & 1.021  & 0.001  & -0.0051  & 0.0000  & 9.69E-05 & 1.36E-07 \\ 
        512480.SH & ridge & 41.59  & 0.01  & 17724.6  & 8.2  & 1.013  & 0.000  & -0.0065  & 0.0000  & 7.66E-05 & 1.37E-07 \\ 
        512480.SH & lasso & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E32 & 0.00E32 \\ 
        512480.SH & elasticnet & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E33 & 0.00E33 \\ 
        512480.SH & lassolars & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E34 & 0.00E34 \\ 
        512480.SH & bayesianridge & 46.75  & 0.03  & 15427.2  & 10.5  & 1.021  & 0.000  & -0.0051  & 0.0000  & 9.68E-05 & 8.85E-08 \\ 
        512480.SH & PassiveAggressiveReg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E36 & 0.00E36 \\ 
        512480.SH & sgdreg & 24.88  & 0.11  & 42839.0  & 201.1  & 0.951  & 0.004  & -0.0349  & 0.0012  & 9.30E-06 & 4.14E-07 \\ 
        512480.SH & svr & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E38 & 0.00E38 \\ 
        512480.SH & mlpreg & 34.48  & 18.55  & 31566.6  & 28382.0  & 1.107  & 0.245  & -0.0237  & 0.0231  & 1.41E-04 & 2.52E-04 \\ 
        512480.SH & knnreg & 29.77  & 0.07  & 25684.2  & 53.6  & 0.949  & 0.002  & -0.0154  & 0.0007  & 3.25E-05 & 2.80E-07 \\ 
        512480.SH & adareg & 33.28  & 1.50  & 10456.4  & 4150.0  & 1.240  & 0.094  & -0.0091  & 0.0014  & 8.72E-05 & 2.16E-05 \\ 
        512480.SH & gbreg & 43.46  & 0.28  & 18192.4  & 146.3  & 1.001  & 0.007  & -0.0113  & 0.0000  & 8.00E-05 & 1.08E-06 \\ 
        512480.SH & baggingreg & 35.94  & 0.19  & 23447.6  & 201.0  & 0.973  & 0.011  & -0.0124  & 0.0012  & 5.20E-05 & 1.08E-06 \\ 
        512480.SH & extratreereg & 24.43  & 0.03  & 43054.0  & 238.7  & 0.954  & 0.003  & -0.0377  & 0.0014  & 8.09E-06 & 2.77E-07 \\ 
    \bottomrule
    \end{tabular}
    \caption{Baselines. Long position with lastprice.}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{l|l|cc|cc|cc|cc|cc}
    \toprule
        etf & method & Precision(\%) &  & Trans &  & PLR &  & MDD &  & OTR &  \\ 
    \midrule
        512880.SH & ols & 55.07  & 0.05  & 12583.4  & 26.2  & 0.916  & 0.001  & -0.0226  & 0.0000  & 1.34E-04 & 2.89E-07 \\ 
        512880.SH & gls & 55.07  & 0.05  & 12583.4  & 26.2  & 0.916  & 0.001  & -0.0226  & 0.0000  & 1.34E-04 & 2.89E-07 \\ 
        512880.SH & glsar & 55.08  & 0.05  & 12581.8  & 26.2  & 0.916  & 0.001  & -0.0226  & 0.0000  & 1.34E-04 & 2.83E-07 \\ 
        512880.SH & autoreg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E49 & 0.00E49 \\ 
        512880.SH & arima & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E50 & 0.00E50 \\ 
        512880.SH & expsmooth & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E51 & 0.00E51 \\ 
        512880.SH & ets & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E52 & 0.00E52 \\ 
        512880.SH & linearreg & 55.07  & 0.05  & 12583.4  & 26.2  & 0.916  & 0.001  & -0.0226  & 0.0000  & 1.34E-04 & 2.89E-07 \\ 
        512880.SH & ridge & 55.88  & 0.07  & 5641.0  & 26.7  & 0.987  & 0.001  & -0.0210  & 0.0000  & 2.51E-04 & 8.70E-07 \\ 
        512880.SH & lasso & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E55 & 0.00E55 \\ 
        512880.SH & elasticnet & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E56 & 0.00E56 \\ 
        512880.SH & lassolars & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E57 & 0.00E57 \\ 
        512880.SH & bayesianridge & 55.10  & 0.06  & 12569.8  & 22.4  & 0.917  & 0.001  & -0.0226  & 0.0000  & 1.35E-04 & 2.42E-07 \\ 
        512880.SH & PassiveAggressiveReg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E59 & 0.00E59 \\ 
        512880.SH & sgdreg & 35.62  & 0.15  & 45195.8  & 160.4  & 0.987  & 0.003  & -0.0435  & 0.0004  & 8.66E-06 & 1.92E-07 \\ 
        512880.SH & svr & 24.46  & 0.00  & 90317.0  & 0.0  & 1.002  & 0.000  & -0.0437  & 0.0000  & 3.70E-06 & 4.74E-22 \\ 
        512880.SH & mlpreg & 26.75  & 1.87  & 50997.2  & 27141.8  & 1.013  & 0.034  & -0.0435  & 0.0007  & 1.04E-05 & 6.23E-06 \\ 
        512880.SH & knnreg & 31.23  & 0.03  & 16253.2  & 68.9  & 0.932  & 0.001  & -0.0381  & 0.0010  & 3.80E-05 & 4.14E-07 \\ 
        512880.SH & adareg & 44.32  & 3.06  & 9540.8  & 3332.9  & 0.872  & 0.023  & -0.0226  & 0.0043  & 1.17E-04 & 3.42E-05 \\ 
        512880.SH & gbreg & 51.83  & 0.30  & 12790.4  & 38.3  & 0.942  & 0.009  & -0.0164  & 0.0016  & 1.17E-04 & 1.69E-06 \\ 
        512880.SH & baggingreg & 45.10  & 0.29  & 21666.2  & 350.2  & 0.944  & 0.004  & -0.0415  & 0.0022  & 5.17E-05 & 7.41E-07 \\ 
        512880.SH & extratreereg & 35.48  & 0.19  & 45046.4  & 194.8  & 0.986  & 0.007  & -0.0428  & 0.0007  & 8.77E-06 & 2.78E-07 \\ 
    \midrule
        515050.SH & ols & 26.83  & 0.02  & 17709.8  & 24.0  & 0.966  & 0.001  & -0.0074  & 0.0000  & 8.14E-05 & 2.27E-07 \\ 
        515050.SH & gls & 26.83  & 0.02  & 17709.8  & 24.0  & 0.966  & 0.001  & -0.0074  & 0.0000  & 8.14E-05 & 2.27E-07 \\ 
        515050.SH & glsar & 26.83  & 0.03  & 17709.0  & 24.0  & 0.966  & 0.001  & -0.0074  & 0.0000  & 8.14E-05 & 2.29E-07 \\ 
        515050.SH & autoreg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E72 & 0.00E72 \\ 
        515050.SH & arima & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E73 & 0.00E73 \\ 
        515050.SH & expsmooth & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E74 & 0.00E74 \\ 
        515050.SH & ets & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E75 & 0.00E75 \\ 
        515050.SH & linearreg & 26.83  & 0.02  & 17709.8  & 24.0  & 0.966  & 0.001  & -0.0074  & 0.0000  & 8.14E-05 & 2.27E-07 \\ 
        515050.SH & ridge & 23.72  & 0.01  & 16725.0  & 22.0  & 0.988  & 0.000  & -0.0093  & 0.0000  & 7.32E-05 & 1.83E-07 \\ 
        515050.SH & lasso & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E78 & 0.00E78 \\ 
        515050.SH & elasticnet & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E79 & 0.00E79 \\ 
        515050.SH & lassolars & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E80 & 0.00E80 \\ 
        515050.SH & bayesianridge & 26.86  & 0.02  & 17685.6  & 24.9  & 0.966  & 0.001  & -0.0074  & 0.0000  & 8.16E-05 & 1.68E-07 \\ 
        515050.SH & PassiveAggressiveReg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E82 & 0.00E82 \\ 
        515050.SH & sgdreg & 13.94  & 0.08  & 50003.0  & 381.8  & 0.975  & 0.001  & -0.0425  & 0.0029  & 5.36E-06 & 2.21E-07 \\ 
        515050.SH & svr & 9.51  & 0.00  & 92417.0  & 0.0  & 1.001  & 0.000  & -0.0550  & 0.0000  & 1.94E-06 & 0.00E84 \\ 
        515050.SH & mlpreg & 16.01  & 4.13  & 23367.4  & 23633.4  & 1.029  & 0.061  & -0.0206  & 0.0112  & 7.48E-05 & 9.33E-05 \\ 
        515050.SH & knnreg & 14.60  & 0.02  & 33695.8  & 36.9  & 0.969  & 0.000  & -0.0208  & 0.0014  & 1.78E-05 & 1.02E-07 \\ 
        515050.SH & adareg & 26.38  & 6.40  & 12238.8  & 8152.6  & 1.023  & 0.044  & -0.0079  & 0.0019  & 1.24E-04 & 8.51E-05 \\ 
        515050.SH & gbreg & 23.00  & 0.09  & 24235.6  & 117.0  & 0.971  & 0.002  & -0.0077  & 0.0004  & 5.09E-05 & 4.17E-07 \\ 
        515050.SH & baggingreg & 18.54  & 0.11  & 32801.2  & 404.2  & 0.961  & 0.002  & -0.0143  & 0.0007  & 2.45E-05 & 6.37E-07 \\ 
        515050.SH & extratreereg & 13.95  & 0.10  & 48740.2  & 232.0  & 0.977  & 0.004  & -0.0475  & 0.0050  & 5.36E-06 & 1.82E-07 \\ 
    \bottomrule
    \end{tabular}
    \caption{Baselines. Long position with lastprice.}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{l|l|cc|cc|cc|cc|cc}
    \toprule
        etf & method & Precision(\%) &  & Trans &  & PLR &  & MDD &  & OTR &  \\ 
    \midrule
        159915.SZ & ols & 24.24  & 0.02  & 9000.6  & 13.7  & 1.094  & 0.000  & -0.0041  & 0.0001  & 1.11E-04 & 3.00E-07 \\ 
        159915.SZ & gls & 24.24  & 0.02  & 9000.6  & 13.7  & 1.094  & 0.000  & -0.0041  & 0.0001  & 1.11E-04 & 3.00E-07 \\ 
        159915.SZ & glsar & 24.24  & 0.02  & 8999.0  & 14.2  & 1.093  & 0.000  & -0.0041  & 0.0001  & 1.11E-04 & 3.14E-07 \\ 
        159915.SZ & autoreg & 0.00  & 0.00  & 3.0  & 0.0  & 3.000  & 0.000  & -0.0005  & 0.0000  & 8.20E-04 & 0.00E3 \\ 
        159915.SZ & arima & 0.00  & 0.00  & 3.0  & 0.0  & 3.000  & 0.000  & -0.0005  & 0.0000  & 8.20E-04 & 0.00E4 \\ 
        159915.SZ & expsmooth & 5.89  & 0.00  & 87521.0  & 0.0  & 1.007  & 0.000  & -0.1645  & 0.0000  & -1.82E-06 & 0.00E5 \\ 
        159915.SZ & ets & 5.89  & 0.00  & 87521.0  & 0.0  & 1.007  & 0.000  & -0.1645  & 0.0000  & -1.82E-06 & 0.00E6 \\ 
        159915.SZ & linearreg & 24.24  & 0.02  & 9000.6  & 13.7  & 1.094  & 0.000  & -0.0041  & 0.0001  & 1.11E-04 & 3.00E-07 \\ 
        159915.SZ & ridge & 23.40  & 0.04  & 8025.0  & 15.0  & 1.086  & 0.001  & -0.0048  & 0.0000  & 1.04E-04 & 1.84E-07 \\ 
        159915.SZ & lasso & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E9 & 0.00E9 \\ 
        159915.SZ & elasticnet & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E10 & 0.00E10 \\ 
        159915.SZ & lassolars & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E11 & 0.00E11 \\ 
        159915.SZ & bayesianridge & 24.23  & 0.02  & 9004.0  & 12.6  & 1.094  & 0.001  & -0.0041  & 0.0001  & 1.11E-04 & 1.27E-07 \\ 
        159915.SZ & PassiveAggressiveReg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E13 & 0.00E13 \\ 
        159915.SZ & sgdreg & 9.04  & 0.21  & 44970.4  & 1507.8  & 0.950  & 0.004  & -0.0912  & 0.0133  & -1.39E-06 & 2.12E-07 \\ 
        159915.SZ & svr & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E15 & 0.00E15 \\ 
        159915.SZ & mlpreg & 7.62  & 2.43  & 54183.8  & 38045.8  & 1.025  & 0.077  & -0.1040  & 0.0817  & 1.14E-05 & 2.34E-05 \\ 
        159915.SZ & knnreg & 11.32  & 0.01  & 19765.8  & 28.0  & 0.943  & 0.001  & -0.0204  & 0.0003  & 1.68E-05 & 2.20E-07 \\ 
        159915.SZ & adareg & 44.09  & 26.11  & 85.0  & 131.2  & 2.828  & 0.833  & -0.0006  & 0.0004  & 7.89E-04 & 2.86E-04 \\ 
        159915.SZ & gbreg & 18.97  & 0.22  & 15020.0  & 438.9  & 1.001  & 0.002  & -0.0053  & 0.0002  & 6.06E-05 & 2.06E-06 \\ 
        159915.SZ & baggingreg & 13.92  & 0.13  & 23344.2  & 488.4  & 0.955  & 0.002  & -0.0094  & 0.0005  & 2.69E-05 & 1.14E-06 \\ 
        159915.SZ & extratreereg & 9.01  & 0.10  & 43719.8  & 555.9  & 0.953  & 0.001  & -0.1052  & 0.0067  & -2.03E-06 & 2.07E-07 \\ 
    \midrule
        512480.SH & ols & 36.43  & 0.02  & 14862.8  & 24.4  & 1.102  & 0.001  & -0.0335  & 0.0000  & 8.54E-05 & 1.45E-07 \\ 
        512480.SH & gls & 36.43  & 0.02  & 14862.8  & 24.4  & 1.102  & 0.001  & -0.0335  & 0.0000  & 8.54E-05 & 1.45E-07 \\ 
        512480.SH & glsar & 36.43  & 0.02  & 14862.4  & 24.1  & 1.102  & 0.001  & -0.0335  & 0.0000  & 8.54E-05 & 1.43E-07 \\ 
        512480.SH & autoreg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E26 & 0.00E26 \\ 
        512480.SH & arima & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E27 & 0.00E27 \\ 
        512480.SH & expsmooth & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E28 & 0.00E28 \\ 
        512480.SH & ets & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E29 & 0.00E29 \\ 
        512480.SH & linearreg & 36.43  & 0.02  & 14862.8  & 24.4  & 1.102  & 0.001  & -0.0335  & 0.0000  & 8.54E-05 & 1.45E-07 \\ 
        512480.SH & ridge & 34.33  & 0.02  & 16258.6  & 31.2  & 1.055  & 0.001  & -0.0208  & 0.0002  & 7.28E-05 & 1.26E-07 \\ 
        512480.SH & lasso & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E32 & 0.00E32 \\ 
        512480.SH & elasticnet & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E33 & 0.00E33 \\ 
        512480.SH & lassolars & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E34 & 0.00E34 \\ 
        512480.SH & bayesianridge & 36.45  & 0.03  & 14862.0  & 28.2  & 1.102  & 0.002  & -0.0334  & 0.0002  & 8.54E-05 & 2.07E-07 \\ 
        512480.SH & PassiveAggressiveReg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E36 & 0.00E36 \\ 
        512480.SH & sgdreg & 21.82  & 0.05  & 42018.0  & 201.1  & 0.907  & 0.005  & -0.0892  & 0.0046  & -2.62E-07 & 1.75E-07 \\ 
        512480.SH & svr & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E38 & 0.00E38 \\ 
        512480.SH & mlpreg & 22.67  & 5.13  & 32326.4  & 32131.2  & 1.158  & 0.320  & -0.0595  & 0.0823  & 7.34E-05 & 1.11E-04 \\ 
        512480.SH & knnreg & 25.75  & 0.05  & 24292.0  & 50.1  & 0.906  & 0.002  & -0.0289  & 0.0007  & 2.40E-05 & 2.25E-07 \\ 
        512480.SH & adareg & 63.36  & 10.57  & 1794.2  & 1318.4  & 1.444  & 0.252  & -0.0041  & 0.0009  & 3.54E-04 & 1.53E-04 \\ 
        512480.SH & gbreg & 37.76  & 0.16  & 15859.8  & 101.5  & 1.022  & 0.005  & -0.0130  & 0.0010  & 7.93E-05 & 9.46E-07 \\ 
        512480.SH & baggingreg & 31.99  & 0.17  & 20288.2  & 111.6  & 0.970  & 0.008  & -0.0249  & 0.0024  & 5.31E-05 & 6.74E-07 \\ 
        512480.SH & extratreereg & 21.58  & 0.15  & 41803.0  & 238.7  & 0.914  & 0.003  & -0.1018  & 0.0179  & -1.21E-06 & 3.30E-07 \\ 
    \bottomrule
    \end{tabular}
    \caption{Baselines. Short position with lastprice.}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{l|l|cc|cc|cc|cc|cc}
    \toprule
        etf & method & Precision(\%) &  & Trans &  & PLR &  & MDD &  & OTR &  \\ 
    \midrule
        512880.SH & ols & 48.93  & 0.03  & 13371.8  & 13.9  & 0.953  & 0.002  & -0.0732  & 0.0007  & 9.37E-05 & 1.51E-07 \\ 
        512880.SH & gls & 48.93  & 0.03  & 13371.8  & 13.9  & 0.953  & 0.002  & -0.0732  & 0.0007  & 9.37E-05 & 1.51E-07 \\ 
        512880.SH & glsar & 48.92  & 0.03  & 13373.4  & 14.2  & 0.953  & 0.002  & -0.0732  & 0.0007  & 9.37E-05 & 1.83E-07 \\ 
        512880.SH & autoreg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E49 & 0.00E49 \\ 
        512880.SH & arima & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E50 & 0.00E50 \\ 
        512880.SH & expsmooth & 4.54  & 10.15  & 3612.6  & 8078.0  & 0.197  & 0.441  & -0.0668  & 0.1493  & -3.64E-06 & 8.13E-06 \\ 
        512880.SH & ets & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E52 & 0.00E52 \\ 
        512880.SH & linearreg & 48.93  & 0.03  & 13371.8  & 13.9  & 0.953  & 0.002  & -0.0732  & 0.0007  & 9.37E-05 & 1.51E-07 \\ 
        512880.SH & ridge & 48.30  & 0.06  & 5384.6  & 19.7  & 0.962  & 0.002  & -0.0382  & 0.0000  & 1.96E-04 & 4.43E-07 \\ 
        512880.SH & lasso & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E55 & 0.00E55 \\ 
        512880.SH & elasticnet & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E56 & 0.00E56 \\ 
        512880.SH & lassolars & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E57 & 0.00E57 \\ 
        512880.SH & bayesianridge & 48.95  & 0.04  & 13369.2  & 13.3  & 0.955  & 0.002  & -0.0728  & 0.0007  & 9.40E-05 & 1.85E-07 \\ 
        512880.SH & PassiveAggressiveReg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E59 & 0.00E59 \\ 
        512880.SH & sgdreg & 33.49  & 0.22  & 45121.2  & 160.4  & 0.964  & 0.003  & -0.2946  & 0.0045  & -5.78E-06 & 2.07E-07 \\ 
        512880.SH & svr & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E61 & 0.00E61 \\ 
        512880.SH & mlpreg & 27.03  & 3.77  & 21329.2  & 24622.4  & 0.977  & 0.043  & -0.1939  & 0.0886  & -5.60E-06 & 2.75E-05 \\ 
        512880.SH & knnreg & 27.98  & 0.06  & 14348.4  & 66.6  & 0.904  & 0.002  & -0.1289  & 0.0048  & 3.09E-06 & 4.94E-07 \\ 
        512880.SH & adareg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E64 & 0.00E64 \\ 
        512880.SH & gbreg & 45.82  & 0.39  & 15410.0  & 236.6  & 0.958  & 0.004  & -0.1283  & 0.0020  & 7.18E-05 & 1.10E-06 \\ 
        512880.SH & baggingreg & 43.12  & 0.42  & 19097.4  & 203.2  & 0.910  & 0.005  & -0.0927  & 0.0122  & 3.73E-05 & 2.14E-06 \\ 
        512880.SH & extratreereg & 33.22  & 0.17  & 45270.6  & 194.8  & 0.965  & 0.007  & -0.3008  & 0.0046  & -6.04E-06 & 1.50E-07 \\ 
    \midrule
        515050.SH & ols & 25.21  & 0.01  & 15068.2  & 2.2  & 0.986  & 0.000  & -0.0088  & 0.0000  & 9.28E-05 & 1.44E-07 \\ 
        515050.SH & gls & 25.21  & 0.01  & 15068.2  & 2.2  & 0.986  & 0.000  & -0.0088  & 0.0000  & 9.28E-05 & 1.44E-07 \\ 
        515050.SH & glsar & 25.21  & 0.00  & 15068.6  & 2.5  & 0.986  & 0.000  & -0.0088  & 0.0000  & 9.28E-05 & 1.41E-07 \\ 
        515050.SH & autoreg & 0.00  & 0.00  & 9.0  & 0.0  & 0.999  & 0.000  & -0.0009  & 0.0000  & 1.02E-04 & 0.00E72 \\ 
        515050.SH & arima & 0.00  & 0.00  & 5.0  & 0.0  & 1.499  & 0.000  & -0.0009  & 0.0000  & 1.84E-04 & 0.00E73 \\ 
        515050.SH & expsmooth & 7.88  & 0.00  & 92417.0  & 0.0  & 0.999  & 0.000  & -0.1887  & 0.0000  & -1.94E-06 & 0.00E74 \\ 
        515050.SH & ets & 7.88  & 0.00  & 92417.0  & 0.0  & 0.999  & 0.000  & -0.1887  & 0.0000  & -1.94E-06 & 0.00E75 \\ 
        515050.SH & linearreg & 25.21  & 0.01  & 15068.2  & 2.2  & 0.986  & 0.000  & -0.0088  & 0.0000  & 9.28E-05 & 1.44E-07 \\ 
        515050.SH & ridge & 22.04  & 0.01  & 14555.2  & 11.0  & 0.985  & 0.000  & -0.0096  & 0.0000  & 7.52E-05 & 1.23E-07 \\ 
        515050.SH & lasso & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E78 & 0.00E78 \\ 
        515050.SH & elasticnet & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E79 & 0.00E79 \\ 
        515050.SH & lassolars & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E80 & 0.00E80 \\ 
        515050.SH & bayesianridge & 25.22  & 0.02  & 15071.8  & 6.9  & 0.987  & 0.001  & -0.0088  & 0.0000  & 9.28E-05 & 9.12E-08 \\ 
        515050.SH & PassiveAggressiveReg & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E82 & 0.00E82 \\ 
        515050.SH & sgdreg & 13.12  & 0.08  & 42414.0  & 381.8  & 0.963  & 0.002  & -0.0963  & 0.0056  & -1.28E-06 & 2.19E-07 \\ 
        515050.SH & svr & 0.00  & 0.00  & 0.0  & 0.0  & 0.000  & 0.000  & 0.0000  & 0.0000  & 0.00E84 & 0.00E84 \\ 
        515050.SH & mlpreg & 11.98  & 4.56  & 47846.8  & 32086.8  & 0.993  & 0.010  & -0.1122  & 0.0800  & 1.87E-05 & 3.32E-05 \\ 
        515050.SH & knnreg & 13.60  & 0.02  & 27247.2  & 29.4  & 0.954  & 0.001  & -0.0240  & 0.0000  & 1.49E-05 & 2.08E-07 \\ 
        515050.SH & adareg & 42.21  & 5.05  & 922.4  & 345.8  & 1.161  & 0.029  & -0.0039  & 0.0010  & 3.40E-04 & 4.14E-05 \\ 
        515050.SH & gbreg & 21.94  & 0.14  & 19902.2  & 158.1  & 0.977  & 0.001  & -0.0085  & 0.0005  & 6.03E-05 & 8.53E-07 \\ 
        515050.SH & baggingreg & 18.98  & 0.09  & 24368.4  & 218.1  & 0.964  & 0.003  & -0.0159  & 0.0023  & 3.59E-05 & 1.38E-06 \\ 
        515050.SH & extratreereg & 12.64  & 0.10  & 43676.8  & 232.0  & 0.967  & 0.003  & -0.1099  & 0.0040  & -1.83E-06 & 1.27E-07 \\ 
    \bottomrule
    \end{tabular}
    \caption{Baselines. Short position with lastprice.}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{l|l|cc|cc|cc|cc|cc}
    \toprule
        etf & method & Precision(\%) &  & Trans &  & PLR &  & MDD &  & OTR &  \\ 
    \midrule
        159915.SZ & ols & 43.12  & 0.04  & 1000 & 0 & 2.1372  & 0.0057  & -0.0082  & 0.0000  & 1.17E-03 & 1.87E-06 \\ 
        159915.SZ & gls & 43.12  & 0.04  & 1000 & 0 & 2.1372  & 0.0057  & -0.0082  & 0.0000  & 1.17E-03 & 1.87E-06 \\ 
        159915.SZ & glsar & 43.12  & 0.04  & 1000 & 0 & 2.1364  & 0.0062  & -0.0082  & 0.0000  & 1.17E-03 & 1.52E-06 \\ 
        159915.SZ & autoreg & 4.56  & 0.05  & 1000 & 0 & 2.1809  & 0.0502  & -0.0426  & 0.0000  & 1.03E-03 & 5.72E-05 \\ 
        159915.SZ & arima & 5.60  & 0.00  & 1000 & 0 & 4.2400  & 0.0000  & -0.0426  & 0.0000  & 1.81E-03 & 2.42E-19 \\ 
        159915.SZ & expsmooth & 5.08  & 0.41  & 1000 & 0 & 0.7414  & 0.1822  & -0.6880  & 0.3254  & -8.45E-04 & 7.59E-04 \\ 
        159915.SZ & ets & 5.60  & 0.00  & 1000 & 0 & 4.1275  & 0.0000  & -0.0426  & 0.0000  & 1.81E-03 & 2.42E-19 \\ 
        159915.SZ & linearreg & 43.12  & 0.04  & 1000 & 0 & 2.1372  & 0.0057  & -0.0082  & 0.0000  & 1.17E-03 & 1.87E-06 \\ 
        159915.SZ & ridge & 43.12  & 0.15  & 1000 & 0 & 2.0517  & 0.0144  & -0.0058  & 0.0000  & 1.01E-03 & 1.99E-06 \\ 
        159915.SZ & lasso & 5.60  & 0.00  & 1000 & 0 & 4.1275  & 0.0000  & -0.0426  & 0.0000  & 1.81E-03 & 2.42E-19 \\ 
        159915.SZ & elasticnet & 5.60  & 0.00  & 1000 & 0 & 4.1275  & 0.0000  & -0.0426  & 0.0000  & 1.81E-03 & 2.42E-19 \\ 
        159915.SZ & lassolars & 5.60  & 0.00  & 1000 & 0 & 4.1275  & 0.0000  & -0.0426  & 0.0000  & 1.81E-03 & 2.42E-19 \\ 
        159915.SZ & bayesianridge & 43.12  & 0.15  & 1000 & 0 & 2.1256  & 0.0084  & -0.0082  & 0.0000  & 1.17E-03 & 2.96E-06 \\ 
        159915.SZ & PassiveAggressiveReg & 5.60  & 0.00  & 1000 & 0 & 4.1275  & 0.0000  & -0.0426  & 0.0000  & 1.81E-03 & 2.42E-19 \\ 
        159915.SZ & sgdreg & 16.66  & 2.13  & 1000 & 0 & 1.2974  & 0.0643  & -0.0134  & 0.0062  & 4.45E-04 & 4.23E-05 \\ 
        159915.SZ & svr & 5.60  & 0.00  & 1000 & 0 & 4.1275  & 0.0000  & -0.0426  & 0.0000  & 1.81E-03 & 2.42E-19 \\ 
        159915.SZ & mlpreg & 10.76  & 6.64  & 1000 & 0 & 1.1547  & 0.3050  & -0.0769  & 0.0643  & 2.80E-04 & 2.58E-04 \\ 
        159915.SZ & knnreg & 15.46  & 0.65  & 1000 & 0 & 1.3749  & 0.0204  & -0.0111  & 0.0020  & 4.57E-04 & 8.90E-06 \\ 
        159915.SZ & adareg & 29.16  & 2.94  & 1000 & 0 & 1.6978  & 0.1872  & -0.0303  & 0.0110  & 8.30E-04 & 1.20E-04 \\ 
        159915.SZ & gbreg & 43.86  & 0.47  & 1000 & 0 & 2.4976  & 0.1110  & -0.0029  & 0.0006  & 1.21E-03 & 2.40E-05 \\ 
        159915.SZ & baggingreg & 30.88  & 0.68  & 1000 & 0 & 1.9799  & 0.1016  & -0.0046  & 0.0008  & 9.03E-04 & 2.88E-05 \\ 
        159915.SZ & extratreereg & 14.20  & 1.12  & 1000 & 0 & 1.3437  & 0.1231  & -0.0113  & 0.0056  & 3.69E-04 & 6.61E-05 \\ 
    \midrule
        512480.SH & ols & 81.66  & 0.09  & 1000 & 0 & 2.7672  & 0.0023  & -0.0127  & 0.0000  & 2.44E-03 & 2.07E-06 \\ 
        512480.SH & gls & 81.66  & 0.09  & 1000 & 0 & 2.7672  & 0.0023  & -0.0127  & 0.0000  & 2.44E-03 & 2.07E-06 \\ 
        512480.SH & glsar & 81.66  & 0.09  & 1000 & 0 & 2.7672  & 0.0023  & -0.0127  & 0.0000  & 2.44E-03 & 2.07E-06 \\ 
        512480.SH & autoreg & 12.18  & 0.18  & 1000 & 0 & 1.0136  & 0.0109  & -1.0000  & 0.0000  & -1.31E-03 & 3.70E-05 \\ 
        512480.SH & arima & 23.52  & 1.03  & 1000 & 0 & 3.3989  & 0.3367  & -0.5926  & 0.1409  & 3.32E-03 & 4.84E-04 \\ 
        512480.SH & expsmooth & 18.28  & 1.39  & 1000 & 0 & 2.6570  & 1.8237  & -0.5443  & 0.0774  & 3.35E-03 & 1.14E-03 \\ 
        512480.SH & ets & 5.20  & 0.00  & 1000 & 0 & 0.2635  & 0.0000  & -1.0000  & 0.0000  & -1.75E-03 & 2.42E-19 \\ 
        512480.SH & linearreg & 81.66  & 0.09  & 1000 & 0 & 2.7672  & 0.0023  & -0.0127  & 0.0000  & 2.44E-03 & 2.07E-06 \\ 
        512480.SH & ridge & 81.64  & 0.15  & 1000 & 0 & 3.9930  & 0.0136  & -0.0031  & 0.0000  & 2.15E-03 & 2.75E-06 \\ 
        512480.SH & lasso & 5.20  & 0.00  & 1000 & 0 & 0.2635  & 0.0000  & -1.0000  & 0.0000  & -1.75E-03 & 2.42E-19 \\ 
        512480.SH & elasticnet & 5.20  & 0.00  & 1000 & 0 & 0.2635  & 0.0000  & -1.0000  & 0.0000  & -1.75E-03 & 2.42E-19 \\ 
        512480.SH & lassolars & 5.20  & 0.00  & 1000 & 0 & 0.2635  & 0.0000  & -1.0000  & 0.0000  & -1.75E-03 & 2.42E-19 \\ 
        512480.SH & bayesianridge & 81.64  & 0.15  & 1000 & 0 & 2.6740  & 0.2132  & -0.0127  & 0.0000  & 2.44E-03 & 7.26E-06 \\ 
        512480.SH & PassiveAggressiveReg & 5.20  & 0.00  & 1000 & 0 & 0.2635  & 0.0000  & -1.0000  & 0.0000  & -1.75E-03 & 2.42E-19 \\ 
        512480.SH & sgdreg & 35.60  & 1.43  & 1000 & 0 & 1.7419  & 0.0873  & -0.0190  & 0.0031  & 9.09E-04 & 5.66E-05 \\ 
        512480.SH & svr & 5.20  & 0.00  & 1000 & 0 & 0.2635  & 0.0000  & -1.0000  & 0.0000  & -1.75E-03 & 2.42E-19 \\ 
        512480.SH & mlpreg & 50.62  & 15.99  & 1000 & 0 & 2.0782  & 0.5923  & -0.0374  & 0.0255  & 1.34E-03 & 5.30E-04 \\ 
        512480.SH & knnreg & 42.28  & 0.31  & 1000 & 0 & 2.2000  & 0.0374  & -0.0129  & 0.0002  & 1.11E-03 & 1.39E-05 \\ 
        512480.SH & adareg & 36.22  & 4.55  & 1000 & 0 & 2.1746  & 0.2690  & -0.0192  & 0.0062  & 1.02E-03 & 1.53E-04 \\ 
        512480.SH & gbreg & 79.62  & 0.36  & 1000 & 0 & 2.9550  & 0.0574  & -0.0176  & 0.0003  & 2.43E-03 & 2.11E-05 \\ 
        512480.SH & baggingreg & 66.28  & 1.54  & 1000 & 0 & 2.7310  & 0.2925  & -0.0120  & 0.0028  & 2.05E-03 & 7.20E-05 \\ 
        512480.SH & extratreereg & 35.88  & 2.27  & 1000 & 0 & 1.8200  & 0.0979  & -0.0202  & 0.0068  & 9.16E-04 & 1.09E-04 \\ 
    \bottomrule
    \end{tabular}
    \caption{Baselines. Long position with lastprice condition on 1000 trades.}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{l|l|cc|cc|cc|cc|cc}
    \toprule
        etf & method & Precision(\%) &  & Trans &  & PLR &  & MDD &  & OTR &  \\ 
    \midrule
        512880.SH & ols & 64.44  & 0.11  & 1000 & 0 & 0.9941  & 0.0142  & -0.2227  & 0.0000  & 1.77E-03 & 1.12E-05 \\ 
        512880.SH & gls & 64.44  & 0.11  & 1000 & 0 & 0.9941  & 0.0142  & -0.2227  & 0.0000  & 1.77E-03 & 1.12E-05 \\ 
        512880.SH & glsar & 64.48  & 0.13  & 1000 & 0 & 0.9956  & 0.0150  & -0.2227  & 0.0000  & 1.77E-03 & 1.10E-05 \\ 
        512880.SH & autoreg & 14.22  & 6.36  & 1000 & 0 & 1.1171  & 0.2154  & -0.3160  & 0.1341  & -3.63E-05 & 1.66E-04 \\ 
        512880.SH & arima & 8.88  & 0.18  & 1000 & 0 & 1.6555  & 0.1214  & -0.1844  & 0.0619  & 8.40E-04 & 1.33E-04 \\ 
        512880.SH & expsmooth & 22.86  & 3.68  & 1000 & 0 & 1.8316  & 1.7105  & -0.5141  & 0.3316  & 6.51E-04 & 1.73E-03 \\ 
        512880.SH & ets & 8.70  & 0.00  & 1000 & 0 & 1.6028  & 0.0000  & -0.2121  & 0.0000  & 7.77E-04 & 0.00E52 \\ 
        512880.SH & linearreg & 64.44  & 0.11  & 1000 & 0 & 0.9941  & 0.0142  & -0.2227  & 0.0000  & 1.77E-03 & 1.12E-05 \\ 
        512880.SH & ridge & 64.58  & 0.13  & 1000 & 0 & 1.3660  & 0.0050  & -0.0796  & 0.0000  & 1.87E-03 & 8.92E-06 \\ 
        512880.SH & lasso & 8.70  & 0.00  & 1000 & 0 & 1.6028  & 0.0000  & -0.2121  & 0.0000  & 7.77E-04 & 0.00E55 \\ 
        512880.SH & elasticnet & 8.70  & 0.00  & 1000 & 0 & 1.6028  & 0.0000  & -0.2121  & 0.0000  & 7.77E-04 & 0.00E56 \\ 
        512880.SH & lassolars & 8.70  & 0.00  & 1000 & 0 & 1.6028  & 0.0000  & -0.2121  & 0.0000  & 7.77E-04 & 0.00E57 \\ 
        512880.SH & bayesianridge & 64.58  & 0.13  & 1000 & 0 & 0.9545  & 0.0025  & -0.2320  & 0.0000  & 1.81E-03 & 4.90E-06 \\ 
        512880.SH & PassiveAggressiveReg & 8.70  & 0.00  & 1000 & 0 & 1.6028  & 0.0000  & -0.2121  & 0.0000  & 7.77E-04 & 0.00E59 \\ 
        512880.SH & sgdreg & 38.84  & 2.72  & 1000 & 0 & 1.1832  & 0.2335  & -0.1201  & 0.0752  & 1.01E-03 & 2.34E-04 \\ 
        512880.SH & svr & 8.70  & 0.00  & 1000 & 0 & 1.6028  & 0.0000  & -0.2121  & 0.0000  & 7.77E-04 & 0.00E61 \\ 
        512880.SH & mlpreg & 37.24  & 6.25  & 1000 & 0 & 0.9113  & 0.5415  & -0.8354  & 0.2327  & 4.14E-04 & 1.35E-03 \\ 
        512880.SH & knnreg & 40.20  & 0.49  & 1000 & 0 & 1.3210  & 0.0653  & -0.0625  & 0.0058  & 9.42E-04 & 5.76E-05 \\ 
        512880.SH & adareg & 46.36  & 6.06  & 1000 & 0 & 1.2094  & 0.2200  & -0.1725  & 0.0299  & 1.42E-03 & 4.98E-04 \\ 
        512880.SH & gbreg & 47.62  & 1.02  & 1000 & 0 & 1.3313  & 0.1198  & -0.0826  & 0.0188  & 1.48E-03 & 7.78E-05 \\ 
        512880.SH & baggingreg & 47.54  & 1.30  & 1000 & 0 & 1.3653  & 0.1042  & -0.0793  & 0.0217  & 1.55E-03 & 1.74E-04 \\ 
        512880.SH & extratreereg & 39.00  & 3.07  & 1000 & 0 & 1.3188  & 0.1772  & -0.1472  & 0.0730  & 1.03E-03 & 3.14E-04 \\ 
    \midrule
        515050.SH & ols & 55.22  & 0.08  & 1000 & 0 & 1.6669  & 0.0042  & -0.0081  & 0.0000  & 1.47E-03 & 4.01E-06 \\ 
        515050.SH & gls & 55.22  & 0.08  & 1000 & 0 & 1.6669  & 0.0042  & -0.0081  & 0.0000  & 1.47E-03 & 4.01E-06 \\ 
        515050.SH & glsar & 55.24  & 0.05  & 1000 & 0 & 1.6709  & 0.0053  & -0.0081  & 0.0000  & 1.47E-03 & 9.99E-07 \\ 
        515050.SH & autoreg & 11.16  & 0.35  & 1000 & 0 & 3.2722  & 0.1903  & -0.0184  & 0.0146  & 2.75E-03 & 2.55E-04 \\ 
        515050.SH & arima & 11.50  & 0.00  & 1000 & 0 & 2.9546  & 0.0000  & -0.0324  & 0.0000  & 2.49E-03 & 0.00E73 \\ 
        515050.SH & expsmooth & 8.08  & 1.29  & 1000 & 0 & 1.4976  & 0.6174  & -0.6688  & 0.3679  & 8.82E-04 & 1.13E-03 \\ 
        515050.SH & ets & 11.40  & 0.00  & 1000 & 0 & 2.8859  & 0.0000  & -0.0324  & 0.0000  & 2.48E-03 & 0.00E75 \\ 
        515050.SH & linearreg & 55.22  & 0.08  & 1000 & 0 & 1.6669  & 0.0042  & -0.0081  & 0.0000  & 1.47E-03 & 4.01E-06 \\ 
        515050.SH & ridge & 55.52  & 0.13  & 1000 & 0 & 1.4807  & 0.0035  & -0.0080  & 0.0000  & 1.21E-03 & 1.77E-06 \\ 
        515050.SH & lasso & 11.40  & 0.00  & 1000 & 0 & 2.8859  & 0.0000  & -0.0324  & 0.0000  & 2.48E-03 & 0.00E78 \\ 
        515050.SH & elasticnet & 11.40  & 0.00  & 1000 & 0 & 2.8859  & 0.0000  & -0.0324  & 0.0000  & 2.48E-03 & 0.00E79 \\ 
        515050.SH & lassolars & 11.40  & 0.00  & 1000 & 0 & 2.8859  & 0.0000  & -0.0324  & 0.0000  & 2.48E-03 & 0.00E80 \\ 
        515050.SH & bayesianridge & 55.52  & 0.13  & 1000 & 0 & 1.6720  & 0.0047  & -0.0081  & 0.0000  & 1.48E-03 & 2.30E-06 \\ 
        515050.SH & PassiveAggressiveReg & 11.40  & 0.00  & 1000 & 0 & 2.8859  & 0.0000  & -0.0324  & 0.0000  & 2.48E-03 & 0.00E82 \\ 
        515050.SH & sgdreg & 20.52  & 1.13  & 1000 & 0 & 1.2582  & 0.0769  & -0.0200  & 0.0084  & 4.78E-04 & 4.31E-05 \\ 
        515050.SH & svr & 11.40  & 0.00  & 1000 & 0 & 2.8859  & 0.0000  & -0.0324  & 0.0000  & 2.48E-03 & 0.00E84 \\ 
        515050.SH & mlpreg & 16.82  & 3.81  & 1000 & 0 & 1.1545  & 0.0852  & -0.0555  & 0.0396  & 3.49E-04 & 1.92E-04 \\ 
        515050.SH & knnreg & 20.64  & 0.22  & 1000 & 0 & 1.2380  & 0.0345  & -0.0285  & 0.0062  & 4.85E-04 & 2.49E-05 \\ 
        515050.SH & adareg & 35.54  & 3.23  & 1000 & 0 & 1.4282  & 0.1420  & -0.0248  & 0.0046  & 1.01E-03 & 1.12E-04 \\ 
        515050.SH & gbreg & 51.78  & 0.29  & 1000 & 0 & 1.8225  & 0.0257  & -0.0057  & 0.0007  & 1.41E-03 & 8.59E-06 \\ 
        515050.SH & baggingreg & 41.68  & 1.20  & 1000 & 0 & 1.6431  & 0.1014  & -0.0181  & 0.0062  & 1.19E-03 & 4.84E-05 \\ 
        515050.SH & extratreereg & 19.22  & 0.99  & 1000 & 0 & 1.3188  & 0.0369  & -0.0209  & 0.0090  & 4.45E-04 & 4.32E-05 \\ 
    \bottomrule
    \end{tabular}
    \caption{Baselines. Long position with lastprice condition on 1000 trades.}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{l|l|cc|cc|cc|cc|cc}
    \toprule
        etf & method & Precision(\%) &  & Trans &  & PLR &  & MDD &  & OTR &  \\ 
    \midrule
        159915.SZ & ols & 46.22  & 0.13  & 1000 & 0 & 2.648  & 0.064  & -0.0019  & 0.0000  & 1.19E-03 & 3.75E-06 \\ 
        159915.SZ & gls & 46.22  & 0.13  & 1000 & 0 & 2.648  & 0.064  & -0.0019  & 0.0000  & 1.19E-03 & 3.75E-06 \\ 
        159915.SZ & glsar & 46.22  & 0.13  & 1000 & 0 & 2.647  & 0.064  & -0.0019  & 0.0000  & 1.19E-03 & 3.97E-06 \\ 
        159915.SZ & autoreg & 2.26  & 0.09  & 1000 & 0 & 0.389  & 0.005  & -0.9937  & 0.0138  & -1.01E-03 & 5.27E-05 \\ 
        159915.SZ & arima & 2.90  & 0.00  & 1000 & 0 & 0.233  & 0.014  & -1.0000  & 0.0000  & -1.69E-03 & 1.28E-04 \\ 
        159915.SZ & expsmooth & 5.50  & 0.83  & 1000 & 0 & 1.324  & 0.908  & -0.3456  & 0.2016  & 5.01E-04 & 1.05E-03 \\ 
        159915.SZ & ets & 3.10  & 0.00  & 1000 & 0 & 0.314  & 0.000  & -1.0000  & 0.0000  & -1.33E-03 & 0.00E6 \\ 
        159915.SZ & linearreg & 46.22  & 0.13  & 1000 & 0 & 2.648  & 0.064  & -0.0019  & 0.0000  & 1.19E-03 & 3.75E-06 \\ 
        159915.SZ & ridge & 46.38  & 0.16  & 1000 & 0 & 2.437  & 0.030  & -0.0022  & 0.0000  & 1.10E-03 & 2.66E-06 \\ 
        159915.SZ & lasso & 3.10  & 0.00  & 1000 & 0 & 0.314  & 0.000  & -1.0000  & 0.0000  & -1.33E-03 & 0.00E9 \\ 
        159915.SZ & elasticnet & 3.10  & 0.00  & 1000 & 0 & 0.314  & 0.000  & -1.0000  & 0.0000  & -1.33E-03 & 0.00E10 \\ 
        159915.SZ & lassolars & 3.10  & 0.00  & 1000 & 0 & 0.314  & 0.000  & -1.0000  & 0.0000  & -1.33E-03 & 0.00E11 \\ 
        159915.SZ & bayesianridge & 46.38  & 0.16  & 1000 & 0 & 2.688  & 0.010  & -0.0019  & 0.0000  & 1.19E-03 & 4.32E-06 \\ 
        159915.SZ & PassiveAggressiveReg & 3.10  & 0.00  & 1000 & 0 & 0.314  & 0.000  & -1.0000  & 0.0000  & -1.33E-03 & 0.00E13 \\ 
        159915.SZ & sgdreg & 16.26  & 3.34  & 1000 & 0 & 1.462  & 0.162  & -0.0122  & 0.0032  & 4.33E-04 & 9.50E-05 \\ 
        159915.SZ & svr & 3.10  & 0.00  & 1000 & 0 & 0.314  & 0.000  & -1.0000  & 0.0000  & -1.33E-03 & 0.00E15 \\ 
        159915.SZ & mlpreg & 8.00  & 5.02  & 1000 & 0 & 1.033  & 0.275  & -0.2322  & 0.1458  & -6.80E-05 & 3.04E-04 \\ 
        159915.SZ & knnreg & 16.36  & 0.28  & 1000 & 0 & 1.449  & 0.011  & -0.0126  & 0.0022  & 4.50E-04 & 6.70E-06 \\ 
        159915.SZ & adareg & 35.16  & 1.36  & 1000 & 0 & 2.016  & 0.233  & -0.0055  & 0.0015  & 1.00E-03 & 2.69E-05 \\ 
        159915.SZ & gbreg & 45.36  & 0.41  & 1000 & 0 & 2.067  & 0.073  & -0.0047  & 0.0008  & 1.19E-03 & 2.13E-05 \\ 
        159915.SZ & baggingreg & 31.12  & 3.77  & 1000 & 0 & 1.869  & 0.105  & -0.0084  & 0.0021  & 8.71E-04 & 5.16E-05 \\ 
        159915.SZ & extratreereg & 15.98  & 1.27  & 1000 & 0 & 1.326  & 0.086  & -0.0161  & 0.0067  & 3.55E-04 & 4.67E-05 \\ 
    \midrule
        512480.SH & ols & 22.78  & 0.33  & 1000 & 0 & 2.548  & 0.022  & -0.1612  & 0.0019  & 2.65E-03 & 7.68E-06 \\ 
        512480.SH & gls & 22.78  & 0.33  & 1000 & 0 & 2.548  & 0.022  & -0.1612  & 0.0019  & 2.65E-03 & 7.68E-06 \\ 
        512480.SH & glsar & 22.78  & 0.33  & 1000 & 0 & 2.548  & 0.022  & -0.1612  & 0.0019  & 2.65E-03 & 7.68E-06 \\ 
        512480.SH & autoreg & 13.00  & 0.45  & 1000 & 0 & 1.462  & 0.365  & -0.5337  & 0.1927  & 1.72E-03 & 2.19E-04 \\ 
        512480.SH & arima & 7.70  & 0.00  & 1000 & 0 & 3.808  & 0.000  & -0.0155  & 0.0000  & 1.75E-03 & 0.00E27 \\ 
        512480.SH & expsmooth & 17.58  & 1.52  & 1000 & 0 & 1.503  & 1.488  & -0.6809  & 0.1788  & 6.98E-04 & 2.22E-03 \\ 
        512480.SH & ets & 7.70  & 0.00  & 1000 & 0 & 3.809  & 0.000  & -0.0155  & 0.0000  & 1.75E-03 & 0.00E29 \\ 
        512480.SH & linearreg & 22.78  & 0.33  & 1000 & 0 & 2.548  & 0.022  & -0.1612  & 0.0019  & 2.65E-03 & 7.68E-06 \\ 
        512480.SH & ridge & 22.82  & 0.35  & 1000 & 0 & 3.630  & 0.037  & -0.0884  & 0.0017  & 3.56E-03 & 5.22E-06 \\ 
        512480.SH & lasso & 7.70  & 0.00  & 1000 & 0 & 3.809  & 0.000  & -0.0155  & 0.0000  & 1.75E-03 & 0.00E32 \\ 
        512480.SH & elasticnet & 7.70  & 0.00  & 1000 & 0 & 3.809  & 0.000  & -0.0155  & 0.0000  & 1.75E-03 & 0.00E33 \\ 
        512480.SH & lassolars & 7.70  & 0.00  & 1000 & 0 & 3.809  & 0.000  & -0.0155  & 0.0000  & 1.75E-03 & 0.00E34 \\ 
        512480.SH & bayesianridge & 22.82  & 0.35  & 1000 & 0 & 2.571  & 0.010  & -0.1604  & 0.0000  & 2.65E-03 & 9.25E-06 \\ 
        512480.SH & PassiveAggressiveReg & 7.70  & 0.00  & 1000 & 0 & 3.809  & 0.000  & -0.0155  & 0.0000  & 1.75E-03 & 0.00E36 \\ 
        512480.SH & sgdreg & 33.32  & 1.47  & 1000 & 0 & 1.527  & 0.252  & -0.0436  & 0.0267  & 7.66E-04 & 9.61E-05 \\ 
        512480.SH & svr & 7.70  & 0.00  & 1000 & 0 & 3.809  & 0.000  & -0.0155  & 0.0000  & 1.75E-03 & 0.00E38 \\ 
        512480.SH & mlpreg & 36.44  & 19.79  & 1000 & 0 & 2.284  & 0.414  & -0.0841  & 0.0910  & 1.70E-03 & 6.73E-04 \\ 
        512480.SH & knnreg & 34.50  & 0.66  & 1000 & 0 & 2.401  & 0.152  & -0.0146  & 0.0017  & 1.09E-03 & 2.76E-05 \\ 
        512480.SH & adareg & 66.48  & 1.82  & 1000 & 0 & 2.230  & 0.258  & -0.0188  & 0.0024  & 1.79E-03 & 8.20E-05 \\ 
        512480.SH & gbreg & 69.78  & 1.42  & 1000 & 0 & 2.612  & 0.227  & -0.0207  & 0.0076  & 2.20E-03 & 8.76E-05 \\ 
        512480.SH & baggingreg & 57.98  & 1.54  & 1000 & 0 & 2.463  & 0.144  & -0.0168  & 0.0061  & 1.88E-03 & 4.91E-05 \\ 
        512480.SH & extratreereg & 32.66  & 2.94  & 1000 & 0 & 1.546  & 0.240  & -0.0307  & 0.0118  & 7.91E-04 & 1.67E-04 \\ 
    \bottomrule
    \end{tabular}
    \caption{Baselines. Short position with lastprice condition on 1000 trades.}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{l|l|cc|cc|cc|cc|cc}
    \toprule
        etf & method & Precision(\%) &  & Trans &  & PLR &  & MDD &  & OTR &  \\ 
    \midrule
        512880.SH & ols & 39.46  & 0.18  & 1000 & 0 & 0.495  & 0.002  & -1.0000  & 0.0000  & -1.52E-03 & 2.41E-05 \\ 
        512880.SH & gls & 39.46  & 0.18  & 1000 & 0 & 0.495  & 0.002  & -1.0000  & 0.0000  & -1.52E-03 & 2.41E-05 \\ 
        512880.SH & glsar & 39.48  & 0.16  & 1000 & 0 & 0.495  & 0.002  & -1.0000  & 0.0000  & -1.52E-03 & 2.27E-05 \\ 
        512880.SH & autoreg & 12.94  & 7.25  & 1000 & 0 & 0.679  & 0.111  & -0.5631  & 0.2445  & -5.78E-04 & 1.11E-03 \\ 
        512880.SH & arima & 11.20  & 0.12  & 1000 & 0 & 0.676  & 0.035  & -0.6101  & 0.0000  & 1.27E-04 & 2.74E-05 \\ 
        512880.SH & expsmooth & 18.68  & 2.89  & 1000 & 0 & 1.516  & 0.628  & -0.5620  & 0.4012  & 5.80E-04 & 1.00E-03 \\ 
        512880.SH & ets & 7.90  & 0.00  & 1000 & 0 & 0.623  & 0.000  & -1.0000  & 0.0000  & -7.83E-04 & 0.00E52 \\ 
        512880.SH & linearreg & 39.46  & 0.18  & 1000 & 0 & 0.495  & 0.002  & -1.0000  & 0.0000  & -1.52E-03 & 2.41E-05 \\ 
        512880.SH & ridge & 39.34  & 0.09  & 1000 & 0 & 0.983  & 0.005  & -0.3403  & 0.0068  & 1.03E-03 & 3.82E-06 \\ 
        512880.SH & lasso & 7.90  & 0.00  & 1000 & 0 & 0.623  & 0.000  & -1.0000  & 0.0000  & -7.83E-04 & 0.00E55 \\ 
        512880.SH & elasticnet & 7.90  & 0.00  & 1000 & 0 & 0.623  & 0.000  & -1.0000  & 0.0000  & -7.83E-04 & 0.00E56 \\ 
        512880.SH & lassolars & 7.90  & 0.00  & 1000 & 0 & 0.623  & 0.000  & -1.0000  & 0.0000  & -7.83E-04 & 0.00E57 \\ 
        512880.SH & bayesianridge & 39.34  & 0.09  & 1000 & 0 & 0.498  & 0.001  & -1.0000  & 0.0000  & -1.49E-03 & 1.87E-05 \\ 
        512880.SH & PassiveAggressiveReg & 7.90  & 0.00  & 1000 & 0 & 0.623  & 0.000  & -1.0000  & 0.0000  & -7.83E-04 & 0.00E59 \\ 
        512880.SH & sgdreg & 30.10  & 4.04  & 1000 & 0 & 0.855  & 0.116  & -0.4168  & 0.2311  & 1.23E-04 & 1.05E-04 \\ 
        512880.SH & svr & 7.90  & 0.00  & 1000 & 0 & 0.623  & 0.000  & -1.0000  & 0.0000  & -7.83E-04 & 0.00E61 \\ 
        512880.SH & mlpreg & 27.24  & 5.16  & 1000 & 0 & 1.111  & 0.394  & -0.4970  & 0.3361  & -1.50E-04 & 1.65E-03 \\ 
        512880.SH & knnreg & 32.50  & 0.47  & 1000 & 0 & 1.541  & 0.042  & -0.1514  & 0.0199  & 8.08E-04 & 6.18E-05 \\ 
        512880.SH & adareg & 54.16  & 2.45  & 1000 & 0 & 1.537  & 0.276  & -0.0279  & 0.0152  & 1.44E-03 & 2.77E-04 \\ 
        512880.SH & gbreg & 42.74  & 1.57  & 1000 & 0 & 1.442  & 0.202  & -0.1586  & 0.0209  & 1.31E-03 & 3.19E-04 \\ 
        512880.SH & baggingreg & 38.84  & 1.99  & 1000 & 0 & 1.038  & 0.218  & -0.2062  & 0.1462  & 9.16E-04 & 2.47E-04 \\ 
        512880.SH & extratreereg & 29.40  & 0.94  & 1000 & 0 & 1.044  & 0.171  & -0.2730  & 0.1354  & 2.55E-04 & 2.29E-04 \\ 
    \midrule
        515050.SH & ols & 55.24  & 0.11  & 1000 & 0 & 1.403  & 0.016  & -0.0212  & 0.0000  & 1.41E-03 & 3.12E-06 \\ 
        515050.SH & gls & 55.24  & 0.11  & 1000 & 0 & 1.403  & 0.016  & -0.0212  & 0.0000  & 1.41E-03 & 3.12E-06 \\ 
        515050.SH & glsar & 55.24  & 0.11  & 1000 & 0 & 1.403  & 0.016  & -0.0212  & 0.0000  & 1.41E-03 & 3.12E-06 \\ 
        515050.SH & autoreg & 7.76  & 0.09  & 1000 & 0 & 0.684  & 0.058  & -1.0000  & 0.0000  & -2.53E-03 & 2.73E-04 \\ 
        515050.SH & arima & 8.50  & 0.00  & 1000 & 0 & 0.137  & 0.000  & -1.0000  & 0.0000  & -3.92E-03 & 0.00E73 \\ 
        515050.SH & expsmooth & 7.12  & 0.50  & 1000 & 0 & 0.739  & 0.246  & -0.9306  & 0.0950  & -7.13E-04 & 6.59E-04 \\ 
        515050.SH & ets & 9.30  & 0.00  & 1000 & 0 & 0.279  & 0.000  & -1.0000  & 0.0000  & -2.92E-03 & 0.00E75 \\ 
        515050.SH & linearreg & 55.24  & 0.11  & 1000 & 0 & 1.403  & 0.016  & -0.0212  & 0.0000  & 1.41E-03 & 3.12E-06 \\ 
        515050.SH & ridge & 55.50  & 0.10  & 1000 & 0 & 1.670  & 0.001  & -0.0073  & 0.0000  & 1.26E-03 & 4.63E-07 \\ 
        515050.SH & lasso & 9.30  & 0.00  & 1000 & 0 & 0.279  & 0.000  & -1.0000  & 0.0000  & -2.92E-03 & 0.00E78 \\ 
        515050.SH & elasticnet & 9.30  & 0.00  & 1000 & 0 & 0.279  & 0.000  & -1.0000  & 0.0000  & -2.92E-03 & 0.00E79 \\ 
        515050.SH & lassolars & 9.30  & 0.00  & 1000 & 0 & 0.279  & 0.000  & -1.0000  & 0.0000  & -2.92E-03 & 0.00E80 \\ 
        515050.SH & bayesianridge & 55.50  & 0.10  & 1000 & 0 & 1.392  & 0.002  & -0.0212  & 0.0000  & 1.41E-03 & 1.50E-06 \\ 
        515050.SH & PassiveAggressiveReg & 9.30  & 0.00  & 1000 & 0 & 0.279  & 0.000  & -1.0000  & 0.0000  & -2.92E-03 & 0.00E82 \\ 
        515050.SH & sgdreg & 20.68  & 3.21  & 1000 & 0 & 1.187  & 0.102  & -0.0320  & 0.0121  & 4.48E-04 & 9.94E-05 \\ 
        515050.SH & svr & 9.30  & 0.00  & 1000 & 0 & 0.279  & 0.000  & -1.0000  & 0.0000  & -2.92E-03 & 0.00E84 \\ 
        515050.SH & mlpreg & 12.42  & 4.92  & 1000 & 0 & 1.106  & 0.115  & -0.0801  & 0.0432  & 2.33E-04 & 2.06E-04 \\ 
        515050.SH & knnreg & 23.94  & 0.38  & 1000 & 0 & 1.348  & 0.023  & -0.0300  & 0.0011  & 6.65E-04 & 1.61E-05 \\ 
        515050.SH & adareg & 40.76  & 1.07  & 1000 & 0 & 1.622  & 0.080  & -0.0186  & 0.0049  & 1.29E-03 & 6.19E-05 \\ 
        515050.SH & gbreg & 55.18  & 0.51  & 1000 & 0 & 1.840  & 0.160  & -0.0046  & 0.0008  & 1.52E-03 & 1.84E-05 \\ 
        515050.SH & baggingreg & 40.22  & 1.18  & 1000 & 0 & 1.455  & 0.113  & -0.0136  & 0.0075  & 1.10E-03 & 4.02E-05 \\ 
        515050.SH & extratreereg & 18.82  & 0.73  & 1000 & 0 & 1.197  & 0.132  & -0.0269  & 0.0160  & 4.27E-04 & 5.90E-05 \\ 
    \bottomrule
    \end{tabular}
    \caption{Baselines. Short position with lastprice condition on 1000 trades.}
\end{table*}


==> Understand.tex <==
\begin{algorithm}[h]
    \small
    % \caption{\fontsize{9pt}{9pt}\selectfont RA-Labeling: Iterative \underline{R}efinement L\underline{a}beling}
    \caption{RA-Labeling}
    \label{alg:Bi-level-label}
    \KwIn{Training data $\left(\mX, \vy^{0}\right) \in \mathbb{R}^{N \times d} \times \mathbb{R}^{N}$, the initial model $f_{\theta_0}: \mathbb{R}^{d} \rightarrow \mathbb{R}$. }
  	\Parameter{Iteration number $K$, combination scheme $C$.}
  	%\KwOut{$f_{\theta_{\left[k\right]}} \in \mathbb{R}^N$.}
  	\KwOut{$F: \mathbb{R}^d \rightarrow \mathbb{R}$}
%   	\textcolor{red}{\sout{Init $f_{\theta_0}$ trained on $(X,Y_0)$.\\}}
  	Init: $\theta^0 = \argmin_{\theta^0} \sum_{j=1}^N \mathcal{L} \left(f_{\theta^0}(\vx_j), y^{0}_j\right)$ \\
    \For{$k \in \left\{0,\dots,K-1\right\}$}{
        % \textcolor{red}{\sout{$\hat{p} = f_{\theta_i}(X)$. }} \\
        \For{$j \in \left\{1,\dots,N\right\}$}{
            \footnotesize
            $y^{k+1}_j = y^{k}_j + (1-2 \cdot y^{k}_j) \cdot \mathbbm{1}\left(\mathcal{L} \left(f_{\theta^k}(\vx_j), y^{k}_j \right) > \epsilon^k\right)$
        }
        % \textcolor{red}{\sout{Sort $\hat{p}$ in descending order to obtain $\left(X, Y_{i+1}\right)$.}} \\
        % \textcolor{red}{\sout{Reset the labels in $Y_{i+1}$ with $r$ according to Eq.~\ref{equ:reset}.}} \\
        % \textcolor{red}{\sout{Retrain $f_{\theta_i}$ according to $(X,Y_{i+1})$ to get $f_{\theta_{i+1}}$.}}\\
        $\theta^{k+1} = \argmin_{\theta^{k+1}} \sum_{j=1}^N \mathcal{L} \left(f_{\theta^{k+1}}(\vx_j), y^{k+1}_j \right)$ \\
    }
    % \textbf{Return:} $f_{\theta_{\left[k\right]}}$ = $F\left(\{f_{\theta_{i}}(\mX), 0 \leq i \leq k\}\right)$. \\
    \textbf{Return:} $F = C\left( \{f_{\theta^k} | 0 \leq k \leq K\} \right)$. \\
\end{algorithm} 

% \section{More Discussions on LARA}
% \label{sec:understanding}
% We use a running example to illustrate why LA-Attention helps extract potentially profitable samples followed by the discussion of the computational complexity of LARA.

% \paragraph{LA-Attention has a proper estimation of $p_{\vx_t}$.}
% We use a visual and intuitive example to further understand the effectiveness of the~\emph{metric learning module} incorporated into the LA-Attention method, as shown in Fig.~\ref{fig:tsne}. 
% We search for potentially profitable~\emph{samples with high $p_{\vx_t}$} via the $\hat{p}_{\vx_t}>thres$ criterion~($thres$ equals 0.5 in this demo).
% We aim to verify whether $\hat{p}_{\vx_t}$ calculated by LA-Attention is a proper estimation of the predefined $p_{\vx_t}$.
% In Fig. \ref{fig:tsne}(a), We plot embeddings of randomly sampled 1000 points in the ETF dataset using t-SNE \cite{van2008visualizing}. 
% We find that the positive and negative points are mixed together and there are only 174 positive samples. 
% It exhibits the return distribution with almost the zero mean, and $\hat{p}_{\vx_t} \approx 0.174$ are far away from the desired $p_{\vx_t}$.
% After introducing the \emph{localization module} (Fig. \ref{fig:tsne}(b)), we also randomly sampled 1000 points with $\hat{p}_{\vx_t}>thres$, and find that there are 279 positive samples. The mean return of potentially profitable samples is obviously larger than zero, which indicates the effectiveness of the \emph{localization module}. 
% However, the negative ones still account for a large part and the estimated $\hat{p}_{\vx_t}$~(0.279) is much less than 0.5. 
% In Fig.~\ref{fig:tsne}(c), further incorporated into the \emph{metric learning module}, the number of the positive samples (424) accounts for almost half of all samples, which is in line with expectations that $\hat{p}_{\vx_t}$ equals 0.5 and is a proper estimation of $p_{\vx_t}$.
% We also find that the learned embedding has a more compact structure and clearer distinct boundaries. 
% It achieves the $8.42E\text{-}4$ mean return, which is much larger than zero with a greater margin compared with (a) and (b).
% Hence, this learned distance metric can assist LA-Attention method to distinguish potentially profitable \emph{samples with high $p_{\vx_t}$}.

% \subsection{Masked Attention Model}
% % In \emph{locality-aware attention}, we propose the \emph{masked attention model} to extract the potentially profitable samples by attending to label information of samples in the neighborhood. 
% % Specifically, it divides the feature space of training samples into distinct regions with respect to the results of \emph{masked attention model} (Sec. \ref{sec:attention}).
% % % and gets potentially profitable samples in the light of the results of \emph{locality-aware attention} (Sec. \ref{sec:attention}). 
% % % As a consequence, 
% % Therefore, a natural question arises here: 
% % \emph{Is masked attention model useful for extracting potentially profitable samples?}

% We use an intuitive example to further study the \emph{masked attention} model in Fig. \ref{fig_case}.
% Even though the optimal linear classifier (omitting the bias term for convenience) is determined\footnote{This conclusion is intuitive, and the rigorous mathematical proof can refer to \cite{bishop2006pattern}.}, $y = x$ , to classify $\mathcal{N}\left( \left(-2,2\right), 4I_2 \right)$ and $\mathcal{N}\left( \left(2,-2\right), 4I_2 \right)$, the actual classifier built over the sampled datasets deviates from the optimal classifier owing to the insufficient sample size and noise, especially in the middle region where positive and negative samples are mixed together. 
% Intuitively, extracting \emph{super-class} samples in the blue and red regions with less noise and training classifiers over them can generate a more robust predictor nearer to the optimal line, which is not susceptible to the \emph{noisy} samples out of the \emph{super-class} area.
% In the testing phase, we merely focus on the samples on the \emph{super-class} area, which are easy to be distinguished with respect to the learned predictor.
% % in the green region.
% Hence, the \emph{locality-aware attention} algorithm, which trains and predicts on the \emph{super-class} samples in the blue and red regions, is more robust to the deviation of the learned decision boundary and generate real profitable signals.
% % and deserves further study.

% \begin{figure}[htbp]
% 	% \setlength{\belowcaptionskip}{-0.5cm}
% 	\centering
% 	\includegraphics[width=.40\textwidth]{pics/case-study.pdf}
% % 	\vspace{-0.85cm}
% 	\caption{The didactic example for illustrating \emph{locality-aware attention}. Sample 200 data points from $\mathcal{N}\left( \left(-2,2\right), 4I_2 \right)$ and $\mathcal{N}\left( \left(2,-2\right), 4I_2 \right)$ as positive and negative training samples, respectively. Testing samples are from the same distribution. The blue region (upper left) stands for the super-positive area with less noise. The same for the super-negative area in the red region (lower right). For a linear classifier $y = w \cdot x$, the red dotted line represents the optimal solution and other solutions deviate from the optimal one (mainly located in green) due to insufficient sample size and noise.}
% 	\label{fig_case}
% \end{figure}

% \vspace{-0.8em}
% \paragraph{Computational Complexity.}
% \label{appendix:complexity}
% Due to the low feature dimension in our task (only 40), the optimization speed of $d \times d$ sparse Mahalanobis distance matrix in Metric learning (SDML) is fast. 
% We denote $N$ and $N_{\text{test}}$ as the number of training data and testing data respectively.
% Let $d$ be the feature dimension.
% For LA-Attention, the main time consumption is to search for neighbors of input samples and we adopt the approximate nearest neighbor search method, \ie,~HNSW~\cite{malkov2018efficient}. 
% HNSW costs $\mathcal{O}\left(N \log N \right)$ time for construction of the data structure.
% There are $(N+N_{\text{test}})$ samples needed to search for neighbors, each of them takes $\mathcal{O}\left(\log N\right)$ time. 
% Hence, it takes $\mathcal{O}\left(\left(2N+N_{\text{test}}\right)\log N\right)$ time in LA-Attention in total.
% In addition, we define the time for constructing one estimator as $T_c$ in \emph{LightGBM} \cite{ke2017lightgbm}. Let $N_l$ be the number of estimators and $T_p$ be the time for predicting the testing data. RA-Labeling repeats the training and testing process for $K$ times, thus, the time cost is $\mathcal{O}\left(K\left(N_lT_c + T_p\right)\right)$ in total. Note that searching for neighbors in LA-Attention and predicting results via tree estimators can all be well paralleled, so we can react quickly in the actual financial market.

% \begin{figure}[tbp]
% 	% \setlength{\belowcaptionskip}{-0.5cm}
% % 	\vspace{-0.3cm}
% 	\centering
% 	\includegraphics[width=.42\textwidth]{pics/t-sne.pdf}
% 	\vspace{-0.3cm}
% 	\caption{Visualization of randomly sampled 1000 points with t-SNE and their corresponding return distributions. \textbf{Left:} the input dataset. \textbf{Middle:} \emph{samples with high $p_{\vx_t}$} selected by the \emph{localization module} only. \textbf{Right:} \emph{samples with high $p_{\vx_t}$} selected by LA-Attention~(\emph{localization module}+\emph{metric learning module}).}
% 	\vspace{-0.4cm}
% 	\label{fig:tsne}
% \end{figure}
